Quantum Data Management in the NISQ Era: Extended Version

Quantum computing has emerged as a promising tool for transforming the landscape of computing technology. Recent efforts have applied quantum techniques to classical database challenges, such as query optimization, data integration, index selection, and transaction management. In this paper, we shift focus to a critical yet underexplored area: data management for quantum computing. We are currently in the noisy intermediate-scale quantum (NISQ) era, where qubits, while promising, are fragile and still limited in scale. After differentiating quantum data from classical data, we outline current and future data management paradigms in the NISQ era and beyond. We address the data management challenges arising from the emerging demands of near-term quantum computing. Our goal is to chart a clear course for future quantum-oriented data management research, establishing it as a cornerstone for the advancement of quantum computing in the NISQ era.

==> Data_full_ver.tex <==
\section{Data in quantum era}
\label{sec:def}


Since the 1960s, database systems have been developed and operated on classical computers, which rely on bits as their fundamental units of data. Classical bits represent binary values of 0 or 1. In the development of quantum computers and their associated software systems, a key challenge in advancing quantum computers and their associated software systems is the implementation of qubits \cite{doi:10.1126/science.354.6316.1090}, the quantum counterparts of classical bits. Following the principles of quantum mechanics, qubits possess unique properties such as superposition and entanglement. These properties fundamentally differentiate quantum data from classical data, which we will explore in this section.
 

\subsection{Classical data vs. quantum data}\label{sec:classical-vs-quantum-data}

\emph{Classical data} is the information that is collected, processed, and stored with traditional computing methods. Today, most of the classical data is stored and queried using database systems such as relational databases, document stores, graph databases, and vector databases \cite{dbms}.

We refer to \emph{quantum data} as information that is collected and processed using \emph{quantum computing devices}, i.e., computing devices that follow the rules of quantum mechanics to their advantage \cite{nielsen2010quantum}. \ % using quantum computing methods \cite{nielsen2010quantum}.
% \tim{explicitly use the laws of quantum mechanics to their advantage (as an ordinary laptop is also governed by quantum mechanics ;))}
Quantum data is represented by qubits, and the data computation operations are conducted through quantum gates. For instance, a recent vision \cite{huang2022quantum} shows a possible future:  quantum data is collected from quantum sensing systems, e.g.,  discover a black hole \cite{Bland-Hawthorn:21}; then stored and processed via the quantum memory of a quantum computer.
We list key differences between quantum and classical data below to help understand the new features of quantum data.

\underline{\emph{1. Quantum data is probabilistic.}} 
Unlike a classical bit can only be 0 or 1, a quantum bit can be in \emph{superposition}. \ 
Mathematically, a zero state and a one state may be represented by a unit vector in the \emph{standard basis}, that is, the zero state $\ket{0}$ is represented by the vector $(1,0)$ and the one state $\ket{1}$ is represented by the vector $(0,1)$. \ 
A single qubit state, denoted $\ket{\psi}$, may be represented by a superposition, i.e., a linear combination, of $\ket{0}$ and $\ket{1}$: $\ket{\psi}=\alpha\ket{0}+\beta\ket{1}$, or equivalently the unit vector $(\alpha,\beta)$, for some pair of complex numbers $\alpha,\beta$ satisfying $|\alpha|^2+|\beta|^2=1$. \ 

The probabilistic nature arises when a \emph{measurement} is performed. 
When a measurement is performed on the state $\ket{\psi}$, an outcome 0 is obtained with probability $|\alpha|^2$ and 1 obtained with probability $|\beta|^2$, and the state permanently changes to the obtained outcome. \ 

% A classical bit can only be 0 or 1. \ 
% Similarly, a quantum state can be in the zero state $\ket{1}$ or in the one state $\ket{1}$, or any superposition of the two. \ 
% The first difference between a classical and quantum bit is: a classical bit can only be 0 or 1, like a coin with a head or tail; but a qubit can exist in a \emph{superposition} of $\ket{0}$ and $\ket{1}$ at the same time.
% % The possible states of a qubit are more than $\ket{0}$ and $\ket{1}$.    
% Mathematically, the superposition of a qubit is represented using the linear combination of basic states $\ket{0}$ and $\ket{1}$: 
% \begin{equation*}
% \vspace{-0.1cm}
% \ket{\psi} = \alpha \ket{0} + \beta \ket{1}.
% % \vspace{-0.1cm}
% \end{equation*}
% The states $\ket{0}$ and $\ket{1}$ may be represented as orthonormal vectors in a two-dimensional space, e.g., 
% \begin{align}
%     \ket{0} \mapsto
%     \left[\begin{array}{c}
%          1 \\ 0 
%     \end{array}\right]
%     \qquad 
%     \ket{1} \mapsto
%     \left[\begin{array}{c}
%          0 \\ 1 
%     \end{array}\right].
% \end{align}
% The state $\ket{\psi}$ is a linear combination of the two vectors. 
% Here, $\ket{\psi}$ is the state of the qubit with $\alpha$ and $\beta$ being complex numbers. 
% $\alpha \ket{0} + \beta \ket{1}$ means that a qubit would be measured as 0 with the probability of $\left | \alpha \right |^{2}$ and 1 with the probability of $\left | \beta \right |^{2}$. 
% Such a state is also called a pure state, as opposed to a mixed state we will explain later. \ 
\begin{exmp}[A pure state] Consider the qubit in the following superposition:
	\label{exmp:superposition}
\begin{equation*}
% \vspace{-0.1cm}
\ket{\psi} =  \frac{1}{\sqrt 2} \ket{0} +  \frac{1}{\sqrt 2} \ket{1}  
% \vspace{-0.1cm}
\end{equation*}

When measuring this qubit, there is an equal probability of 50\% ($\left | \alpha \right |^{2}=\left | \beta \right |^{2}=\frac{1}{ 2}$) to get a 0 or 1 as a result.
\end{exmp}

In physical implementations, a classical bit 0 and 1 may describe a wire in low and high voltage, respectively.
Similarly, a state $\ket{0}$ or $\ket{1}$ represents the a particle in low or high energy in a two-level system, respectively. \ 

% \tim{Is it needed to explain mixed states?}\shih{Noise is a channel which maps a pure state to a mixed one.}
A quantum state in its most general form can be any probabilistic mixture of pure states. \ 
A pure state $\ket{\psi}$ may be represented as a density matrix by multiplying its transpose conjugate, denoted $\bra{\psi}$, and itself, i.e., $\proj{\psi}$. \
A mixed state $\rho$ can be mathematically written as a convex combination of pure states in the form of rank-1 matrices, i.e., $\rho=\sum_i p_i \proj{\psi_i}$ for pure states $\ket{\psi_1},\ket{\psi_2},\ldots$ \ 
\shih{perhaps we can talk about quantum noise without saying it maps a pure state to a mixed state, and then we remove the introduction to mixed states.}
% \shih{a few brief explainations about bra, ket, density matrix}
\begin{exmp}[A mixed state]
A quantum state with probability $1/3$ in $\ket{0}$ and $2/3$ in $\ket{1}$ can be written as a density matrix 
\begin{align}
    \frac{1}{3}\ket{0}\!\bra{0} + \frac{2}{3}\ket{1}\!\bra{1},
\end{align}
where $\bra{\psi}$ denotes the transpose conjugate of state $\ket{\psi}$, and $\ket{\psi}\!\bra{\phi}$ denotes the matrix multiplication of $\ket{\psi}$ and $\bra{\phi}$. 
\end{exmp}
% \tim{would be useful for later on to mention that an $n$-qubit quantum state is a $2^n$ long vector} \shih{done below}

In classical computing, individual bits can be concatenated to form a bit string, e.g., three-bit string `010'.
Similarly, we may concatenate qubits into a multi-qubit state. 
In this case, an $n$-qubit state can be represented as a superposition of $\ket{x}=\ket{x_1}\ket{x_2}\ldots\ket{x_n}$ for $x\in\{0,1\}^n$, or equivalently a vector of $2^n$ components. \ Later, we will discuss a three-qubit state in Fig.~\ref{fig:tensors_example}a.

\underline{\emph{2. Quantum data is fragile.}} 
While quantum computers are anticipated to outperform classical computers in computational power. However, with current quantum technology in the NISQ era, quantum resources remain scarce,  and quantum data is prone to noise.  \ 
Quantum noise, resulting from unintended couplings with the environment, can severely degrade the power of quantum computers \cite{unruh1995maintaining}. Mathematically, quantum noise is modeled by quantum processes that map pure states to mixed states. Since quantum states encode information in both amplitude and phase, realistic noise models are often written as combinations of information decaying in amplitude and phase. \ 
Two commonly considered noise models are \emph{amplitude damping} and \emph{phase damping}. \ 


The amplitude damping noise, describing the dissipation of energy (hence the information), maps a state to another with more weights on the ground state $\ket{0}$. \ The phase damping noise describes the dissipation of information without energy loss and introduces fluctuation in the relative phase. \ 
These noise models allow us to mathematically describe \emph{decoherence} \cite{preskill1999lecture}, a phenomenon where pure quantum states evolve into mixed states, resulting in the gradual loss of quantum information.

% A bit flip noise, a straightforward quantum analogue of classical bit flipping, can be modeled as an swap between basis vectors $\ket{0}$ and $\ket{1}$ with probability determined by the noise rate \cite{nielsen2010quantum}. \ 
% A phase flip, which may be viewed as a bit flip in a rotated basis, changes the relative phase between components in the superposition.
% For example, a phase flip maps the state $\ket{\psi}$ in Example~\ref{exmp:superposition} to $(\ket{0}-\ket{1})/\sqrt 2$. \ 
% Though they are both uniform superposition on a single qubit, the statistics of measurement outcomes in different bases are different. \ 


 
\tim{Is it useful to give numbers? i.e. the coherence times for typical hardware (superconducting has lowest, I think (while they are the hardware for the devices with the most qubits at the moment!), and NV centers in diamond the highest)}
\shih{I'm not that familiar with the current experimental status, perhaps Tim can add it?}


\underline{\emph{3. Quantum data can be entangled.}}
Another difference between qubits and bits is \emph{entanglement} 
\cite{einstein1935can}, 
% \cite{schrodinger1935discussion}, 
referred to as the 
\emph{spooky action at a distance} by Einstein. Imagine two qubits with qubit A being in Amsterdam and qubit B in San Francisco. When qubit A and qubit B are entangled this means their states are correlated. The \emph{spooky} part is that if we measure qubit A in Amsterdam and find it in a state of 0 (or 1), we instantaneously know the state of qubit B is 0 (or 1), even though it is far away in San Francisco. This correlation is maintained independently of the physical distance between them.  With below example, we introduce one of the most well-known states for entanglement, \emph{Bell's state}.
% , also known as the \emph{EPR pair}.

\begin{exmp} (\textbf{Bell's state}) We extend the one-qubit state in Example~\ref{exmp:superposition} to a two-qubit state as follows:  
	\label{exmp:EPR pair}
\begin{equation*}
\ket{\Psi}=\frac{1}{\sqrt 2}(\ket{00}+\ket{11})=\frac{1}{\sqrt{2}}\begin{bmatrix}
1\\ 
0\\ 
0\\ 
1
\end{bmatrix}
\end{equation*}

\end{exmp}

\tim{is there a way to connect these quantum-specific properties of data to the new challenges with regards to handling data? Why do these properties make data management difficult or at least different?}


% \subsection{Transformation between classical and quantum data} 
\subsection{Quantum-classical data transformation}
\label{ssec:transf}
% \tim{why this title? where are the transformations?}
\tim{It is not clear to me what message the details on noise processes and measurements convey. }
% Also: maybe also good to mention that measurement changes the state}
% \tim{is it useful to define the elements of a quantum circuit/quantum algorithm here? Will be talked about later in secs 3 and 4}
\shih{mentioned quantum algorithms, and the circuit model; not sure what are the best terms referring to tranformations between classical and quantum data}
% \shih{from classical data to quantum states: encoding, e.g., basic (1-to-1 classical to quantum bit, X gate), rotation, amplitude of qubit (supercondensed encoding).
% From quantum states to classical data: measurement. (done)}

\subsubsection{From quantum data to classical data} To use quantum computers to get useful information for the classical world, transformations that maps classical data to quantum date and vice versa are essential ingredients. \ 
These transformations can be described as quantum algorithms. \ 


%-------------------------include in the journal ver.-------------------------%
\para{Quantum process and algorithm} A \emph{quantum process} (also called quantum channel) maps one quantum state to another state \cite{nielsen2010quantum}. \rihan{?}
% \rihan{here maybe a citation so db people can check?}\shih{done}
A special case is the unitary operators, which refer to reversible operations on quantum states. \ 
More generally, quantum process may include irreversible operations, which may be implemented by an application of a unitary operator followed by discarding part of the qubits \cite{nielsen2010quantum}. \ 
%-------------------------------------------------------%
\para{Quantum algorithms, circuits, and gates} A quantum algorithm is a carefully designed quantum process that maps some input classical or quantum data to desired output data \cite{nielsen2010quantum}. \ 
The most commonly used model to describe quantum algorithms is the quantum circuit model. 
%, which we briefly introduce in this section. \ 
 A unitary operator may be composed by a sequence of basic unitary operations, called quantum gates, acting on appropriate qubits. \ 
The sequence of quantum gates forms a quantum circuit.
A set of quantum gates is universal if it can approximate any unitary operator to desirable precision \cite{nielsen2010quantum}. \ 
A widely known universal gate set consists of Pauli gates (including $X,Y,Z$ gates defined by Pauli matrices), the Hadamard gates (see Example~\ref{exmp:hadamard}), the $T$ gate, and the controlled-NOT (CNOT) gate \cite{nielsen2010quantum}. \ 

\begin{exmp}\label{exmp:hadamard}
    The Hadamard gate is a unitary operator, which maps $\ket{0}$ to $(\ket{0}+\ket{1})/\sqrt 2$, and $\ket{1}$ to $(\ket{0}-\ket{1})/\sqrt 2$. \ 
    In matrix form, the operator is represented as 
    \begin{align}
        \frac{1}{\sqrt 2}\left[\begin{array}{cc}
             1 & 1 \\
             1 & -1
        \end{array}\right]
    \end{align}
    One can easily check that $H^2$ is the identity operator, and this implies that the application of a Hadamard gate is reversible. 
\end{exmp}
% A special case is the unitary operator, which may be viewed as a rotation in the Hilbert space. \ 
% Any general quantum processes can, without loss of generality, be implemented by applying a unitary jointly with auxiliary memory \cite{nielsen2010quantum}. \ 
% \shih{example about unitary operators}



\para{Quantum measurements} To use a quantum computer to get results for computational problems, it is essential to extract classical information from quantum states. \ 
In quantum physics, quantum measurements allow for manipulations on a quantum system to yield classical outcomes. \ \rihan{system}
For example, applying a standard basis measurement on the quantum state $\ket{\psi}$ in Example~\ref{exmp:superposition} yields an outcome $0$ with probability $|\alpha|^2$ and $1$ with probability $|\beta|^2$. \ 
In general, measurement in different bases may be obtained by applying unitary operations followed by a standard basis measurement. \ 
Since a measurement only extracts a random outcome with probability determined by the amplitudes, we do not expect quantum computers to own the full power of parallel computations on exponentially many threads. 

\subsubsection{From classical data to quantum data}
Classical data can be encoded as quantum states in various ways. \rihan{what}\ 
A well-known example to encode two classical bits into one quantum bit is via superdense coding \cite{nielsen2010quantum}: \ 
Alice and Bob share an Bell's state (see Example~\ref{exmp:EPR pair}), and the goal is to allow Alice to send two bits $(a,b)$ to Bob using her half of the state. \ 
To encode the bits in the qubit, she applies an $X$ gate to introduce a bit flip when $a=1$ (and no operation when $a=0$), followed by a $Z$ gate to introduce a phase flip when $b=1$ (similarly, no-op when $b=0$).
Finally she sends her qubit to Bob. \ 
To extract both bits, Bob performs a measurement in a designated basis (called the Bell basis) on the qubits. \ 
The entire procedure allows Alice to transmit one qubit for Bob to extract two bits of information, with the help of one shared Bell's state. \ 

% \subsection{NISQ era vs. FTQC era} 
% \label{ssec:nisq}
% The \emph{Noisy Intermediate-Scale Quantum} (NISQ) era \cite{Preskill_2018} represents the current phase in quantum computing, characterized by the development and deployment of quantum processors with tens \cite{kelly2015state} to hundreds of qubits \cite{kjaergaard2020superconducting, gambetta2020ibm}. 
%  %on the order of 10-20, 50-100
%  % These quantum devices, while powerful, are still limited by significant noise and error rates, which hinder their ability to reliably perform long, complex calculations \cite{clerk2010introduction}. 
%  % One of the ongoing quantum research goal focuses on mitigating noise through error correction techniques.\shih{change previous sentence to both directions. in the NISQ era, qubits are scarce and fault tolerance is resource prohibited; this sentence should be placed somewhere else?} 
%  % and developing hybrid quantum-classical algorithms that leverage the strengths of both quantum and classical computing methods \rihan{Why the following reference?} \cite{mcardle2020quantum}. 
%  %FG. Comment to myself. Not so sure about the following paragraph because it seems to already say where we believe that qdm should happen at a level where the noisy nature is present and plays a role. Let's discuss what we want to say here as the next paragraph is part of the vision?
%  % \all{Floris says: The following para already seems part of the vision? I would dedicate this paragraph only to describe that we are looking at NISQ here.}
%  In the near term, quantum data management research will be constrained by the noisy nature of quantum processors. That is, we should look into new methods and database systems robust to qubit errors and also seek hybrid quantum-classical solutions. 
 


% The \emph{Fault-Tolerant Quantum Computing} (FTQC) era \cite{DBLP:conf/focs/Shor96, DBLP:conf/qcqc/Gottesman98, PhysRevA.57.127} looks beyond the NISQ era and envisions quantum systems capable of executing large-scale, error-free computations. Achieving fault tolerance requires the implementation of robust quantum error correction codes and the construction of logical qubits from multiple physical qubits \cite{fowler2012surface}. In this era,  ideally, quantum databases could fully realize their potential, handling vast amounts of data with unprecedented efficiency. \tim{not sure that we should mention q computers handling large amounts of data (see also 3rd misconception below)}
% %FG: Comment to myself. The following paragraph seems to come out of promotion folder for QC. Is this what *we* believe?
% The FTQC era promises to revolutionize fields such as cryptography, material science, and complex system simulations \cite{campbell2017roads}, possibly demanding  
% % \rihan{Why would qdms be at the forefront? It may be useful to make this claim stronger by means of an example? }
% future data management systems coping with the quantum information theory and error-corrected quantum computers in the FTQC era. 
% %FG: Comment to myself: Let's discuss this as the next paragraph is part of the vision?
%  \floris{The following para already seems part of the vision? I would dedicate this paragraph only to describe that we are looking at NISQ here. }
% A few decades from today, quantum data management theory and systems will be needed for scalable quantum algorithms and use cases, which will seamlessly integrate with existing classical database technologies.

\subsection{Avoiding a few misconceptions} 
\label{sec:misconceptions}
%-------------------------------------------------------
% \rihan{a rigorous discussion that quantum-related data management is in infantile state: we are really just talking about qubits, not data; limited no. of qubits; lower-level gate-based computation; noisy}
% \tim{todo FILL with similarities and differences. ``Therefore a structured approach is needed''}
%-------------------------------------------------------
 
% \floris{The aim of this section is not very clear to me}
% \tim{I updated, better now?}
%Quantum computing fundamentally differs from classical computing, often leading to misinterpretations about its capabilities and limitations.
We here aim to take away a few potential misunderstandings before sketching our vision in the next sections.
%We here aim to take away a few potential misunderstandings about quantum computing and its relation to data management before sketching our vision in the next sections.
%These misconceptions can misdirect research directions in data management for quantum computing. Next, we aim to clarify a few common misunderstandings by examining key quantum computing principles and their implications.

% Similarities:
% \begin{itemize}
%     \item ...
% \end{itemize}
% Differences:
%\tim{@Rihan:
%\begin{itemize}
%\item{ I also shortened the text (original commented out). Please check}
%\item{I removed underline because it breaks latex formatting}
%\item{to clarify: superdense coding is for faster communication, not better compression: communicating 2 bits by sending 1 qubit, which was entangled beforehand to a qubit on the receiver's side.}
%\item{I rewrote the `data loading' part to also address Floris' question ``Perhaps a silly question, but these non-cloning, non-deletion and non-copying properties of quantum, don’t they rule out a native implementation of database, that is, if one would attempt to store data inside the qubits, there will be no way to do standard operations (like copy/delete) on them.''}
%\end{itemize}
%}
\begin{itemize}[leftmargin=*]
    \item \emph{A quantum computation does not perform parallel computation with exponentially-many processors.}
Classical parallel computing relies on splitting the task across many processors, each working \emph{independently}.
Quantum computing might at first sight look similar as a quantum state also represents multiple (exponentially-many) possibilities.
However, these possibilities are in a single \emph{superposed} state.
Moreover, to extract information from the state, one needs measurement, which returns only one random outcome and also permanently changes the state.
    % \item \emph{\underline{Quantum computers do not run parallel computation}}: 
%    While quantum algorithms can exhibit substantial speedups for various computational problems, a common misconception of why this is possible is that quantum computers achieve fast computation by creating superpositions to execute exponentially many threads simultaneously. \ 
%    As discussed in Section~\ref{sec:classical-vs-quantum-data}, quantum measurements allow for the extraction of classical information from quantum states. \ 
%    Upon measurement, only one random outcome is extracted from the state, and the state changed permanently to the example we observe.
These make a quantum computation qualitatively different.
%Consequently, a quantum computation is qualitatively different from a parallel computation on exponentially-many processors.
% (it is even expected, but not proven(?), to be strictly weaker in the complexity-theoretic sense~\cite{}).
%It is therefore incorrect to say that quantum computing is the same as parallel computing with exponentially-many processors, 
%even though its computation power in the complexity-theoretic sense has not yet been fully pinpointed yet~\cite{}.
%quantum computing different from parallel computing with many processors, although the unconditional complexity-theoretic separation remains unproven.
%It is expected that there are tasks that quantum computers can efficiently tackle
%From a complexity-theory perspective, quantum computing is separate from
%lies somewhere in between parallel computing with exponentially-many processors (strict separation~\cite{}) and single-core classical computing (separation only proven for tasks with restricted input, i.e. promise problems~\cite{}).
%    \floris{I understand what you want to say but the latter goes beyond the capabilities of understanding by VLDB folks :-). Perhaps something more simple like this suffices: "Classical parallel computing relies on splitting the task across many processors, each working \emph{independently}. Quantum computing, on the other hand, handles multiple possibilities in a \emph{superposed} and \emph{entangled} state, and extracts one random outcome from the state, hereby permanently changing the state."}
%

\item \emph{There exist other quantum computers and database applications than only quantum annealers and QUBO solving.}
Quantum annealers~\cite{schonberger2023quantum} are a different type of quantum computers than the gate-based type explained above.
Recent works on accelerating database operations \cite{trummer2016multiple, fankhauser2021multiple, fankhauser2023multiple, SchonbergerSIGMOD22, schonberger2023SIGMOD, schonberger2023quantum, ScherzingerVLDB2023demo, GroppeIDEAS20, OJCC,  groppe2021optimizing} have a heavy focus on quantum annealers because some database problems are formulated as \emph{quadratic unconstrained binary optimization} (QUBO) problem, which are natural to solve on quantum annealers.
Although quantum annealing is in principle capable of running any quantum computation~\cite{aharonov2008adiabatic}, the focus is typically to solve QUBO on a specialized, non-universal quantum annealer such as the one by D-Wave Systems Inc.~\cite{dwavewebsite}.
% implementing the transverse Ising Hamiltonian https://journals.aps.org/rmp/pdf/10.1103/RevModPhys.94.015004
Our vision is not restricted to quantum annealing and QUBO, and broadens the view to universal quantum computing and other applications.
%However, gate-based quantum computers are universal, potentially enabling opportunities for database research that annealers do not.\tim{such as... Let's link to the rest of the paper} \floris{Is this all still true given \url{https://arxiv.org/abs/quant-ph/0405098}?}
  
%    Quantum computers come in various models, including quantum annealers and physical systems for implementing gate-based models such as superconducting \cite{}, semiconductor quantum dots \cite{}, and trapped ion \cite{}. %, neutral-atom, topological, and photonic quantum computers. 
%    Recent works on accelerating database operations \cite{trummer2016multiple, fankhauser2021multiple, fankhauser2023multiple, SchonbergerSIGMOD22, schonberger2023SIGMOD, schonberger2023quantum, ScherzingerVLDB2023demo, GroppeIDEAS20, OJCC,  groppe2021optimizing} have a heavy focus on quantum annealers and quantum-inspired classical hardware, i.e., digital annealers \cite{schonberger2023quantum}. The reason is, take query optimization \cite{trummer2016multiple, schonberger2023SIGMOD} for example, compared to gate-based quantum computers, quantum/digital annealers
%    provide a larger number of qubits/bits and better connectivity, which facilitates query optimization over more tables. Accordingly, the database problems \cite{trummer2016multiple, fankhauser2021multiple, fankhauser2023multiple, SchonbergerSIGMOD22, schonberger2023SIGMOD, schonberger2023quantum, ScherzingerVLDB2023demo, GroppeIDEAS20, OJCC,  groppe2021optimizing} are formulated as \emph{quadratic unconstrained binary optimization} (QUBO) problem, which is a typical problem solved by annealers.  
%    % So far, database studies only looked into QUBO \cite{trummer2016multiple, fankhauser2021multiple, fankhauser2023multiple, SchonbergerSIGMOD22, schonberger2023SIGMOD, schonberger2023quantum, ScherzingerVLDB2023demo, GroppeIDEAS20, OJCC,  groppe2021optimizing} and variational quantum circuit (VQC) algorithm \cite{GroppeQMLBiDEDE23}.  
%    Although quantum annealers or digital annealers offer more qubits and better qubit connectivity for tackling near-term optimization problems in databases, we should also put effort into gate-based quantum computers. 
%    Because quantum annealers are not universal quantum computers, we do not expect them to solve all computational problems that a full-power quantum computer can do. 
%    % \shih{revise the previous sentence to explain why quantum annealer is not as powerful as gate-based models, it solves a subset of problems; maybe with refs}
%    Exploring more quantum algorithms for gate-based models will bring more opportunities in this line of research. 

\item \emph{Loading large relational-database tables into a quantum computer will not be possible in the near term, and will maybe never be advantageous at all.}
In principle, one could load classical data onto a quantum chip by simply copying a single bit onto a quantum bit.
This however does not make use of quantum-computing properties such as superposition, which is crucial for a quantum advantage.
%Loading data to quantum amplitudes is done by
%Loading classical data onto a quantum chip in a way that takes advantage of exponential superposition is done by
%encoding the data as the quantum state's amplitudes.
A functional alternative is to convert the data into a quantum circuit, which is either used directly as part of a quantum algorithm~\cite{suenderhauf2024blockencoding} or outputs a quantum state whose amplitudes hold the classical data~\cite{cortese2018loading}.
%The size of the circuit depends on the data and the used encoding, but is typically at least $O(\log(N))$ large for encoding $N$ classical bits.
For large amounts of data, this data-loading will not be beneficial practically in the near term, as qubits will be limited in number but also in lifetime (see Sec.~\ref{sec:classical-vs-quantum-data}), hindering their ability to store large amounts of data for a long time.
%However, given the decade-long perfectioning of performance and I/O for classical databases and the limited speed, lifetime and accuracy of quantum operations,
It is at the moment not clear for which applications this quantum data-loading will ever outweigh the use of the classical database for acting on the data directly~\cite{aaronson2015read,Preskill_2018}.
% also cite viamontes et al. "Is Quantum Search practical?"
In this work, we consider this question out of scope, as we focus on data management for supporting quantum technologies.
%, in contrast to the converse.
%a quantum data-management advantage.

%sketch how data management can contribute to quantum technologies, instead of the opposite question of 
%This avoids 

%describe different means in which classical data can contribute to a future with a quantum advantage.

%\tim{This is the vision that quantum computers will be good for computationally-hard problems which can be phrased succinctly}
%\floris{The above clearly dispels that an implementation of quantum database which stores all the day is not what one may want to aim for.}
%\todo[inline]{Tim: trying to answer Floris' question here: Perhaps a silly question, but these non-cloning, non-deletion and non-copying properties of quantum, don’t they rule out a native implementation of database, that is, if one would attempt to store data inside the qubits, there will be no way to do standard operations (like copy/delete) on them. }

%For the existing limitation of qubits we cannot process any industrial-level tables in the classical database in a quantum processor due to the constraint of limited quantum resources. It may be not worth the effort to import all classical data into a quantum processor. 
%    Furthermore, it lacks generic methods to transform classical data to a quantum state that encodes the information in the amplitudes, which is essential for quantum algorithms to exhibit speedups (see, e.g., \cite{harrow2009quantum}). 
%    It is important to think about which subset of classical data (or a sketch, metadata) needs to be encoded and passed to a quantum device, and design corresponding quantum algorithms for transforming it to useful quantum states. 

%\todo[inline]{mention loading data onto a quantum chip, which is done by preparing a quantum circuit, not copying}


%For the existing limitation of qubits we cannot process any industrial-level tables in the classical database in a quantum processor due to the constraint of limited quantum resources. It may be not worth the effort to import all classical data into a quantum processor. 
%    Furthermore, it lacks generic methods to transform classical data to a quantum state that encodes the information in the amplitudes, which is essential for quantum algorithms to exhibit speedups (see, e.g., \cite{harrow2009quantum}). 
%    It is important to think about which subset of classical data (or a sketch, metadata) needs to be encoded and passed to a quantum device, and design corresponding quantum algorithms for transforming it to useful quantum states. 


    % \item \emph{\underline{query model is different}}: superposition is different from parallel computing;
    % cannot extract classical information in general without destroying the properties of the quantum state. Measurement destroys information.
    


\end{itemize}




==> Littau.tex <==
\subsubsection{Execution Time}\label{sssec:time}
The execution time results reveal a nuanced tradeoff between sparse and dense circuits. Sparse quantum circuits, such as the W State circuit, showed significant runtime advantages with database systems. As shown in figure \ref{fig:wstate_time}, the RDBMS implementation is comparable to state-of-the-art methods, especially for higher qubit counts. However, for smaller qubit counts (e.g., below 20 qubits), NumPy outperformed some of the database systems due to its lower constant overhead and direct handling of tensor operations. \\
As shown in figure \ref{fig:qft_time}, dense ciruits, such as the QFT circuit, exhibited a different trend. Numpy's tensor contraction implementation outperformed PostgreSQL, DuckDB and SQLite, primarily due to its efficient handling of dense tensor operations without additional overhead and the COO representation that is used in RDBMS. This highlights that while database systems offer scalability for sparse scenarios, their performance deteriorates for dense circuits compared to specialized numerical libraries. However, this also shows a potential for improvement on the database side, since at least some of the reasons for bad performance lie in the naive data representation used in this implementation. While both implementations show an exponential increase over the number of qubits, the increase for RDBMS implementations is even higher as previously shown in the theoretical time complexities in table \ref{tab:time}.

\rihan{Littau: Addition on the Query Creation} As discussed in the previous section, the creation of SQL queries introduces an additional time overhead in the current implementation. This overhead results from constructing a string representation of the SQL query, where the string's length scales with the number of gates in the quantum circuit. The time complexity of this process is thus proportional to the number of gates, a relationship reflected in Figure \ref{fig:querytime}.

The time overhead is attributable to two main factors: the translation of tensors into COO-formatted database relations and the conversion of the contraction path into a sequence of \texttt{JOIN} operations. Each of these steps introduces computational effort that grows linearly with the number of gates or circuit depth. However, this overhead is separate from the actual contraction operation, which represents the core simulation task.

Separating the evaluation of query creation from the contraction phase allows for a more accurate assessment of the simulation performance. While query creation time is an artifact of the current implementation, it is not a fundamental limitation of using RDBMS for quantum circuit simulation. Future improvements, such as pre-storing tensors in the database or optimizing the contraction path generation process, could significantly reduce this overhead. This separation ensures that our performance comparisons between NumPy and RDBMS implementations reflect the true efficiency of the contraction operation rather than the idiosyncrasies of the query generation process. 

\subsubsection{Discussion} \label{sssec:b4discussion}
The preliminary results presented in this section reveal a compelling case for leveraging relational database management systems (RDBMS) to simulate quantum circuits with sparse intermediate states. Sparse quantum circuits, such as those used to prepare W states, exemplify the benefits of leveraging the core strengths of RDBMS, namely, efficient memory utilization and advanced query optimization of sparse representations. These systems are intrinsically designed to handle sparse data and optimize operations like filtering, joining, and aggregating, which align well with the mathematical and structural characteristics of sparse quantum states.\\

\vspace{0.2cm}
\begin{myframe}[roundcorner=3pt,innerleftmargin = 5pt]
{\bf Q1.} \textit{Should we push the simulation workload to existing DBMSs?}
\end{myframe}

One of the most significant advantages of using RDBMS for sparse circuit simulation is their memory efficiency. Relational databases are designed to store and process large datasets with high sparsity, avoiding the overhead associated with explicitly representing zero or negligible values. This makes them particularly suitable for simulating quantum circuits where the state space scales exponentially with the number of qubits but remains predominantly sparse due to the limited number of non-zero amplitudes.\\

Moreover, modern RDBMS systems are highly scalable, with robust indexing mechanisms, partitioning strategies, and distributed architectures that enable the efficient handling of very large datasets. These features allow them to handle high-qubit-count simulations without the scalability issues that traditional numerical libraries often face, making them a strong candidate for specialized quantum simulations in distributed or cloud environments.\\

RDBMS are equipped with sophisticated query optimizers capable of transforming high-level operations into efficient execution plans. When simulating quantum circuits, this translates to the potential for automating and optimizing complex operations like tensor manipulations and sparse matrix multiplications. Although the current implementation uses a rudimentary approach, the inherent ability of databases to optimize query execution suggests that tailored SQL-based formulations for quantum operations could yield significant performance gains.\\

For instance, integrating concepts from state-of-the-art simulation techniques like Matrix Product States (MPS) into RDBMS workflows could result in a novel hybrid approach. By rethinking MPS-style simulations within the relational algebra framework, one could develop efficient algorithms that exploit database indexing and partitioning to simulate sparse circuits even more effectively.\\

While sparse quantum circuits demonstrate advantages when simulated with RDBMS, dense circuits such as Quantum Fourier Transform (QFT) and Quantum Phase Estimation (QPE) circuits present a more significant challenge. These circuits require dense tensor contractions, where the overhead of translating these operations into SQL queries and the lack of direct support for dense linear algebra within RDBMS become bottlenecks. Numerical libraries like NumPy or TensorFlow are more suited to such workloads due to their direct support for tensor operations.\\

However, this context-specific limitation does not diminish the value of RDBMS for specific quantum circuit classes. Instead, it underscores the importance of identifying and targeting use cases where the strengths of RDBMS — such as handling sparsity, indexing, and efficient query execution — can be fully leveraged.\\

The preliminary results presented here are compelling because they were achieved without any domain-specific optimizations of the RDBMS workflows. This suggests an opportunity for further research to enhance the performance of quantum circuit simulations using relational databases.\\

The promising preliminary results underscore the viability of RDBMS as a platform for quantum circuit simulation, particularly for sparse circuits. While the initial implementations are rudimentary, they reveal a potential for optimization and innovation. By building on the inherent strengths of RDBMS—scalability, memory efficiency, and query optimization — future research can benefit from the integration of RDBMS for simulating specific classes of quantum circuits. \\

 \vspace*{0.2cm}
\begin{myframe}[roundcorner=3pt, innerleftmargin = 5pt]
{\bf Q4.} \textit{What are good data representations -- possibly beyond tensors -- for supporting simulations?} 
\end{myframe}
 

The choice of data representation is a critical factor in determining the efficiency and scalability of quantum circuit simulations. The exploration of tensor networks and Matrix Product States (MPS) highlights distinct trade-offs between exactness, memory efficiency, and computational complexity.

Tensor networks, when implemented using RDBMS, offer a promising avenue for exact simulation results. By leveraging relational database features such as sparse indexing, query optimization, and scalable storage, RDBMS-based tensor networks achieve competitive performance while maintaining exactness. In contrast, MPS provides an approximate representation that is particularly memory-efficient, especially for systems with low or moderate degrees of entanglement.

The distinction between these representations becomes even more pronounced when additional sparsity is exploited in the MPS framework. This opens the door to tuning the accuracy of MPS simulations to accommodate higher degrees of entanglement while preserving memory efficiency. A critical question remains: how does the RDBMS implementation of tensor networks perform against MPS in scenarios where memory constraints and simulation accuracy are simultaneously critical? Preliminary results suggest that RDBMS implementations could offer a unique balance, providing exact results with scalable performance, particularly for circuits with sparse characteristics.

Future work in this area could explore hybrid representations, where different parts of a circuit utilize the most suitable data representation. For example, highly sparse regions could leverage RDBMS-backed tensor networks for exact simulations, while regions with higher entanglement could benefit from approximate MPS-based techniques. This approach could optimize both memory usage and simulation accuracy, further validating the versatility of RDBMS as a simulation platform.\\

\vspace{0.2cm}
\begin{myframe}[roundcorner=3pt,innerleftmargin = 5pt]
{\bf Q3.} \textit{Can we build an optimizer for simulations?} 
\end{myframe}
 
An effective optimizer for quantum circuit simulations must consider both the structural characteristics of the circuit and the properties of the chosen simulation backend. Our investigation into sparse circuits such as W State and GHZ preparation circuits has revealed that key characteristics, like the degree of sparsity and entanglement evolution, significantly influence simulation performance.

For instance, in the W State preparation, sparsity decreases gradually as the circuit evolves, while for the GHZ state, it remains constant after the initial Hadamard operation. These observations suggest that understanding the dynamic properties of a circuit can inform decisions on how best to simulate it. An optimizer could analyze such characteristics to segment the circuit into sub-circuits that are best suited for specific simulation methods or data representations.

In this context, integrating MPS with RDBMS offers intriguing possibilities. While MPS excels at representing circuits with moderate entanglement, its accuracy can be improved by leveraging additional sparsity, as suggested in Q4. Combining this with RDBMS's ability to efficiently handle sparse data opens up opportunities to design hybrid simulation strategies.

A potential optimizer design could follow these steps:

\begin{enumerate}
    \item \para{Circuit Analysis} Analyze the input circuit to determine key properties such as sparsity, entanglement evolution, and gate connectivity.
    \item \para{Segmentation} Divide the circuit into sub-circuits based on these properties. Sparse regions could utilize RDBMS-based tensor networks, while denser regions leverage MPS or direct numerical libraries.
    \item \para{Representation Assignment} Assign the most efficient data representation to each sub-circuit, optimizing for memory usage, computation time, and desired accuracy.
    \item \para{Parallelization} Exploit the independence of sub-circuits wherever possible to enable parallel simulation, further improving scalability.
\end{enumerate}

Preliminary results already indicate the potential of such an optimizer. The ability of RDBMS to inherently utilize sparsity, combined with the flexibility of MPS for approximate results, makes this approach both viable and promising. Future work could focus on formalizing this optimizer, developing algorithms for automated segmentation, and validating its effectiveness across a broader range of circuit types.

This integrated approach underscores the potential for RDBMS not only as a simulation backend but also as a central component of a more intelligent, adaptable simulation framework that aligns well with the evolving demands of quantum computation research.

\mybox{\textbf{Takeaways:}  
\begin{enumerate}
    \item \textbf{RDBMS for Sparse Circuits:} \\
    Efficient handling of sparsity; performance comparable to MPS for circuits like W and GHZ states.
    \item \textbf{Hybrid and Optimized Approaches:} \\
    Combine RDBMS with MPS; leverage circuit segmentation, sparsity, and parallelization.
    \item \textbf{Future Optimizations:} \\
    Develop and utilize SQL extensions and tailored optimizers to improve RDBMS efficiency for quantum simulations.
\end{enumerate}
}

==> NearTerm_old.tex <==


\section{Near-term research problems}
\label{sec:structure}
\floris{This is Rihan's version}

\begin{figure*}[t]
    \centering
        % \includegraphics[width=\linewidth]{figures/tn-Page-1.drawio.pdf}
                \includegraphics[width=\linewidth]{figures/tn-Page-1.drawio_new.pdf}
    % \includegraphics[width=0.7\linewidth]{figures/tn-Page-1}
    \caption{(a) The 3-qubit  GHZ state  $D=\frac{1}{\sqrt 2}(\ket{000}+\ket{111})$ represented in state vector, whose amplitude is $2^3=8$. (b) GHZ state represented as matrix product states, factorized as three tensors. Each qubit is represented as a tensor. For understandability we write the tensors in  vector/matrix form. 
    (c) Tensor contraction between A and B.
    (d) Quantum operation, Hardmard gate, represented in matrix product operators.} 

    \label{fig:tensors_example}
         \vspace{-0.2cm}
\end{figure*}


In this section, we explore the open research questions across the three paradigms of quantum data management. To provide specific directions,  Sections~\ref{ssec:simu} and \ref{ssec:dbq} focus on a key challenge within Paradigm II, the hybrid classical-quantum approach. By integrating recent advancements from the database community, we identify and discuss emerging research opportunities. In Section 4.3, we broaden our scope to highlight further opportunities across all three paradigms.

\subsection{Quantum challenge of simulation} 
\label{ssec:simu}
% \floris{I think it is perhaps more insightfull to describe the problem of simulation in more details? There are various notions, strong/weak and for some classes, strong is $\#P$-hard whereas weak is poly, in general weak is PH-hard. Clifford stuff is poly. What should we focus on?}
% \floris{Perhaps weak simulation is not good but it may open up extra challenges \url{https://arxiv.org/pdf/2007.15285} Theoretically, connections with tractable circuits \url{https://starai.cs.ucla.edu/papers/ProbCirc20.pdf} maybe be possible as well?}
% \floris{\url{https://arxiv.org/abs/0811.0898} argues against strong simulation ...}
% \floris{Another point: \url{https://arxiv.org/pdf/2406.16142} refers to $d$-sparse quantum states (those having at most $d$  nonzero amplitudes). Not sure whether this is *the* reference for that, but just pointing out sparse things exist in the quantum world.}
\emph{Simulation} is the process of emulating quantum computation,  
allowing researchers to model and analyze quantum processes as if they were running on actual quantum hardware
\cite{young2023simulatingquantumcomputationsclassical, xu2023herculeantaskclassicalsimulation}.\footnote{In this work, by simulation we refer to \emph{classical simulation}. Another similar term is \emph{quantum simulation} \cite{georgescu2014quantum}, which refers to simulating quantum mechanics, a topic studied in physics.} % and out of the scope of this paper. } 
Simulations are of upmost importance in the NISQ era. Indeed, take quantum supremacy \cite{boixo2018characterizing} for example, which aims to demonstrate the superior capabilities of quantum computers over classical computers. 
% In the NISQ era, researchers are still exploring how powerful quantum computing will be,  such as calculation that is infeasible for any classical computer, even the most powerful supercomputers. A core question in near-term quantum computing is quantum supremacy : how much do quantum computing methods and hardware surpass classical computational methods and hardware? 
Large-scale quantum computers are not yet available in the NISQ era, simulation is indispensable to compare scalable quantum computers with classical computers. 
Another use of simulations is for the development of new quantum algorithms. Indeed, simulation enables researchers to design, debug, and validate the correctness of quantum algorithms before deploying them on expensive quantum processors. 
% One of the key challenges in quantum computing is verifying that a quantum algorithm is functioning correctly, especially when quantum hardware is prone to errors. Classical simulators can precisely calculate the expected outcomes of quantum circuits for small to moderate-sized systems. By comparing the outputs of quantum hardware to those of a classical simulation, researchers can validate the correctness of quantum algorithms and ensure they are implemented as intended.
% \floris{I would also briefly explain what simulation actually entails. }
% Using classical representation and methods to simulate quantum computations, is one of the main driving forces in the development of quantum technologies such as new quantum algorithms, error correction, and quantum circuit compilation \cite{jones2019quest, villalonga2019flexible,  xu2023herculeantaskclassicalsimulation}. \floris{Perhaps add why simulation is needed? Eg., because running quantum system is slow/expensive?}
% In the NISQ era, 
Other examples illustrating that simulation is a foundational tool in the NISQ era relate to
% In general, in the NISQ era, simulation serves as a foundational tool across key areas of quantum computing, including  quantum supremacy, quantum algorithms, 
quantum hardware, error correction, and the exploration of potential quantum applications \cite{xu2023herculeantaskclassicalsimulation}. 
% Various notions of simulation can be found in the literature \ref{}. Here, we focus on strong simulation in which, given  (family of) quantum circuits and a final measurement, one wants
% to compute the measured probabilities to a certain precision using
% a classical computer. 

The major practical bottleneck of simulation is  \emph{scalability} \cite{boixo2018characterizing, 8869942, xu2023herculeantaskclassicalsimulation, young2023simulatingquantumcomputationsclassical}. 
Typically, a quantum state is represented as a vector, e.g., the two-qubit state in Example~\ref{exmp:EPR pair}. Additionally, Fig.~\ref{fig:tensors_example}a shows the vector form of a three-qubit state, Greenberger-Horne-Zeilinger (GHZ) state.
% , represented as a state vector with amplitude of 8. 
When simulating a quantum state with $n$ qubits, the state vector's amplitude is $2^n$, which grows exponentially 
% as the number of qubits $n$ in the state increases, 
as $n$  increases, 
hitting hardware limitations. 
For instance, in an experiment demonstrating quantum supremacy \cite{boixo2018characterizing}, the wavefunction needs to be stored in random-access memory. 
% in single precision, requiring  $2^{n+3}$ bytes, 
%$2^{n+4}$ for the amplitude of the vector, and 4 for the double-precision complex numbers
% where $n$ is the number of qubits. 
It required 2.25 petabytes for 48 qubits, reaching the memory limits of today's supercomputers.  To overcome the memory restriction, existing simulation tools have explored approximation \cite{vidal2003efficient, medvidovic2021classical, jonsson2018neural}, data compression \cite{wu2019full}, 
%tensor network  
parallelization \cite{huang2021efficient},  and distributed computing \cite{smelyanskiy2016qhipsterquantumhighperformance}. 
 
An rather unexplored direction is to store the simulation data in a DBMS, i.e., out-of-core simulations over databases, which has the potential to facilitate faster simulation of more qubits and to lower the hardware requirements on memory size and computational power. 
However, storing and querying such quantum data in modern DBMS is not straightforward. A widely adopted data structure for simulating quantum computation is \emph{tensor networks}.
% To represent qubit states and quantum operations, 
% tensor networks are one of the most widely used data structures.
A \emph{tensor} is a multidimensional array, and the dimensions along which a tensor extends are its \emph{indices}. 
 % The total number of indices is referred to as {rank}
 For example, a vector is a one-dimensional tensor, and a matrix is a two-dimensional tensor.  
 A \emph{tensor network} is a collection of tensors represented as nodes, 
 % with their connections represented as edges  
with the shared indices contracted, which leads to a more compact and efficient representation \cite{biamonte2020lecturesquantumtensornetworks}. 
% Tensor networks are widely used in machine learning \cite{} and quantum computing \cite{}. 
Tensor contraction is the summation of shared indices between tensors.

% \floris{moved this away from above.. let's discuss  }
% \cite{pan2021simulatingsycamorequantumsupremacy}, such as
We next exemplify tensor networks by means of
 \emph{matrix product states (MPS)}  \cite{perez2007matrix, orus2014practical} for representing quantum states and \emph{matrix product operator (MPO)}  \cite{pirvu2010matrix} for quantum operations. 
 % , which are well-supported by open-source libraries  \cite{broughton2020tensorflow}. 
 
\begin{exmp} (\textbf{Quantum state in tensor network}) 
In Fig.~\ref{fig:tensors_example}b, the three-qubit GHZ state is presented in MPS, a factorized form of 3 tensors.   
The three qubits $A$, $B$, and $C$ are represented as nodes, and each node can be written as a tensor. To simplify the visualization, we illustrate the tensor $A$ of size $2*2*1$ as $A^0$ and $A^1$. It is possible to transform MPS to the state vector. For instance, the value of the last element in GHZ's vector, i.e., $D_{111}$ for state $\ket{111}$, can be computed by the tensor computation of $A^1B^1C^1$. 
\end{exmp}
\begin{exmp} (\textbf{Tensor contraction}) 
Fig.~\ref{fig:tensors_example}c depicts two two-dimensional tensors, matrices $A_{ik}$ and $B_{kj}$, which share the same index $k$. The  contraction  of $A_{ik}$ and $B_{kj}$ is the matrix multiplication operation $C_{ij}=\sum_{k}^{}A_{ik} B_{kj}$, which is often written as $A_{ik} B_{kj}$   in Einstein notion \cite{albert1916foundation}. 
% The simulation takes two inputs: the qubit state and a bitstring representing the measurements, and produces another bitstring as output. 
% The contraction of the tensor network gives the amplitude of the output bitstring. 
\end{exmp}

Quantum algorithms such as Grover's algorithm \cite{grover1996fast}, are implemented via quantum circuits. A quantum circuit include qubits, gates, and measurement. The gates  perform operations on qubits, and manipulate the qubit states. 
To represent quantum circuits,  in a tensor network a quantum state is represented as a node, and the gate operations can be seen as a series of tensor contractions. That is tensor contraction is the core operation when applying an MPO to an MPS or when measuring an MPS
\begin{exmp} (\textbf{Quantum operations in tensor network})  
Fig.~\ref{fig:tensors_example}d shows an example of a quantum operation, Hadamard gate, in MPO. 
The Hadamard gate H, represented as nodes $E$ and $F$, are performed on qubit states $A$ and $B$. The gate operation H is conducted by contracting $E$ and $A$,  $F$ and $B$, respectively, leading to new states of qubits $A'$ and $B'$. 
% The simulation takes two inputs: the qubit state and a bitstring representing the measurements, and produces another bitstring as output. 
% The contraction of the tensor network gives the amplitude of the output bitstring. 
\end{exmp}

\floris{It may be good for a db person to also get a feeling what the measurement is about and how it is implemented?}
As illustrated in above examples, the quantum-specific representations used in simulating quantum states and operations are different from the typical data representations and opertions supported in traditional database systems, which lay the unique challenges to out-of-core  simulations over databases.







% \floris{We may need a good argument why HPC people need db folks. I know it is memory, but we may never beat HPC in terms of speed.}

\subsection{Database to the rescue} 
\label{ssec:dbq}
 
The database community has a substantial body of work on tensor computation, 
especially with the recent synergies between databases and machine learning (ML) such as \emph{learning ML models over relational data} \cite{Khamis2020, boehm2023optimizing, Makrynioti2019survey, zhou2020database, 10107490}. These studies range from high-level representations to the runtime optimization of ML workflows. At the representation level, numerous studies represent data as tensors \cite{DBLP:journals/pvldb/KoutsoukosNKSAI21} and aim to integrate relational and tensor operations, with a commonly used algebraic notion being semi-rings \cite{DBLP:conf/sigmod/SchleichOC16, DBLP:conf/pods/Khamis0NOS18, DBLP:journals/pvldb/HuangSL023}. Meanwhile, system-building endeavors \cite{DBLP:conf/sigmod/GaoLPJ17, DBLP:conf/icde/LuoGGPJ17, DBLP:conf/sigmod/NikolicO18, DBLP:conf/sigmod/SchleichOK0N19, DBLP:conf/cidr/BoehmADGIKLPR20, DBLP:conf/osdi/NakandalaSYKCWI20, DBLP:journals/pvldb/HeNBSSPCCKI22, 10.1145/3514221.3526141} focus on performance efficiency and scalability, 
% LMFAO \cite{DBLP:conf/sigmod/SchleichOK0N19}
% F-IVM \cite{DBLP:conf/sigmod/NikolicO18}
% SystemDS \cite{DBLP:conf/cidr/BoehmADGIKLPR20}, 
% Hummingbird \cite{DBLP:conf/osdi/NakandalaSYKCWI20}, 
% TQP \cite{DBLP:journals/pvldb/HeNBSSPCCKI22}, 
% Raven \cite{10.1145/3514221.3526141} 
% SimSQL \cite{DBLP:conf/sigmod/GaoLPJ17, DBLP:conf/icde/LuoGGPJ17}
 employing optimization techniques during compilation (e.g., operator fusion \cite{boehm2018optimizing}) and runtime (e.g., parallelization \cite{DBLP:journals/pvldb/BoehmTRSTBV14}).

 



\subsubsection{Representation gaps} 

Initial efforts from the database community \cite{einsteinSQL2023, Trummer24} have started to tackle the out-of-core simulation challenge by mapping quantum states and gates to SQL queries. In \cite{einsteinSQL2023}, qubit states and gates are represented as tensor networks, with the sparse tensors in COO format\footnote{\url{https://docs.scipy.org/doc/scipy/reference/generated/scipy.sparse.coo_matrix.html}} and Einstein summation
 operation are mapped to SQL queries. The recent abstract \cite{Trummer24} provides the initial idea of supporting dense vectors by adding the SQL UNION ALL and CASE statements. Despite these early efforts that support basic quantum gates and states up to 10-qubit, the core challenges of representing general quantum states and operations in DBMS and scalability remain untouched. As mentioned above, from the database community intensive effort has been put into supporting tensor computation  
 % sparse tensors 
 at theoretical \cite{Khamis2020} and system aspect \cite{boehm2023optimizing}. Below, we initiate the discussion of filling the research gaps with a few open questions. 
 
\vspace{0.2cm}
\begin{myframe}[roundcorner=3pt]
Q1. \textit{How to design a \textbf{good} data abstraction to represent quantum states?} 
\end{myframe}
% \floris{I would start with the fact that on a logical level, quantum systems are commonly described by tensor networks, and as such, any db attempt to assist in quantum simulation must have the functionality  support the tensor computation. }
% \floris{I would use MPS etc as examples of how to represent tensor networks, i.e., physical level, that is, actual representation of tensor and their computation.}


With quantum data, i.e., quantum states, stored in DBMSs, we aim to support the simulation of quantum circuits. One of first questions is about finding the right data abstractions.
% at the logical level, which are independent from their physical implementation. We discuss the physical implementation later with Q3 and Q4. 
% data model,
% While we forsee the rich studies following this direction, 
We emphasize main requirements on the data abstraction: \emph{expressivity},  \emph{succinctness}, and \emph{equivalence}. 

\emph{Expressivity.}
First, the data abstraction should support representing possible quantum states, which also facilitates the gate and measurement operations of a quantum circuit. In Sec.~\ref{sec:classical-vs-quantum-data} we have explained key features of quantum data. Take entanglement for instance, in MPS, the level of entanglement is specified by a parameter called \emph{bond dimension}, which is the rank shared between two neighbouring tensors.  Bond dimension affects the dimensionality  of the tensors. We omit the complicated explanation of entanglement entropy and calculations here, but illustrate the impact of entanglement with the below example. 

\begin{example}
In the GHZ state, there are \emph{two} possible entangled components : $\ket{000}$ and $\ket{111}$. 
Thus, in Fig.~\ref{fig:tensors_example}b, the value of bond dimension is set as two, i.e., the shared rank value between A and B, B and C is two, illustrated in red color. This also affects the dimensions of tensors in MPS, which are marked in red in Fig.~\ref{fig:tensors_example}b. 
\end{example}


With qubit state as vectors (Fig.~\ref{fig:tensors_example}a) or tensors (Fig.~\ref{fig:tensors_example}b), straightforward choices of data abstraction from existing database literature include tensors \cite{DBLP:journals/pvldb/KoutsoukosNKSAI21}, tables \cite{einsteinSQL2023, Trummer24}, or their combination \cite{DBLP:conf/cidr/BoehmADGIKLPR20}. As explained in above example, to preserve the information in quantum states, we also need to consider their quantum-specific features. 

\emph{Succinctness.} In the context of databases, succinctness refers to the efficiency of data representation and storage. A succinct data abstraction minimizes the amount of space needed to store data while still allowing for efficient query processing. As discussed in Sec.~\ref{ssec:simu}, it is important to reduce the space representing a quantum state. 
This is affected with two parameters: number of qubits and the level of entanglement. For simulations based on state vector, the vector size grows exponentially as the number of qubits $n$ grows, i.e., $2^n$.
For MPS, it applies smaller matrices to preserve the information about a quantum state. The number of tensors is the same as the number of qubits. However, the dimensionality of the MPS tensors grow fast with the level of entanglement. It is interesting to explore with we can utilize existing studies of data abastraction from database community to find succinct abstractions for simulating quantum states.

\emph{Equivalence.} Often to choose the optimal data structure for simulation, it is important to check whether two given data structures are equivalent, e.g., whether the state vector in Fig.~\ref{fig:tensors_example}a and MPS in  Fig.~\ref{fig:tensors_example}b are equivalent (the answer is yes). It is an interesting problem how to define data abstraction that support such equivalence check. 
 
  
% \footnote{Tensor networks are widely used in quantum computing beyond simulation. Quantum circuits are a special class of tensor networks with unitary constraints. }




% \para{From formalism to implementation}
% \para{From formal properties to implementation}
% \textbf{From logical level to physical level.}  



% To tackle the data structure question from the implementation perspective,



\vspace{0.2cm}
\begin{myframe}[roundcorner=3pt]
Q2. \textit{Can we define a query language that serves as an abstraction layer \textbf{unifying} classical database operations and simulation programs?} 
\end{myframe}

 % \floris{Rihan: reference of complexity/tractability in db: \url{https://www.cs.rice.edu/~vardi/papers/stoc82.pdf}}

 The existing simulators for quantum computing are mostly implemented in Python \cite{nvidia_cuquantum_team_2022_6964823, vincent2022jet},  C++ \cite{qsim, vincent2022jet} or Julia \cite{luo2020yao}. There are also dedicated quantum programming languages and domain-specific compilation techniques, see the survey \cite{heim2020quantum}. 
% \floris{As described in \url{https://arxiv.org/pdf/2311.16505} Section 3.1, there are quantum programming languages, like \url{https://www.quantum-inspire.com/kbase/cqasm/} and perhaps others. One may need to differentiate from such attempts as well?}
The simulation workload, which includes preparing the initial state, gate, and measurement, requires intensive tensor computation. 
By connecting the simulators with data management systems, we have a pipeline of simulation workloads that are tensor computation and database operations.
To enable the optimization in the end-to-end pipeline


Besides gates and measurement, common quantum operations\footnote{For a more detailed explanation from the quantum computing perspective,  please refer to \cite{young2023simulatingquantumcomputationsclassical}.} also include addition and inner product between states, sampling measurement outcomes, and checking whether two states are equivalent   \cite{vinkhuijzen2024knowledge}.  \floris{Can we make it a bit more explicit what typical quantum operations are needed..}

To tackle the representation question from the logical level, we need to study formal properties such as \emph{expressive power} and \emph{tractability}. A key challenge in simulating quantum circuits is developing memory-efficient data structures that minimize memory usage while being computationally efficient for gate and measurement operations.
At the logical level, we need the data structure to be expressive enough to represent the general quantum states and gates and ideally tractable, i.e., the operation on this data structure finishes in polynomial time in the size of the input. New notions of equivalence check could be useful to verify whether two quantum states are exactly or approximately equivalent, analogous to checking equivalent conjunctive queries \cite{fagin2012local, fagin2008towards, cohen2007deciding}. \floris{Could this be undecidable, or are the results on this showing it is tractable? Perhaps ask Tim?}


Quantum circuits
Linear algebra, with tensor network such as




\floris{we may need to cite again, FAQ, LARA and other attempts for combining tensor and relational?}
We need a query language that can query matrices and tensors, possibly also relational tables. Such a query language would serve as an abstraction for both relational algebra and tensor computation operations. It is necessary to study the formal properties of this language, such as expressive power, complexity, etc. It is also interesting to explore whether we can obtain a generalization such as semi-ring. 
Moreover, many database tasks can
 be rephrased to problems on Boolean functions. By combining existing tractability results ofthe tensor network, can we derive the tractability of the main operation supported by this query language?
% matrix languages \cite{brijder2019matlang}.
% \floris{I don't think the matrix language developed there is human comprehensible. How complex can the queries be that quantum simulation people ask? And given building blocks, is there need for composing them? Who are the users? }



 
\subsubsection{Optimization gaps} 
Initial efforts \cite{einsteinSQL2023, Trummer24} still have not yet touched the challenges of system building and the massive opportunities of optimization. Although the computation of simulation tasks can be generalized as matrix multiplication, they differ significantly from the typical ML workflow studied in  \cite{DBLP:conf/sigmod/GaoLPJ17, DBLP:conf/icde/LuoGGPJ17, DBLP:conf/sigmod/NikolicO18, DBLP:conf/sigmod/SchleichOK0N19, DBLP:journals/pvldb/BoehmTRSTBV14, DBLP:conf/cidr/BoehmADGIKLPR20, DBLP:conf/osdi/NakandalaSYKCWI20, DBLP:journals/pvldb/HeNBSSPCCKI22, 10.1145/3514221.3526141}. Another open challenge is on the classical DBMS side. An interesting experiment result from \cite{einsteinSQL2023} is that it is questionable whether the query optimizers in existing RDBMS can effectively optimize SQL queries of simulation workload.  

\vspace{0.2cm}
\begin{myframe}[roundcorner=3pt]
Q3. \textit{Shall we push the simulation workload to existing DBMS?  Or design new tensor-native systems for simulating quantum states?}
\end{myframe}

By mapping the typical simulation workload to SQL queries, we can enjoy the efficiency and portability of modern database systems. We might need to design intermediate representations and seek more effective query optimization, even beyond existing query optimization techniques \cite{neumann2024closing}. On the other hand, a valuable experience of supporting ML workload \cite{DBLP:conf/cidr/BoehmADGIKLPR20} is that designing dedicated ML systems while adapting database techniques might bring more usability and efficiency. By adapting the representations of common quantum representations, such as tensor networks and existing simulation frameworks, the effort of building simulation tools using databases may be more easily adopted by quantum researchers. 

\vspace{0.2cm}
\begin{myframe}[roundcorner=3pt]
Q4. \textit{How to support efficient tensor computation of simulating quantum states and operations with database technologies?} 
\end{myframe}


% Tensor program 
Tensor computation optimization has been intensively studied by the database, compiler, and HPC communities \cite{schleich2023optimizing, boehm2023optimizing}. The system-building efforts include 
Taco \cite{kjolstad2017tensor}, 
 SystemML \cite{boehm2018optimizing}, TVM \cite{chen2018tvm}, Halide \cite{ragan2013halide}, TASO \cite{jia2019taso}, SystemDS \cite{DBLP:conf/cidr/BoehmADGIKLPR20}, and STOREL \cite{schleich2023optimizing}. 
With tensors as the representation, the runtime performance depends on the operations in the tensor program, the sparsity, and \emph{memory layouts}, i.e., how the tensors are stored in the memory, which can be row-major or column-major. The optimal memory layouts for runtime performance depend on the tensor computation operations (e.g., matrix multiplication), hardware (e.g., GPU module) \cite{jia2019taso}, and the sparsity of the data (dense or sparse). 
Recent work supports sparse matrix computation in relational databases \cite{DBLP:conf/pods/Khamis0NOS18}. There are also efforts to have a unified intermediate representation of relational algebra and tensor computation operations, and end-to-end pipeline optimization \cite{karanasos2extending, DBLP:journals/pvldb/HeNBSSPCCKI22}. The aforementioned works lay the foundation for supporting the tensor computation of simulating quantum circuits over DBMS. However, it is still an open area of how to tailor these techniques for quantum-specific characteristics: sparsity of tensors in the tensor network and compositional pipeline of quantum operations such as gates, measurement, and sampling. 

To identify the most suitable implementation of simulating quantum states and operations, the starting point is the large body of recent database studies exploring and supporting  ML applications over relational data \cite{Khamis2020, boehm2023optimizing, Makrynioti2019survey, zhou2020database, 10107490}. 
However, although both ML and quantum applications may share atomic building blocks of 
 matrices, tensors %\cite{DBLP:conf/cidr/BoehmADGIKLPR20}, 
 and tables, we need to tackle the quantum-specific challenges. 
For instance, the matrices representing quantum states, as shown in Fig.~\ref{fig:tensors_example}, their sparsity and size vary and may lead to different choices of data storage formats \cite{zeng2023empirical}, e.g.,  Parquet, ORC, HDF5, and Zarr.
% file format for large-scale data analytics
The compositional operations of quantum circuits may have different requirements for the data structure, such as searching the most efficient paths for tensor contraction.



% Q1: how to design a new data structure for centralized databases on quantum computers or distributed databases over the quantum internet, such that we can perform complicated computation?


% Q2: What is the optimum data structure that maximizes the quantum advantage and minimizes the quantum resources? 

% Q3: Can existing classical data structure help improve quantum data structures, e.g., simulation?

% \begin{figure}
% \centering
%  \includegraphics[width=\linewidth]{figures/arc.drawio.pdf}  
% %for discussion only, cannot use this picture
% \caption{Layered architecture}
% \label{fig:paradigms}
%  % \vspace{-0.4cm}
% \end{figure}


\subsection{More data management opportunities} 
\label{ssec:opp}

Beyond simulation for quantum computing,
quantum-related research is broad, e.g., error correction \cite{shor1995scheme, PhysRevLett.77.793, gottesman1997stabilizer}, %quantum mechanics \cite{}, quantum chemistry \cite{mcardle2020quantum}, 
quantum network \cite{wehner2018quantum, dahlberg2019link}. Next, we expand our discussion to uncover more opportunities spanning all three paradigms in Fig.~\ref{fig:paradigms}.

\vspace{0.2cm}
\begin{myframe}[roundcorner=3pt]
Q5. \textit{Can we develop novel data structures, formal methods, and systems for more quantum use cases?}  
\end{myframe}
 
\para{Quantum error correction \& Graph analytics  } 
As discussed in Sec.~\ref{ssec:nisq}, quantum processors in the NISQ era are inherently vulnerable to noise, which can significantly impact the reliability of computation results.  Quantum error correction is crucial for ensuring reliable quantum computation. This process consists of two main phases: coding and decoding. In the coding phase, the input quantum information is coded into a quantum error-correcting code such as the surface code \cite{fowler2012surface, bravyi2018correcting, fowler2009high}. During the decoding phase, errors are detected and corrected. Typically, errors are modeled as graphs. The error detection and correction algorithms, referred to as \emph{decoders}, are built upon graph theory such as graph matching \cite{fowler2015minimum} and shortest path problems. 
Exploring the recent effort of graph analytics \cite{10.14778/3611540.3611577, yan2005substructure, 10.1145/3448016.3452826} and graph databases \cite{tian2023world} such as Neo4j\footnote{\url{https://neo4j.com/}},  TigerGraph\footnote{\url{https://www.tigergraph.com/}}, might yield valuable insights to advance these error correction techniques. 
A unique challenge in graph data management for error correction is balancing accuracy and efficiency \cite{iolius2024decodingalgorithmssurfacecodes}. A more accurate decoder generally requires higher computational complexity and, therefore, operates more slowly. However, the fidelity of a qubit decays over time, demanding fast error detection and correction by the decoder. 

\rihan{ask Floris what this indicates}
\floris{\url{https://arxiv.org/abs/1901.03744} this is a paper based on FOCS 2019 paper on studying WMPC in the MPC model, the latter is being studied in db as well.}
\para{Quantum experiments \& Scientific data management} Quantum experiments, like any other scientific experiences, generate data and require data management. 
For instance, quantum mechanics experiments on supercomputers often apply HDF5 files to store data and XML files to store metadata \cite{de2011implementing}. 
Typical challenges include avoiding I/O bottleneck (efficient I/O parallelization) and handling the sheer volume and heterogeneity of data files.  The scientific data management challenge is also domain-dependent, e.g., experiment data from quantum chemistry \cite{rossi2014code} or condensed-matter physics.  These new data-related quantum challenges may require us to push forward the frontier of existing database topics such as metadata management \cite{bernstein2000panel, amano2014xml} and data formats \cite{zeng2023empirical}. It is also interesting to explore how to build novel data lakes \cite{nargesian2019data, hai2023data} or lakehouses \cite{armbrust2020delta, armbrust2021Lakehouse, jainanalyzing} for quantum applications.
% , i.e., \emph{quantum data lakes}.

% \para{Time series and stream processing}




\para{Quantum network \& Distributed databases} 
% \para{Distributed \& cloud-native databases} 
Quantum network holds the potential to offer advantages and capabilities beyond the power of classical internet systems, e.g., secure communication \cite{5438603} or distributed computing \cite{nickerson2014freely}. 
 Developing quantum network requires simulator tools such as NetSquid \cite{coopmans2021netsquid}, SimulaQron \cite{dahlberg2018simulaqron},  QuNetSim \cite{diadamo2021qunetsim}. 
It is interesting to explore whether these tools can be supported and enhanced by distributed databases \cite{ozsu1999principles} or cloud-native databases \cite{10574374}.







 

==> Vision_original.tex <==

\section{Our vision: data in the quantum era}
% 
 \floris{This section title has a large overlap with the previous section? Also, we are just sketching the landscape, is this our vision?  Perhaps: Data Management for Quantum Computing}
 \tim{agree on title. Or: 'Identifying data tasks in quantum computing' since effectively, we are guiding the classical data audience where they can contribute. Maybe it helps if somewhere in bold (maybe a subtitle) we say 'so there are many tasks, dealing with classical data only, where current data management research and practices can contribute'.}
\label{sec:roadmap}


% \todo[inline]{Todonotes can be turned off using usepackage[disable]\{todonotes\}}

%In this section, we describe various applications of quantum technologies, and then sketch our vision that data management theory and systems can significantly contribute to their realization.\footnote{Recall again that in this work, we give our vision on how database can support quantum technologies, not the opposite direction such as speeding up classical database operations using a quantum computer (e.g., query optimization~\cite{trummer2016multiple, schonberger2023SIGMOD}).}
%In this section, we consider possible ways in which data, both quantum and classical, occurs in the context of quantum technologies.
%We distinguish three paradigms, depicted in Figure~\ref{fig:paradigms}, depending on how close the paradigm's data is to a quantum state.
% In two of the three paradigms the data is classical (i.e. bits), whereas in the
% the third quantum data (i.e. qubits) is considered.
%For each paradigm, we explain how classical and quantum data interact and provide a few example applications.
In this section, we distinguish three different ways in which classical and quantum data co-occur.
% in the context of quantum technologies.
% , depending on how close the data is to a quantum state.
For each type of occurrence, depicted in Figure~\ref{fig:paradigms}, we explain the data's role and provide a few example applications.
\floris{I feel that we have to say why we do this? E.g., it is important for formalizing a vision/concrete research agenda?}
\floris{This part needs to be made stronger: I would repeat that we are looking that data management {\bf for} quantum computing and as part of our vision we here identify three different ways in which database technology can be leveraged, and at the same time, in doing so, clearly delineate focus points for  database researchers to contribute. After reading this section, a reviewer must have the feeling, yes, I never thought about applying database stuff in this way in relation to quantum, i.e., these authors are damn good visionaries...  }

% We emphasize in advance that these three paradigms have different purposes and co-exist simultaneously, i.e. one is \emph{not} a successive generation of the other.
%the extent in which the data that is central in the paradigm, represents a quantum state.
%much knowledge of the quantum state the database holds.
% remaining paradigm the database contains quantum bits.
% (see Section~\ref{sec:def} for an introduction to quantum bits).
% and sketch direction for data management research.
%objectives for data management development.
%, and can be developed independently.
% We envision three paradigms of designing and developing data management theory and systems for quantum computing, as depicted in Figure~\ref{fig:paradigms}.
%\tim{we need an introduction paragraph of three types on the high level, maybe also connect to NISQ and FTQC}

\floris{The more I think about this, the more confusing things get :-) Are we classifying types of data here, or more the use cases? It seems that the words "Simulative", "Interactive", "Quantum Pure"  better describe type II, I and III. }
\tim{good point! I would say use cases, or rather: tasks in quantum technology or its development which require handling of data.}

\subsubsection*{\textbf{I Classical Type: quantum technology's in/output stored and processed as classical data.}}
Here, we consider the following setting. A classical computer ships instructions to a quantum chip.
These instructions are classical data, and for example describes the quantum circuit that should be run.
The quantum chip runs its computation and after some time performs measurements onto one or more of its quantum bits.
The measurement outcomes, which are bits and hence classical data, are then returned to the classical computer, which in turn stores these in a classical database.
Thus, the quantum chip receives classical input (the instructions) and returns classical output (the measurement outcomes).
For some applications, this process is continued as a loop: new instructions are computed from the classical output, which are then fed back as input into the quantum computer.

The \emph{Classical Type} of data is the classical in- and output to the quantum chip.\looseness=-1
%
The kind of applications here fall into two categories: first, applications where the quantum computation is finished as soon as it returns.
%all qubits are measured is used once and the classical data is processed classically.
For example, two separated quantum computers can generate a secure, shared key (password) by encoding bits into qubits, followed by sending and measuring the qubits~\cite{bennett1984quantum,pirandola2019advances}.
This is followed by classical postprocessing on the bitstring (i.e. classical data) that the measurement returns~\cite{elkouss2011information}.
The resulting bitstring is a secret key which can later be used for secure communication.
%by both parties individually, which consists of sifting the data and a decoding step to reconcile from errors~\cite{information-reconciliation}.
%
In the other category, the quantum computation is stalled temporarily, and the quantum chip still holds quantum data on which the computation will continue later.
%the algorithm is a classical-quantum loop: the classical output is processed and then fed back into the quantum computer.
An example is the detection of errors during a quantum computation, where at fixed timesteps during the computation check measurements are performed~\cite{gottesman1997stabilizer,terhal2015quantum}, whose outcomes are then decoded to find out which error has most likely occurred~\cite{maurya2024managing,battistel2023real}.
% which has one node for each check measurement, and typically the number of check measurements is on the same order as the number of qubits.
%\tim{I moved a paragraph on q error correction from here to sec 4. If the paragraph is accepted \& processed into sec 4, then we could forward refer here to that part}


%
%Another example are variational quantum algorithms~\cite{}, a type of quantum machine learning method where solving a computationally-difficult optimization task is offloaded to a heuristic quantum circuit which is assumed to produce a good instance; from the quantum circuit's measurement outcomes an updated quantum circuit is then inferred.
%

\begin{figure}[t]
\centering
 \includegraphics[width=\linewidth]{figures/three-types.jpg}  
%for discussion only, cannot use this picture
\caption{Three ways in which data, either  classical (left, center) or quantum (right), occurs in quantum technology's context. See text for explanation.
	\textcolor{blue}{Tim: I now realize I have not mentioned Quantum Memory in the text. Is it clear nonetheless?}
	}
\label{fig:paradigms}
 % \vspace{-0.4cm}
\end{figure}

For both examples applications, the main challenge is that the data processing and I/O has to be fast for practical use.
For the second category the need for speed is particularly crucial, as the quality of the waiting quantum bits on the quantum chip decays (see Sec.~\ref{sec:def}) to the point that the quantum computation no longer functions correctly.
For error decoding for example, the required decoding should take at most several microseconds for some types of quantum hardware~\cite{battistel2023real}.
Existing data management tools and knowledge could potentially significantly contribute to scalable error decoding.
On the other hand, since in the two examples the bitstring is not huge (it is the message length\footnote{If one uses the information-theoretically secure one-time pad scheme for encrypting the message, the key has to be as long as the message in bits.} and the number of qubits\footnote{
For a promising and arguably most-researched type of quantum error-correction schemes~\cite{fowler2012surface}, the decoding is a graph task on a graph whose number of nodes is of the same order as the number of qubits, see also Sec.~\ref{ssec:opp}.}, respectively), it is a topic of research whether databases are the right tool for all tasks in this category.





%\floris{What graph problem? And what algorithm is used for it? How large are the instances? E.g., matching has a long history and has been studied by many algorithm folks, also in models of interest to db researchers like MPC \url{https://arxiv.org/pdf/1901.03744}. In summary, this needs to be made a bit more specific in order to be convincing.}


%Most applications require classical postprocessing of the data, and some consists of a loop where the result is fed back into the quantum circuit.
%Examples are:
%Quantum circuits, in both a computing, sensor, or network context, will produce a lot of data, which needs to be processed afterwards and for some applications fed back into the quantum circuit.
%Database theory and practice will contribute to designing systems that enable the required fast processing of the classical data, with objectives such as:
%Challenges that arise in these situations are for example:
%\begin{itemize}
%\item{
%An error decoding algorithm that strikes a balance between speed and performance~\cite{}, and scales to many qubits.
%The decoding task can be formalized as a graph problem~\cite{}, pointing in the direction of developing a graph-based database.
%
%Does the design also work for a modular quantum chip~\cite{modular q error correction}?
 %Although for many of the applications mentioned above, only common database operations such as `filter' are needed, the speed of these operations is crucial in case the quantum computation is running in tandem with the classical database, such as quantum error correction: in this scenario, the qubits' quality decays while the classical data operations are running.
%It might be that these specific applications require the design of new database structures and algorithms to meet the timing requirement.
%}
%\item{
%A scalable design for creating consensus between QKD parties.
%}
%\end{itemize}

%In the \emph{Classical Paradigm}, the data at best provides partial information of the quantum states held during the computation. In contrast, in the next paradigm the data is a full classical ``mirror'' of quantum data.

%The questions above deal with processing classical in- and output of quantum circuits, which at best provide partial information of the quantum states held during the computation.
%\todo[inline]{``The classical database remains ignorant about the fact that it interacts with a quantum computer? but in type II, we explicitly use the fact that we deal with quantum data, i.e. we explicitly take it into account in our design.'' Is that what we mean? If so, then verification (HKP protocol) should be in type II}
%\todo[inline]{explicit goal is to keep track of the quantum state}
%In contrast, in the next paradigm one requires a full classical `mirror' of quantum data.




\subsubsection*{\textbf{II Classical-Quantum Type: classical data represents quantum states and operations.}}
%\tim{could call `white-box paradigm'}
% \subsubsection*{\textbf{Second type (``CQ''): the data is a classical representation of (properties of) a quantum state.}}
The Classical-Quantum type of data represents a quantum state, for example a $2^n$-sized vector to represent an $n$-qubit state (see Sec.~\ref{sec:def}).
No quantum computer is involved, only a classical computer with a classical database containing the data.
The classical computer queries this data, or sends classical descriptions of (quantum) operations which change the quantum-state representation.
%The classical computer sends a description of a quantum operation to the database, which should then update its quantum-state representation as if the operation was performed on the quantum state.

The typical task here is \emph{classical simulation} of a real quantum device.


Simulation is useful for evaluating mitigation schemes for errors that occur in the device, predicting algorithm runtimes, etc. (see \cite{zulehner2018advanced, jones2019quest, zhou2020limits, villalonga2019flexible, azuma2021tools} and references therein).
%for identifying the most influential error types that should thus be targeted first when improving fabrication, etc.
%Since quantum devices are imperfect and introduce errors into the computations they run, 
%to predict the performance of these devices if they run useful quantum algorithms, 
%In this task, the classical computer holds an \emph{error model} of the real quantum device together with the desired quantum algorithm that it should perform, which consists of quantum operations such quantum gates and measurements but also of classical logic such as if-then-else-branches, etc.
When performing simulation, there are several types of instructions that the computer sends to the database~\cite{vinkhuijzen2024knowledge}.
Most importantly, the gates and measurements that together make up a quantum algorithm. 
For each gate, the database updates its quantum-state representation as if the gate was performed on the quantum state.
A measurement changes the data too, but also returns the measurement outcome as classical data to the classical computer, like a query.
Another instruction is for example the query how close the quantum state (representation) in the database is to some target quantum state.
%, e.g. in the metric called fidelity~\cite{}.
%the classical computer starts with an adjusted version of the quantum algorithm to-be-run according to an \emph{error model} of the real quantum device (such as by randomly inserting gates or perturbing potential measurement outcomes, see Sec.~\ref{sec:def}).


%The final instruction from the classical computer is the computation of some performance metric, such as how close the quantum state (representation) in the database is to some target quantum state.

%Another application of classical simulation is to understand where a quantum advantage cannot be obtained, by
%
%
%
%
%, where the goal is to predict the device's performance 
%
%of real devices when deployed into the wild
%
%
%
%Alternatively, the data could represent a sequence of quantum gates
%the computer could send descriptions of gates
%
%, and the goal of the database is to 
% equivalent but shorter sequence of gates.
%
%task here is to update the data 
%
%A typical example in this paradigm
%
%
%The quantum computer i
%
%a classical computer tracks a copy of a quantum state or (a sequence of) quantum gates.
%For example, for simulating a noisy quantum circuit, i.e. keeping track of the quantum state as quantum operations are applied to it.
%
%analysis and performance prediction of real devices when deployed into the wild
%
%subsequent design questions such as ...
%
%One application of simulation is to determine how individual noise parameter of the quantum chip influence the measurement outcomes at the end of the circuit~\cite{}.
%
%where no quantum advantage can be obtained

Alternatively, Classical-Quantum data does not represent a quantum state but instead a sequence of quantum gates~\cite{wetering2020zx,hubig2017generic}.
%An example application in this scenario is that the classical computer sends instructions which change the gates but not the function that the combined quantum-gate sequence computes, i.e. adjustments that leave the computed function invariant~\cite{zx}.
This is useful for design questions such as optimizing the number of quantum gates or gate depth~\cite{kissinger2020reducing,zulehner2018efficient} or compilation of textbook quantum circuits to only include the low-level operations that real quantum devices support~\cite{smith2020open}.
% and mapping qubits from one a textbook quantum circuit type onto another~\cite{}.


%\tim{I think can remove the following}
%Another example are Quantum-Internet applications where small quantum states are distributed between the network nodes and converted into larger, more complex ones~\cite{}. Keeping track of the exact state, and particularly its degree of noise, in a distributed manner is crucial for their operation.


%Classical-shadow methods, also referred to as `measure today and compute tomorrow', allow one to obtain a lot of information from the output state of a quantum circuit using only few runs~\cite{huang-kueng-preskill-protocol}.
%\tim{Let me dive deeper into the exact application here (error analysis?)}
%\tim{Maybe the required operation here is a simple, albeit very large, sum and therefore might not be too interesting for desinging a database system. Let me check}

The main challenge for dealing with Classical-Quantum data is that the representation of a quantum state (a vector) or quantum gate (a matrix) generally grows exponentially with the number of quantum bits.
Thus, the representation will not fit into main memory for already a modest number of quantum bits and needs to be distributed over secondary storage (out of core), a feat where databases can support.
%An alternative is to find incomplete yet efficient representations~\cite{stabilizer-formalism, matchgates, etc}.
Another application is efficient caching of expensive operations, for example when a quantum circuit is simulated several times with different error parameters.
Generally, we need the design of efficient data systems to distribute but also accommodate the efficient querying and manipulation of the quantum-state representations, whether this is a vector or a more compressed representation such as tensor networks~\cite{orus2019tensor} or other~\cite{bravyi2017improved,wetering2020zx,zulehner2018advanced, jozsa2008matchgates}.
We zoom in onto the tensor-network based simulation in Sec.~\ref{ssec:simu2}.


%Another is searching for relevant subsets of quantum circuits which allow for a concise classical representation~\cite{e.g. stabilizer formalism for Clifford circuit}.





%\begin{itemize}
%    \item ...
%\item{
%A scalable design for quantum-network nodes to keep track of a large distributed quantum state, and reconciliation of mismatches in it.
%\tim{I now wrote only high-level and want to make this more explicit}
%%if one performs the one-time pad with QKD, many bits will be produced, of which roughly half will be thrown away. Can we store these bits securely?
%}
%    \item ...
%\end{itemize}
 

\subsubsection*{\textbf{III Quantum Type: storage of quantum data.}}
% \subsubsection*{\textbf{Third type (``Q''): the data are quantum bits.}}
In the final case, we deal with genuine quantum data, i.e. qubits.
Here, the quantum hardware supports storing qubits for long enough to perform other tasks in the meantime.
%, so that, in principle, the amount of involved classical data is minimal. For example, quantum circuits are not limited in depth and there is no need to resort to methods to split up quantum computations by classical processing~\cite{circuit-cutting}.
%\todo{rewrite}
This enables for example a cloud quantum computer~\cite{broadbent2009universal} who rotates its resources among multiple clients, various types of quantum machine learning~\cite{cerezo2022challenges}, and Quantum Random Access Memory~\cite{giovannetti2008quantum}, where one queries data in superposition (although the latter's real-world advantage is debated, also see Sec.~\ref{sec:misconceptions}).
%, where the quantum server equally divides its time between the clients and, when hopping to the next clients without having finished a previous computation task, stores the latter's qubits in memory~\cite{}.
%These examples show that for large tasks, this paradigm is only reached in the FTQC era.
%For simple tasks, however, ...
%Another example in this paradigm is the availability of 

The main focus centered around quantum data is the development of quantum algorithms.
In addition, because storing quantum data will remain costly in various ways (number of qubits not unbounded, robust storage of quantum data requires large-scale quantum error correction, which is computationally intensive, etc.), another research topic is to efficiently allocate the available qubits.
This includes for example various scheduling and allocation tasks~\cite{chandra2022scheduling,fittipaldi2023linear,vanmeter2007system,skrzypczyk2021architecture,gauthier2023control,higgott2021subsystem} and efficient use of different quantum hardware types each of which have speed-decoherence trade-offs~\cite{de2021materials}.
 
%quantum algorithms are developed for acting on large amounts of quantum data (e.g. for quantum machine learning~\cite{cerezo2022challenges}) but also scheduling of quantum resources (e.g. quantum hardware types with different speed-decoherence trade-offs~\cite{}) is researched.
%\\

%\floris{This part is a bit far fetched from a db perspective perhaps. Why not selling this as if everything is quantum, quantum algorithms need to be developed for the entire dbms software stack? Or alternatively, how quantum can be used for classical data? Let's discuss.}
%Quantum databases are needed for the following applications.

%\begin{itemize}
%\item In the stack approach to quantum networks, lower levels of the stack produce quantum bits at random times and provide it to upper levels. The stream of quantum data should be handled, such that there are enough qubits available for the application, yet they are discarded after not too long (because of decoherence).
%\item Other types of memory management and scheduling tasks, such as scheduling~\cite{}, in distributed computation~\cite{}, quantum error correction~\cite{}, and other divide-and-conquer quantum algorithms~\cite{}
%%\item re-use of qubits (also when not really reset(?))
%\item Multi-client cloud quantum computing with fewer communication qubits than clients, leading to congestion ~\cite{tim-bling-quantum-computing-in-preparation}
%\item \tim{I want one more that does not have to do with q networks}
%\end{itemize}

%Tackling the scheduling and memory management issues for quantum data above would greatly benefit from a \emph{hierarchy of memory for quantum data}, in analogy to the classical hierarchy consisting of L1 cache memory, RAM, etc \cite{}.
%Such a design could include various types of quantum hardware whose different properties match the requirements of the different levels of the memory hierarchy (e.g. nitrogen-vacancy carbon spins have long coherence times but are also slow to operate on~\cite{}, in contrast to superconducting qubits~\cite{}).

For each way in which classical and quantum data interact, different data management methods might be needed, urging a distinction into data types such as the one above.
Finally, we remark that a single quantum application, or its development, can involve data of multiple types simultaneously.
For example, error correction methods act on quantum data (type III), but need decoding (I) and are assessed using simulation (II).
%quantum applications such as multi-client cloud computing (paradigm III) but also error correction methods (I) are assessed and optimized using simulation and compilation (II).
%(third paradigm) benefits from good compilers (developed in second paradigm) and the performance assessment of error correction schemes (a typical first-paradigm application) is also done using simulation~\cite{} (second paradigm).
%Also, the current roadmap to long-lived quantum memories (III) is through the use of error correction codes (I).
%, so the paradigms might co-exist even within a single application of quantum technology.
%performance assessment of quantum devices (a typical second-paradigm application) can also be done using a partial representation of the quantum state~\cite{classical-shadows}.


% guides the development of such methods.

%the above division into paradigms 
%
%guides the development of data management methods for different types of use cases.
%
%, the distinction into paradigms will aid developing data management for quantum technologies in the future.


%\tim{in type III: mention superposed queries: QRAM.}

%\todo{note: don't forget to note before that a quantum computation can output classical bits, but for state preparation, it outputs quantum bits}




 
\input{misconceptions}


==> auxiliaries.tex <==
\subsection{Quantum Data Quality}
\label{sec:quality}
\para{quantum noise}
A common way to interpret the differences of classical physics and quantum mechanics is that 
classical physics describes the macroscopic world such as Newton's laws of motion, while quantum mechanics describes the microscopic world at the scale of atoms and subatomic particles. Similarly, while we describe data quality by dimensions such as accuracy and timeliness on data instances or schemas, here we introduce \emph{fidelity} for qubit states and gates. 

\subsubsection{Noisy entanglement generation}
\para{Quantum decoherence}

noisy model: depolarizing noise

Werner states (worst case noise model)

Time-dependent, w, s, X(w, s), T(w, s)

non-locality as resources, but now as error-correction
CHSZ and GHZ as means to show error correction, quantum better than classical

\subsubsection{Fidelity as a DQ dimension}
We introduce metrics to quantitatively discuss the quality of the qubits.
Following existing quantum internet literature, \cite{avies2024tools, coopmans2021netsquid} We model time as discrete events. 

 
First, we introduce the ``perfect'' states for entanglement, \emph{Bell's state}, which is maximally entangled.
 
\begin{equation}
|\Phi^+\rangle = \frac{1}{\sqrt{2}} \left(|00\rangle + |11\rangle\right)
\end{equation}

However, we may not obtain such an ideal state because the generation of entanglement is noisy, denoted with a success probability $p$ in the range of [0, 1].
The heralded generation process contains a message to indicate whether the shared bipartite entangled state is successfully generated.
As a result of depolarizing noise,
the commonly used noisy model is \emph{Werner state} \cite{dur2005standard}, which is a worst-case noise model.
A Werner state $ \rho_W $ using the Bell state $ |\Phi^+\rangle $ can be written in the equation environment as follows:

\begin{equation}
\rho_W = p |\Phi^+\rangle \langle \Phi^+| + \frac{1-p}{4} I
\end{equation}

where$ I $ is a identity matrix. For two qubits, $ I $ is the 4x4 identity matrix.

\rihan{add fidelity from the book}
In quantum computing, fidelity is a classical notion of measuring the ``closeness'' of two states \cite{nielsen2010quantum}. The fidelity $ F $ between a mixed state $ \rho $ and a pure state $ |\psi\rangle $ is defined as 

\begin{equation}
F(\rho, |\psi\rangle) = \langle \psi | \rho | \psi \rangle
\end{equation}

The fidelity $ F $ between the Werner state $ \rho_W $ and the Bell state $ |\Phi^+\rangle $ is calculated as follows based on Equation 1-3:

\[
F(\rho_W, |\Phi^+\rangle) = \langle \Phi^+ | \rho_W | \Phi^+ \rangle = \langle \Phi^+ | \left( p |\Phi^+\rangle \langle \Phi^+| + \frac{1-p}{4} I \right) | \Phi^+ \rangle
\]
\[
F(\rho_W, |\Phi^+\rangle) = p + \frac{1-p}{4} = \frac{3p + 1}{4}
\]

Now, we insert the above result $F =  \frac{3p + 1}{4}$ ($p =  \frac{4F-1}{3}$) to Equation 1, and obtain the Werner state  $ \rho_W $ represented by Bell's state $ |\Phi^+\rangle $ and the fidelity $ F $. 
\begin{equation}
\rho_W = \frac{4F-1}{3} |\Phi^+\rangle \langle \Phi^+| + \frac{1-F}{3} I
\end{equation}
% where  $I$ is the identity matrix. For instance, in the case of two qubits, $I$ is the 4x4 identity matrix.

A quantum state in the quantum network changes over time due to the imperfect, noisy quantum memory where qubits are stored.
That is, fidelity is it is time-dependent, as the quality of the generated bipartite entangled state decays with time. Here, we give the time-dependent representation of fidelity \cite{inesta2023optimal}. 

\rihan{change citation}

\begin{equation}
F(t) = \frac{1}{4} + (F(t-\Delta t)-\frac{1}{4})e^{-\Delta t/\tau }
\end{equation}

where:
\begin{itemize}
  \item  $\Delta t$ is an arbitrary interval of time.
  \item  $\tau$ characterizes the exponential decay in fidelity; its value is hardware-specific, dependent on the physical realization of the qubits stored in quantum memories.
\end{itemize}
In practice, there is often a thread that needs to be set for minimal fidelity, as we want to generate good-quality entanglement.


\rihan{how to show time as discrete, non-overlapping slots; check the tool paper}
To build benchmarking tools for data management over quantum internet, it should be discrete-event based.

\subsection{Data cleaning using nonlocality theory} 
In Sec.~\ref{sec:challenge}, we mentioned superposition and entanglement. 



\para{Nonlocal games} To make it simple, we consider only two players, Alice and Bob. 
A two-player nonlocal game is a game that consists of two players and a referee. \
During the game, each player receives an input (like a question or a number) from the referee. Two players, Alice and Bob, however, cannot communicate once the game starts. 
The intriguing aspect of nonlocal games is that if Alice and Bob share an entangled quantum state, e.g., Bell's state from Example~\ref{exmp:EPR pair}, they sometimes can win the game with a higher probability than classical strategies. We give an example:

\begin{exmp} \textbf{Quantum machine learning}
\end{exmp}

\begin{exmp} \textbf{Blind quantum computation} protocols allow the client to delegate the quantum computation to a quantum server and to keep the client's input private. 
In the context of quantum data management, the client maintains a quantum database, and allows the server to have access to it through predefined operations.
Throughout the computation, the server is capable of performing the intended sequence of operations but learns no information. 
\end{exmp}
 

% \begin{acks}
 
% \end{acks}

%\clearpage
\subsection{Hybrid solution} 


\section{temp}
\subsection{Quantum data structure}
  



In databases, to retrieve data efficiently, we have data structures such as skipped list, B-tree, inverted index. The future research direction of quantum data management is in 2 aspects:

Q1: how to design a new data structure for centralized databases on quantum computers or distributed databases over the quantum internet, such that we can perform complicated computation?


Q2: What is the optimum data structure that maximizes the quantum advantage and minimizes the quantum resources? 

Q3: Can existing classical data structure help improve quantum data structures, e.g., simulation?


\para{possible data structures} \rihan{Shih-han to add}






\subsection{Unified query language }
\rihan{Usage: why we need this?}
So we need a unified query language that serves as the abstraction layer,  Moreover, 
such query language, maybe also provide possibilities with optimization of the operations  (the classical analogy is relational algebra) 
Quantum advantage is still part of ops using classical computing and quantum computing. In Fig.2, in the near term, we have their combination, even in the longer term. Still, classical DB will be there.






 

 
 


==> letter.tex <==
\pagestyle{empty}
\begin{strip}
\begin{minipage}{2\columnwidth}
\centering\Huge\bf Response to Reviewer Comments   
\end{minipage}
\end{strip}

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
% \floris{Copy paste letter here }
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
 

We thank the reviewers and meta-reviewer for their valuable feedback to help improve our paper. We appreciate the opportunity to revise our work and have carefully considered each reviewer's comments. In the following sections, we explain the revisions made based on the suggestions. Corresponding revisions in the main text are indicated in \revisionone{blue for Reviewer \#1}, \revisionthree{orange for Reviewer \#3}, and \revisionfour{green for Reviewer \#4}. 

In view of the many changes made, some parts of the paper have been moved to the appendix, hereby making space for the responses to reviewers.  For your convenience, the appendix can be found at the end of this response letter. The full technical report, consisting of the main paper and appendix, as well as the code for experiments are publicly available at: 
\begin{center}
  \url{https://github.com/infiniData-Lab/Quantum}.
\end{center}

Furthermore, to assist in the experiments, we have added an author to the paper (Tim Littau, PhD student at TU Delft). We requested and received permission from the PVLDB chairs to add this author.

\section*{Response to Meta reviewer}
\vspace{0.1cm}
\begin{myframe}[innerleftmargin = 5pt]
Please address as many of the specific revision items suggested by the reviewers as possible. Beyond these, our major concern is that a concrete novel analysis is missing, which could be theoretical (showing e.g. improvements in runtime complexity) or practical (based on at least preliminary experimental results). The vision is then founded upon this analysis.
 \end{myframe}
 \vspace{0.2cm}
\para{Response summary}
In response to the reviewers’ feedback, we have made the following changes:
\\1. \textbf{Novel analysis and  preliminary experimental results}: To address comments R1W1, we have added a novel candidate data representation based on our recent theoretical findings \cite{vinkhuijzen2024knowledge, 10412203}, now incorporated in Sec. 4.2 (Q4). Additionally, we expanded our discussion on error correction in Sec. 4.3.  Furthermore, we provide a preliminary investigation in the feasibility of RDBMS for simulation (Q1). In this context, for comments R3D1, and R3D3, we have provided a detailed analysis of space and time complexity of using a relational representation, now included in Appendix B1 and B2 of our online technical report \cite{techreport}, 
% \footnote{\href{https://github.com/infiniData-Lab/Quantum/blob/main/technical_report.pdf}}{github.com/infiniData-Lab/Quantum/technical\_report.pdf}}, 
which is also included at the end of this letter. 
Furthermore, we have conducted preliminary experiments, with key results added in Sec. 4.2. Detailed experimental settings and comprehensive results are provided in Appendices B3 and B4 of our online technical report,  but also included at the end of this letter. For the code we refer to the above mentioned github repository.
% The codes are publicly available at: \url{https://github.com/infiniData-Lab/Quantum}.

\smallskip
\noindent
2. \textbf{Modifications for all remaining comments}: We have revised relevant sections of the paper to address all the remaining reviewer comments. Please refer to the detailed responses below for more information on these changes.

Additionally, we would like to emphasize that our vision is also grounded in the convergence of our expertise across several domains: simulation and quantum data representation \cite{coopmans2021netsquid, vinkhuijzen2023limdd, vinkhuijzen2024knowledge}, formal verification \cite{hietala2020proving,hung2019quantitative,hietala2023verified,zhu2020principles}, quantum circuit optimization \cite{hietala2023verified}, computational complexity of near-term devices \cite{chia2024oracle,chia2022classical,cryptoeprint:2023/1911,aaronson2023certified}, optimizing linear algebra operations using database technologies \cite{10412203}, and database theory, particularly matrix query languages \cite{geerts2021matrix}.

 

% \floris{I think we should indeed make very clear why we all four are together on this paper, and how the vision in this paper originates from our own expertise, theoretical or practical. If possible, it would be fantastic if we could point to specific theoretical results (recent, by Tim and/or Shih-Han) that we believe can form a good basis for our simulation system. }

\section*{Response to Reviewer 1}
\vspace{0.1cm}
\begin{myframe}[innerleftmargin = 5pt]
W1. While the paper presents a comprehensive vision and highlights key challenges, it lacks in-depth technical solutions for the issues it raises. For example, specific algorithms or methodologies to tackle data representation or error correction in quantum systems are only briefly mentioned.
 \end{myframe}
 \vspace{0.2cm}
\para{Response}
Thank you for your feedback.  


For data representation, we build on our expertise and earlier work \cite{vinkhuijzen2024knowledge} and now propose a novel solution, which is added at the end of Q4 in Sec. 4.2. For your convenience, we have included %the newly added in-depth technical solutions
newly added solutions addressing Q4 below.

\smallskip
% \floris{This needs to be cleaned up and references need to be added. Tim?}
% \tim{thanks, will do.}
``\revisionone{A concrete idea for a novel data representation is to combine matrix product states (MPS) and the recently-proposed \emph{local-invertible map decision diagram} (LIMDD)~\cite{vinkhuijzen2023limdd}. LIMDD compresses a state vector by lumping together parts of the vector that are equivalent modulo simple quantum gates.
LIMDDs can simulate circuits that MPS cannot and vice versa~\cite{vinkhuijzen2024knowledge}.
One approach to combine these strengths in a single data structure is applying the lumping to the MPS matrices instead of quantum state vectors, by building upon existing work on equivalence characterizations of MPS~\cite{PhysRevLett.133.010602}.
%, hence combining the two into a single data representation resolves this incomparability, 
%are incomparable in the sense that each can, in polynomial space in the number of qubits, represent a family of quantum state vectors for which the other needs exponential space~\cite{vinkhuijzen2024knowledge}.
}''


\smallskip
For the quantum error correction part, we offer a more concrete technical analysis in Sec.4.3.   We include the revised paragraph here for your convenience.

\begin{table*} [t]
  \centering
  \caption{Recent data management works using quantum computers: an overview \cite{10597772}}
 % \vspace{-0.2cm}
\label{tbl:DB}
\resizebox{\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Reference}                                                                              & \textbf{DB problem}                 & \multicolumn{1}{c|}{\textbf{Subproblem}}                                                                           & \textbf{Formulation}  & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Intermediate \\ quantum algorithm\end{tabular}}}        & \textbf{Quantum computer}     \\ \hline
\cite{trummer2016multiple}                                                & \multirow{5}{*}{Query optimization} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Multiple query \\ optimization (MQO)\end{tabular}}} & \multirow{4}{*}{QUBO} & \multicolumn{1}{c|}{--}                                 & Annealing-based               \\ \cline{1-1} \cline{5-6} 
\cite{fankhauser2021multiple, fankhauser2023multiple}                     &                                     & \multicolumn{1}{c|}{}                                                                                              &                       & \multicolumn{1}{c|}{QAOA}                                 & Gate-based                    \\ \cline{1-1} \cline{3-3} \cline{5-6} 
\cite{SchonbergerSIGMOD22, schonberger2023SIGMOD, schonberger2023quantum} &                                     & \multicolumn{1}{c|}{\multirow{3}{*}{Join ordering (JO)}}                                                           &                       & \multicolumn{1}{c|}{QAOA}                               & Gate-based \& annealing-based \\ \cline{1-1} \cline{5-6} 
\cite{GroppeBiDEDE23}                                                     &                                     & \multicolumn{1}{c|}{}                                                                                              &                       & \multicolumn{1}{c|}{QAOA, VQE}                               & Gate-based \& annealing-based               \\ \cline{1-1} \cline{4-6} 
\cite{GroppeQMLBiDEDE23}                                                  &                                     & \multicolumn{1}{c|}{}                                                                                              & --                    & \multicolumn{1}{c|}{VQC} & Gate-based                    \\ \hline
\cite{ScherzingerVLDB2023demo}                                            & Data integration                    & \multicolumn{1}{c|}{Schema matching}                                                                               & QUBO                  & \multicolumn{1}{c|}{QAOA}                                 & Gate-based \& annealing-based \\ \hline
\cite{GroppeIDEAS20, OJCC,  groppe2021optimizing}                                                      & Transaction management              & Two-phase locking                                                                                                  & QUBO                  & --                                                      & Annealing-based               \\ \hline
\end{tabular}}
 % \vspace{-0.3cm}
\end{table*} 


\smallskip
``\para{Quantum error correction \& Graph analytics} 
% As discussed in Sec.~\ref{sec:classical-vs-quantum-data}, qubits in the NISQ era are inherently vulnerable to noise, which can significantly impact the reliability of computation results.
\revisionone{Quantum error correction (QEC) enables reliable execution of quantum computation on noisy quantum processors and is a crucial part of the roadmap to fault-tolerant quantum computation~\cite{terhal2015quantum}.
QEC process consists of two main aspects: coding and decoding.
The input quantum information as well as the operations to be performed are coded using a quantum error-correcting code such as the surface code \cite{fowler2012surface, bravyi2018correcting, fowler2009high}. Intermittently, decoding is applied: errors are detected and corrected.}
Decoders ~\cite{fowler2015minimum, iolius2024decodingalgorithmssurfacecodes, wu2022interpretationunionfinddecoderweighted} often leverage graph theory, solving tasks like a minimum-weight perfect matching (MWPM) problem on a graph where each node represents a check measurement. 
\revisionone{
% Despite the benefits of data management systems for speed and scalability, we remark that future research should show whether databases are indeed the right tool.
% For example, 
For MWPM, the number of nodes is of the same order as the number of qubits.
% which might be too small to observe benefits from the application of data management.
Many interesting research problems arise how to model such graphs and design the data formats. 
}
\revisionone{Moreover, QEC has to be performed at high speeds to avoid decaying quantum states over time (see Sec.~2), e.g. at most several microseconds for some types of quantum hardware for decoding~\cite{battistel2023real}.
The scalability to many qubits, and speed required for QEC might benefit from advanced data management tools and techniques \cite{10.14778/3611540.3611577, yan2005substructure, 10.1145/3448016.3452826, 
10.1145/2627692.2627694,
behnezhad2023exponentially}, offering a promising direction for further exploration.
% The required speed, combined with scalability to many qubits, could be delivered by existing data management tools and techniques .
}''

% \rihan{@Tim, if you have papers on error correction, please don't hesitate to cite them here}

% \floris{@All:We may want to additionally link back to expertise argument to meta-reviewer, if that works out.}

Furthermore, for challenge Q1 in Sec. 4.2, we provide complexity analysis and preliminary experiment results in Appendix B of the online technical report,  also included at the end of this letter. 

\vspace{0.2cm}
\begin{myframe}[innerleftmargin = 5pt]
W2. While the need for quantum-specific optimizations is highlighted, the discussion on how these might differ from existing classical structures and processes remains relatively shallow.
 \end{myframe}
 \vspace{0.2cm}
\para{Response}
Thank you for your comment. By ``classical structures and processes,'' we assume that you mean those related to the optimization in classical databases? In Sec 4.2.1, We added a paragraph highlighting the key differences between the quantum-specific optimizations and the existing database structures and optimization processes. More specifically, we have added (figure references correspond to references in main paper):
% \floris{Rihan, instead of pointing to 4.2.1, we could copy (part of) the added text here?} \rihan{clear, after shortening and polishing the texts, will put them here}

\smallskip
``\revisionone{Quantum-specific optimizations share some conceptual similarities with classical database optimization, yet they diverge significantly due to the unique characteristics of quantum data and operations. 
First, classical databases rely on relational or NoSQL data models (graph, document-based, etc.) with indexing mechanisms like B-trees or hash tables to facilitate efficient access and retrieval. In simulations, however, quantum states are represented as state vectors (Fig.~2a) or by using more advanced data structures such as tensor networks (Fig.~2b). 
% Instead, tensor networks break down entangled quantum states into manageable structures, reducing the computational complexity involved in simulating high-dimensional quantum states. Unlike classical databases, where indexing optimizes access to static datasets, quantum simulations must account for state entanglement, a uniquely quantum phenomenon, complicating data representation and requiring alternative structures for managing entangled data relationships.
Second, in classical databases, query optimization involves techniques like join ordering to identify the optimal ordering
of join operations between relations for an efficient query plan \cite{steinbrunn1997heuristic, DBLP:journals/pvldb/LeisGMBK015, trummer2017solving}. 
For tensor-based simulators,
a defining feature is the optimization of \emph{contraction order},  %finding the optimal contraction path, 
which determines the most efficient sequence to contract tensors representing quantum states \cite{young2023simulatingquantumcomputationsclassical, cuQuantum}.  
Contraction order optimization parallels the role of join order optimization in traditional databases but is more complex due to the exponential growth of quantum state dimensions and the unique features of quantum data, such as entanglement. 
Third, classical database systems rely heavily on cost estimation to predict and minimize resource use for query execution. Quantum computation simulators, however, lack cost estimation frameworks and instead use optimizations like parallelization, SIMD (Single-Instruction, Multiple-Data) processing, and matrix decomposition techniques (e.g., SVD) to improve performance \cite{young2023simulatingquantumcomputationsclassical}. Quantum-specific issues, such as quantum noise (Sec. 2), complicate simulation further. 
% Optimizations thus focus on resource efficiency and data fidelity under noise, requiring adaptive methods beyond the static cost estimates used in classical systems.
% In summary, while classical database optimization is grounded in structured data models, indexing, join planning, and cost estimation, quantum simulations require fundamentally different techniques due to the unique nature of quantum states, entanglement, and noise.  
These differences lead to the need for fundamentally new optimization frameworks to manage and simulate quantum computation effectively, beyond classical structures and processes.}'' 

%\tim{I see tensor networks as \textit{one} way of compressing the quantum-state vector. There are other techniques, which we cite (extended stabilizer formalism, decision diagrams, ...)}
% \tim{@Rihan: I made a mini-change to the text above in sentence ``In simulations, ...''}

\vspace{0.2cm}
\begin{myframe}[innerleftmargin = 5pt]
W3. Although the paper proposes classical preprocessing and postprocessing in quantum computing workflows, a deeper dive into how quantum algorithms can inherently manage data more efficiently compared to classical methods will benefit the paper.
 \end{myframe}
 \vspace{0.2cm}
\para{Response}
Thank you for your comments. 

% To address this, we have included a focused analysis in Sec. 3 on variational quantum algorithms (VQAs), one of the most representative quantum algorithms capable of inherently managing data more efficiently than classical methods. 

% \shih{A new paragraph added below to address the question of whether QC can speedup data management positively: }



\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/roadmap.drawio.pdf}
    \caption{Roadmap for solving data management problems on quantum computers \cite{10597772}.}
    \label{fig:roadmap}\Description[]{}
% \vspace{-0.4cm}
\end{figure}


Regarding the question of whether data management can become more efficient using quantum technology, we believe that the community may benefit from the development of quantum algorithm research over the years. 
In terms of research methodology, quantum speedups for data management problems can be tackled by i) reducing a data management problem to another computational task for which a quantum algorithm is known, and ii) using the algorithm as a subroutine to construct the algorithm for the original problem. 
For example, certain database problems,  such as query optimization,  can be reduced to quadratic unconstrained binary
optimization (QUBO) \cite{glover2022quantum}, for which Quantum Approximate Optimization Algorithm (QAOA) has the potential to speedup over classical computers \cite{farhi2014quantum}. 

In fact, in our recent tutorial \cite{10597772}, we summarized recent works addressing database problems using quantum algorithms (cf. Table.~\ref{tbl:DB}) and proposed a research roadmap (cf. Fig.~\ref{fig:roadmap}). We here simply show the table and figure and refer to the tutorial for more details.

Another example is searching over an unstructured database. The well-known Grover’s algorithm \cite{grover1996fast} provides a quadratic speedup for this task.  
% For Grover’s search to work, we must allow the queries to the database to be made in the Quantum Random Access Memory (QRAM) model \cite{phalak2023quantum}. 
% In this model, the algorithm is allowed to make queries on a superposition of entries, and gets back the fields, or whether the fields satisfy the conditions, in superposition in another register. 
For Grover’s search to work, it requires the Quantum Random Access Memory (QRAM) model \cite{phalak2023quantum}, which allows queries to be performed on a superposition of entries. 
% The results, 
% \floris{I do not understand this sentence: Field values are attribute values, right? Who is ``they'' in `` whether they satisfy the conditions''? And which conditions? Do you mean ``The results, i.e., entries satisfying the search conditions''?}
% such as field values or whether they satisfy the conditions, are returned in superposition within another quantum register.
% \floris{I do not understand ``why it is important to mention in superposition within another quantum register? What is the other quantum register? The one holding the answer? }
For search over graphs, quantum walk algorithms are known to yield polynomial speedups generally, and lead to exponential speedups for specific problems \cite{childs2003exponential}. 
To find duplicates in databases, we can exploit the  collision finding algorithm \cite{brassard1997quantum}. 



% \floris{I am not convinced at all by the VQA answer. I didn't know what they were before but after reading
% a bit, VQAs do not relate to the management of data.
% It is  a way to solve some cost-based optimalization where the costs function corresponds to a small enough quantum circuit so that it could (maybe) be implemented for real in the NISQ era machines. Since the calls to the cost function oracle is embedded in a classical setting,  it serves as a nice example of paradigm I, but doesn't really say anything about more efficient data management. The selling point VQAs is that are a potential way to show supremacy, computation-wise, but there also many doubts about that.
% }
% \shih{I agree with Floris that VQA does not seem to support the goal of using quantum computers to speedup data management. In fact I am not sure if I know a mathematical formulation (optimization?) for this point (perhaps you could name some so I will search for related papers). I think we can say quantum algorithms for some mathematical problems have speedups, and cite some papers if we want to, but VQA doesn't seem to work well with W3.}

% Below, we provide the refined texts for your reference:

% \tim{I think the reviewer misunderstood our paper. We can point this out (see Floris' very good text below), and I think then there is no need to say anything about VQAs as below.}
% \revisionone{For example, variational quantum algorithms (VQA) are considered as a promising proposal to obtain quantum advantage with a near-term device \cite{cerezo2021variational}. Similarly to classical neural networks, VQAs run a quantum circuit parameterized by a set of parameters, whose optimization is delegated to a classical computer receiving measurement outcomes from the quantum computer. 
% Moreover, using hybrid quantum-classical approaches, recent works have accelerated database operations such as query optimization (multiple query optimization \cite{trummer2016multiple, fankhauser2021multiple, fankhauser2023multiple}, join ordering \cite{SchonbergerSIGMOD22, schonberger2023SIGMOD, schonberger2023quantuma, GroppeBiDEDE23, GroppeQMLBiDEDE23}). These works map query optimization problems to quadratic unconstrained binary optimization (QUBO) formulations \cite{glover2018tutorial} for annealing-based or gate-based quantum systems, leveraging algorithms like quantum approximate optimization algorithm (QAOA) \cite{farhi2014quantum} and variational quantum circuit (VQC) algorithm \cite{chen2020variational}. For more in-depth explanations, please refer to our recent tutorial  \cite{10597772}.} 


% \floris{Below is a kind response that more efficient quantum is out of reach.}
% The reviewer raises an important question as to whether data management can become more efficient using quantum technology.  
In summary, we acknowledge the development of quantum algorithms for data management as an important research direction; and indeed, as highlighted  in Sec. 1 in the main paper, numerous surveys, tutorials, and vision papers \cite{ccalikyilmaz2023opportunities, 10597772, yuan2023quantum, yuan2024quantum, winker2023quantum} have already investigated how quantum technologies can accelerate classical data management tasks.
Unlike these studies, we would like to emphasize that 
our primary focus in this paper is on data management challenges \emph{for}  quantum computing. This is an equally important yet underexplored area, which lays the foundation for further deeper integration of data management and quantum computing.  
% Exploring the uncharted domain of data management challenges for quantum computing stands as our primary contribution.



% However, for large datasets, this data-loading process is not practically advantageous in the near term due to limitations in the number and lifetime of qubits, which restrict their capacity to store substantial data for extended periods. It remains unclear if quantum data-loading will ever surpass the efficiency of classical databases for directly acting on data, a view shared by quantum experts such as Scott Aaronson~\cite{aaronson2015read} and John Preskill~\cite{Preskill_2018}. Consequently,\tim{I think this is a great response, although I would replace `Consequently' by `Instead'} our focus is on data management \emph{for} quantum systems, rather than the reverse.
% It also explain why we only briefly touch upon the third paradigm (now called quantum-memory paradigm) in the paper.

% \tim{for reviewer1w3, could re-use the text from the third item in misconceptions.tex. But maybe it suffices to only reply to this in the rebuttal letter, not in the text itself}
% \floris{The response above is inspired by  what was written in misconception.tex: }

% \shih{If I understand what they say correctly, R1W3 asks how quantum computers can be used to speedup data management, and R4D1 asks to use classical computers to preprocess/postprocess so that quantum advantage won't disappear. To me they seem to be different questions. Here seems to be the place to respond to R4D1 (see above paragraph) but where should the answer to R1W3 be? }



\vspace{0.2cm}
\begin{myframe}[innerleftmargin = 5pt]
W4. Some terms such as "tensor networks" or "ZX calculus" are introduced without sufficient explanation. Including clear definitions or more detailed explanations of key terms, especially for readers outside the quantum computing domain.
 \end{myframe}
 \vspace{0.2cm}
\para{Response}
Thanks for pointing out this. In Sec. 4.2, we have added definitions and explanations for “tensor networks” and “ZX calculus” where they are introduced.  More specifically, we have added

\smallskip
``\revisionone{A tensor network consists of vertices representing tensors, and edges the indices. 
Free indices are depicted as legs, i.e., edges that only connect to one vertex in the graph. 
Connecting two vertices by joining a leg  corresponds to the contraction with the corresponding indices. 
% Quantum states can be represented as a set of tensors whose contraction yields the vector. 
% \shih{Can you please add here for R1W4?---done above, perhaps we only need to say why quantum states can be represented as a tensor network}
Fig.~2b shows an example of the tensor network representation of GHZ state.}''

Then, for the ZX-calculus we have added

\smallskip
``\revisionone{ZX-calculus is a graphical language for representing and reasoning about quantum computations, represented as tensor networks with specialized tensors called \emph{spiders}  \cite{van2020zx}. \ 
% In ZX-calculus, a computation or a state is represented as a graph, called a ZX-diagram, which is composed with a set of basic operations, called spiders. 
% Similarly to quantum circuits, ZX-calculus is a special class of tensor networks. 
% A spider denotes a tensor, and is depicted as a vertex with a few legs (see the paragraph above Q1), each corresponding to a two-dimensional index in the tensor.
% A wire connecting two spiders corresponds to a tensor contraction. 
Its graphical nature enables simplifications by locally merging connected vertices while preserving the original tensor, useful in various contexts including formal verification \cite{van2020zx,lehmann2022vyzx,de2020zx}. }''
\smallskip

% In the context of circuit optimization, one can further collect a set of rewrite rules, and use them to simplify the ZX-diagram translated from and to quantum circuits. 

% ``\revisionone{ZX-calculus is a graphical language for representing and reasoning about quantum computations \cite{van2020zx}.
% In ZX-calculus, a computation or a state is represented as a graph, called a ZX-diagram, which is composed with a set of basic operations, called spiders. 
% Similarly to quantum circuits, ZX-calculus is a special class of tensor networks. 
% A spider denotes a tensor, and is depicted as a vertex with a few legs (see the paragraph above Q1), each corresponding to a two-dimensional index in the tensor.
% A wire connecting two spiders corresponds to a tensor contraction. 
% Its graphical nature allows us to simplify the graph by locally merging multiple connected vertices into one when the simplified graph and the original denote the same tensor. 
% In the context of circuit optimization, one can further collect a set of rewrite rules, and use them to simplify the ZX-diagram translated from and to quantum circuits. 
% }''
% \floris{I like animals but introducing new concepts without needing them may raise more questions. This non quantum person just want to understand on a high level what it is. I uncommented an alternative in the appendix A6 in the main paper. }
% \shih{removed the unnecessary parts; now only say ZX-calculus is tensor network and what the language is used for.}

Moreover, to ensure clarity on all key terms, we reviewed the entire paper and extracted terms that may need further explanation. Due to the 6-page limit, we included comprehensive definitions, explanations, and examples in Appendices A and B1 of our online technical report, which is also included at the end of this letter. 

% \rihan{I moved all terms floris marked, to Appendix A of the main texts. @Shih-han, @Tim please add there}

% \floris{I walked over the paper and only found the following concepts not defined...perhaps there are more, but we can always say that we can add more to the reviewer. I used chatGPT to help me, so please check.}
% \begin{description}
%     \item[Tensor network] \cite{biamonte2020lecturesquantumtensornetworks}
%    is a graph where each node represents a tensor (multidimensional array), and where the edges represent contractions (summations) over shared indices. By mapping qubits and gates to tensors, general quantum circuits can be simulated using tensor networks.
%   \item[Einstein summation] \cite{albert1916foundation}
%   is a compact notation for summing over repeated indices in tensor operations. For example, for matrices $A$ and $B$, $A_{ik}B_{kj}$ represents the matrix multiplication $\sum_{k}A_{ik}B_{kj}$. 
%   \item[ZX-calculus] \cite{Coecke_2011}
%   is a graphical formalism used in quantum computing to represent and manipulate quantum circuits and states in a visual and intuitive way. It is based on tensor networks and provides a set of rules and diagrams for reasoning about quantum processes, especially those involving entanglement and measurement. Of particular interest are the ZX-calculus rewriting rules  that allow complex quantum processes to be simplified directly on the diagram without the need for lengthy algebraic computations. It is used, e.g., for circuit optimization, proving properties of quantum protocols, and verifying equivalence between circuits.
%   \item[Matrix product states] are a tensor network representation of quantum states, particularly useful for systems with limited entanglement. They express a large quantum state as a chain of smaller tensors, where each tensor represents a qubit and its local interactions with neighboring qubits. MPS can exactly represent any pure quantum state if the bond dimensions (the size of the internal tensors) are allowed to grow large enough. For states with low entanglement, this representation is compact and efficient. When the bond dimension is truncated (kept finite), MPS provides an approximation of the quantum state by discarding some of the higher entanglement contributions. This makes MPS lossy in the sense that it cannot fully capture states with high entanglement.
%   \item[LIM-decision diagrams]??
% \end{description}
% \floris{references should be added above.}


\begin{table*}[ht]
\centering
\begin{tabular}{|c|cc|c|}
\hline
% \rowcolor{gray!20} \textbf{Type}                             & \multicolumn{2}{c|}{\textbf{Exact representation}}                                             & \textbf{Approximate representation} \\ \hline
\rowcolor{gray!20} \textbf{State}  & \multicolumn{1}{c|}{\textbf{Order-$n$ tensor}}               & \textbf{Relational representation}                         & \textbf{MPS}                                 \\            
\rowcolor{gray!20}       $\ket{\psi}$           & \multicolumn{1}{c|}{\textbf{(Baseline I)}} & \textbf{(RDBMS solutions)}          & \textbf{(Baseline II)}       \\ \hline
\textbf{General state}                                             & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}             & $\mathcal{O}(n \cdot \text{nnz}(\ket{\psi}))$ & $\mathcal{O}(n \chi^2)$             \\ \hline
\textbf{$\text{W}_n$ State}                                             & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}             & $\mathcal{O}(n^2)$                       & $\mathcal{O}(n)$                    \\ \hline
\textbf{$\text{GHZ}_n$ State}                                           & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}             & $\mathcal{O}(n)$                         & $\mathcal{O}(n)$                    \\ \hline
\textbf{$\text{QFT}_n$}                                                 & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}             & $\mathcal{O}(n \cdot 2^n)$                     & $\mathcal{O}(n 
\chi^2)$             \\ \hline
\end{tabular}
\caption{Space complexity comparison of different representations of state $\ket{\psi}$.  Here, $n$ is the number of qubits, $nnz(\ket{\psi})$ denotes the number of non-zero probability amplitudes in the state \( \ket{\psi} \), and the MPS bond dimension $\chi$ is a fixed constant that one chooses oneself, potentially making the representation approximate.}
\label{tab:representation_l}
\end{table*}

% \begin{table*}[t]
% \centering
% \begin{tabular}{|l|ccc|c|}
% \hline
% \rowcolor{gray!20} \textbf{Type}           & \multicolumn{3}{c|}{\textbf{Exact}}                                                                                                  & \textbf{Approximation}  \\ \hline
% \rowcolor{gray!20}\textbf{Representation} & \multicolumn{1}{c|}{\textbf{State Vector}} & \multicolumn{1}{c|}{\textbf{Tensor Network}} & \textbf{RDBMS -- Tensor Network}         & \textbf{MPS}            \\ \hline
% \bfseries General                                             & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}    & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n \cdot \text{nnz($\ket{\psi})$})$ & $\mathcal{O}(n \chi^2)$ \\ \hline
% \bfseries W State                                             & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}    & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n^2)$                       & $\mathcal{O}(n)$        \\ \hline
% \bfseries GHZ State                                           & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}    & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n)$                         & $\mathcal{O}(n)$        \\ \hline
% \bfseries QFT                                                 & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}    & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n 2^n)$                     & $\mathcal{O}(n \chi^2)$ \\ \hline
% \end{tabular}
% \caption{Space complexity of different representations of a qubit state $\ket{psi}$, where $n$ is the number of qubits, $nnz(\bullet)$ is the number of non-zero values, and $\chi$ is the bond dimension when $\ket{\Psi}$ is represented in MPS.}
% \label{tbl:complexity}
% \end{table*}

% \begin{table*}[t]
% \centering
% \begin{tabular}{|l|cc|c|}
% \hline
% \rowcolor{gray!20} \textbf{Representation}           & \multicolumn{2}{c|}{\textbf{Order-N tensor (exact representation)}}                                                   & \textbf{MPS (approximation representation)}  \\ \hline
% \rowcolor{gray!20} \textbf{Approach} & \multicolumn{1}{c|}{\textbf{Baseline I in NumPy}} & \textbf{RDBMS}          & \textbf{Baseline II in NumPy}            \\ \hline
% \textbf{General}                           & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n \cdot \text{nnz($\ket{\psi})$})$ & $\mathcal{O}(n \chi^2)$ \\ \hline
% \textbf{W State}                           & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n^2)$                       & $\mathcal{O}(n)$        \\ \hline
% \textbf{GHZ State}                         & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n)$                         & $\mathcal{O}(n)$        \\ \hline
% \textbf{QFT}                               & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n 2^n)$                     & $\mathcal{O}(n \chi^2)$ \\ \hline
% \end{tabular}
% \caption{Space complexity of baseline and RDBMS implementation for simulating a quantum state $\ket{\psi}$, where $n$ is the number of qubits, $nnz(\bullet)$ is the number of non-zero values, and $\chi$ is the bond dimension when $\ket{\psi}$ is represented in MPS.}
% \label{tbl:complexity}
% \end{table*}

\begin{table*}[ht]
\centering
\begin{tabular}{|c|cc|c|}
\hline
% \rowcolor{gray!20} \textbf{Type}                             & \multicolumn{2}{c|}{\textbf{Exact representation}}                                             & \textbf{Approximate representation} \\ \hline
\rowcolor{gray!20} 
\textbf{State}  & \multicolumn{1}{c|}{\textbf{Order-$n$ tensor}}               & \textbf{Relational representation}                         & \textbf{MPS}                                 \\    
\rowcolor{gray!20}                              $\ket{\psi}$       & \multicolumn{1}{c|}{\textbf{(Baseline I)}} & \textbf{(RDBMS solutions)}          & \textbf{(Baseline II)}       \\ \hline
\textbf{W State}                                             & \multicolumn{1}{c|}{$\mathcal{O}(n \cdot 2^n)$}             &  $\mathcal{O}(n^2)$                      & $\mathcal{O}(n)$                    \\ \hline
\textbf{GHZ State}                                           & \multicolumn{1}{c|}{$\mathcal{O}(n \cdot 2^n)$}             &  $\mathcal{O}(n)$  & $\mathcal{O}(n)$                    \\ \hline
\textbf{QFT}                                                 & \multicolumn{1}{c|}{$\mathcal{O}(n^2 \cdot 2^n)$}             &  $\mathcal{O}(n^3 \cdot 2^n)$                     & $\mathcal{O}(n^3 \chi^3)$             \\ \hline
\end{tabular}
\caption{Time complexity comparison for the circuits from Fig.~\ref{fig:ghz-w-qft} for producing state $\ket{\psi}$.  Here, $n$ is the number of qubits, 
%$nnz(\ket{\psi})$ denotes the number of non-zero probability amplitudes in the state \( \ket{\psi} \), 
and the MPS bond dimension $\chi$ is a fixed constant that one chooses oneself, potentially making the representation approximate.
}
\label{tab:time_l}
\end{table*}
% \begin{table*}[t]
% \centering
% \begin{tabular}{|l|ccc|c|}
% \hline
% \rowcolor{gray!20} \textbf{Type}           & \multicolumn{3}{c|}{\textbf{Exact}}                                                                                                  & \textbf{Approximation}  \\ \hline
% \rowcolor{gray!20}\textbf{Representation} & \multicolumn{1}{c|}{\textbf{State Vector}} & \multicolumn{1}{c|}{\textbf{Tensor Network}} & \textbf{RDBMS -- Tensor Network}         & \textbf{MPS}            \\ \hline
% \bfseries General                                             & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}    & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n \cdot \text{nnz($\ket{\psi})$})$ & $\mathcal{O}(n \chi^2)$ \\ \hline
% \bfseries W State                                             & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}    & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n^2)$                       & $\mathcal{O}(n)$        \\ \hline
% \bfseries GHZ State                                           & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}    & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n)$                         & $\mathcal{O}(n)$        \\ \hline
% \bfseries QFT                                                 & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}    & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n 2^n)$                     & $\mathcal{O}(n \chi^2)$ \\ \hline
% \end{tabular}
% \caption{Space complexity of different representations of a qubit state $\ket{psi}$, where $n$ is the number of qubits, $nnz(\bullet)$ is the number of non-zero values, and $\chi$ is the bond dimension when $\ket{\Psi}$ is represented in MPS.}
% \label{tbl:complexity}
% \end{table*}

% \begin{table*}[t]
% \centering
% \begin{tabular}{|l|cc|c|}
% \hline
% \rowcolor{gray!20} \textbf{Representation}           & \multicolumn{2}{c|}{\textbf{Order-N tensor (exact representation)}}                                                   & \textbf{MPS (approximation representation)}  \\ \hline
% \rowcolor{gray!20} \textbf{Approach} & \multicolumn{1}{c|}{\textbf{Baseline I in NumPy}} & \textbf{RDBMS}          & \textbf{Baseline II in NumPy}            \\ \hline
% \textbf{General}                           & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n \cdot \text{nnz($\ket{\psi})$})$ & $\mathcal{O}(n \chi^2)$ \\ \hline
% \textbf{W State}                           & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n^2)$                       & $\mathcal{O}(n)$        \\ \hline
% \textbf{GHZ State}                         & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n)$                         & $\mathcal{O}(n)$        \\ \hline
% \textbf{QFT}                               & \multicolumn{1}{c|}{$\mathcal{O}(2^n)$}      & $\mathcal{O}(n 2^n)$                     & $\mathcal{O}(n \chi^2)$ \\ \hline
% \end{tabular}
% \caption{Space complexity of baseline and RDBMS implementation for simulating a quantum state $\ket{\psi}$, where $n$ is the number of qubits, $nnz(\bullet)$ is the number of non-zero values, and $\chi$ is the bond dimension when $\ket{\psi}$ is represented in MPS.}
% \label{tbl:complexity}
% \end{table*}



\vspace{0.2cm}
\begin{myframe}[innerleftmargin = 5pt]
O1. What role can machine learning techniques play in optimizing quantum data management systems, particularly in terms of simulating quantum systems, improving error correction, or enhancing the efficiency of quantum algorithms?
 \end{myframe}
 \vspace{0.2cm}
\para{Response}
Thank you for the valuable suggestion. An investigation into machine learning techniques \emph{for} quantum computing would indeed fit well in the NISQ era scope.
At the end of Sec. 4.3, we have added a paragraph dedicated to discussing the role of machine learning in optimizing quantum data management systems in the aspects of simulation, error correction, and enhancing the efficiency of quantum algorithms. 
For your convenience, the newly added text is as, as follows:

\smallskip
``\revisionone{\para{ML \& Quantum data management} i) \underline{Simulation}: as explained in Sec. 4.2.1, a key challenge in optimizing tensor network based simulation is to find optimal tensor contraction order.  A recent research direction is to apply machine learning (ML), specifically reinforcement learning (RL) and graph neural networks (GNN), to optimize tensor contraction order, addressing the computationally intensive nature of this challenge \cite{pmlr-v162-meirom22a, liu2023classical}. 
% By framing the problem as a Markov Decision Process, RL agents—often combined with Graph Neural Networks—are trained to sequentially choose tensor contraction paths that minimize overall computational costs, resulting in substantial performance improvements over traditional methods.
ii) \underline{Error correction}: decoding methods for quantum error correction (QEC), like MWPM, face scalability challenges in large quantum systems, where rapid error detection within strict time limits is essential  \cite{10.1145/3579371.3589037}. An interesting new direction is \emph{data-driven QEC}, which employs ML techniques to   quantum error correction, such as RL \cite{PhysRevLett.131.050601, nautrup2019optimizing, andreasson2019quantum}, multilayer perceptrons (MLP) \cite{chu2022qmlp}, convolutional neural networks \cite{Chamberland_2023}, and GNNs \cite{lange2023datadrivendecodingquantumerror}.
iii) \underline{Improving quantum algorithm efficiency:} Quantum algorithms are represented and implemented as quantum circuits, where efficiency can be improved by reducing costly gates like SWAP gate or by minimizing circuit depth and gate count.
ML methods, specifically RL \cite{fan2022optimizing, fösel2021quantumcircuitoptimizationdeep} and MLP \cite{paler2023machine},  have shown potential in optimizing circuit design to enhance the efficiency of quantum circuits on real devices.
}''
% \floris{Very nice answer - and quite interesting to work on perhaps :-)}

% \floris{We have to be careful here in that the reviewer is not asking for \emph{quantum machine learning}, but for machine learning for quantum. In some sense, addressing this fits our paper well since our focus is on classical stuff for quantum... }

% To the best of our knowledge, machine learning is not a common practice in simulation. One connection points is that tensor networks are one of mainstream representation for simulation, and tensor network are also widely used in machine learning. 
% \floris{the above is connection is rather weak.}\floris{I do not know well enough how ML is used for query optimization, but could we perhaps hint that ML can perhaps be used to assist in finding optimal contraction paths in tensor computations, similarly as how ML is used for query optimization?}



 \newpage


% \floris{Sure, but the reviewer asks ``classical'' ML angle here. I would say that this is a bit beyond the scope of this paper, unless there a concrete works we can cite?}
\vspace{2ex}
\section*{Response to Reviewer 3}

\vspace{0.2cm}
\begin{myframe}[innerleftmargin = 5pt]
D1: For the benefits of the proposed research directions, the authors always refer to related work in that area. Instead, the authors should provide an own novel analysis for at least one of the proposed open challenges. The analysis could be a theoretical one showing possible speedups, or better performance in another way, but at least additional preliminary experimental results would be perfect.
\vspace{1ex}
\\R1: Add an analysis for the benefits for at least one important open challenge (see D1).
 \end{myframe}
 \vspace{0.2cm}
\para{Response} 
Thank you for your insightful feedback. 

We carried out a preliminary investigation into our first research question (Q1) in Sec. 4.2: Should simulation workloads be pushed to existing DBMSs? We address your comment by: (i)~providing complexity analyses for Q1,  (ii)~reporting initial experimental studies for Q1. In addition, we also provide: (iii)~an analysis for other research directions. 



\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.8\linewidth} % Adjusted width to fit three subfigures in one row
        \centering
        \includegraphics[width=0.7\linewidth]{figures/experiments/2212/std_legend.png}
        \phantomsubcaption
        \label{fig:mem_legend_l}
     \end{subfigure}
    \setcounter{subfigure}{0}
    \begin{subfigure}[b]{0.32\linewidth} % Adjusted width to fit three subfigures in one row
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/mem_W.pdf}
        \caption{W state (\textbf{sparse} circuit)}
        \label{fig:wstate_mem_l}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\linewidth} % Adjusted width to fit three subfigures in one row
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/mem_GHZ.pdf}
        \caption{GHZ State (\textbf{sparse} circuit)}
        \label{fig:ghzstate_mem_l_two}
     \end{subfigure}
    \hfill
      \begin{subfigure}[b]{0.32\linewidth} % Adjusted width to fit three subfigures in one row
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/mem_QFT.pdf}
        \caption{QFT (\textbf{dense} circuit)}
        \label{fig:mem_qft_l}
     \end{subfigure}
         % \vspace{-3mm}
         \caption{Memory usage comparison of three RDBMS-based solutions (red) against general order-n tensor baseline (blue) and SotA MPS baseline (green). The x-axis shows increasing numbers of qubits, and the y-axis shows memory consumption (KB) in $\log_{10}$-scale. For sparse circuits (W and GHZ), RDBMS solutions demonstrate significantly lower memory usage than the order-n tensor baseline, with SQLite showing a slight advantage over the MPS baseline. For the dense circuit QFT, the memory usage of RDBMS solutions grows comparably to or exceeds the order-n tensor baseline, indicating the need for improvements in handling dense tensor computations.}
    \label{fig:mem_l}\Description[]{}
       % \vspace{-4mm}\Description[]{}
\end{figure*}
\begin{figure*}[ht]
   \centering
    \begin{subfigure}[b]{0.8\linewidth} % Adjusted width to fit three subfigures in one row
        \centering
        \includegraphics[width=0.8\linewidth]{figures/experiments/2212/std_legend.png}
        \phantomsubcaption
        \label{fig:mem_legend_l_two}
     \end{subfigure}
    \setcounter{subfigure}{0}
    \begin{subfigure}[b]{0.32\linewidth} % Adjusted width to fit three subfigures
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/time_W.pdf}
        \caption{W state (\textbf{sparse} circuit)}
        \label{fig:wstate_time_l}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\linewidth} % Adjusted width to fit three subfigures
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/time_GHZ.pdf}
        \caption{GHZ (\textbf{sparse} circuit)}
        \label{fig:ghz_time_l}
     \end{subfigure}
      \hfill
      \begin{subfigure}[b]{0.32\linewidth} % Adjusted width to fit three subfigures
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/time_QFT.pdf}
        \caption{QFT (\textbf{dense} circuit)}
        \label{fig:qft_time_l}
     \end{subfigure}
      % \vspace{-4mm}
    \caption{Runtime comparison of three RDBMS-based solutions (red) against general order-n tensor baseline (blue) and SotA MPS baseline (green). The y-axis is in log\(_{10}\) scale. The SQLite solution outperforms both baselines for sparse circuits. For the dense circuit QFT, NumPy-based baselines handle dense tensor computations more efficiently, indicating the need for further optimizations in RDBMS solutions.
  }
    \label{fig:exp_l}\Description[]{}
         % \vspace{-4mm}\Description[]{}
\end{figure*}

\smallskip
\textit{(i)~Complexity analyses.}\ 
% We have revisited the manuscript to better clarify the technical contributions and innovations underlying our vision paper, particularly in the context of quantum simulation. While the original scope was designed to outline key directions and opportunities in the field, we recognize the need to explicitly highlight our novel approaches and their significance.
To analyze the potential benefits of pushing simulation workload to RDBMS, we first explicitly define the relational representation for qubit states.\footnote{Similar to \cite{einsteinSQL2023}, our relational representation is based on encoding general tensor expressions in a relation schema comprising tensor indices and values. In addition, we extend this representation to incorporate quantum-specific semantics. i.e., treating an n-qubit state as an order-n tensor, and storing only non-zero probability amplitudes. With simple transformations (merging multiple column values into a single text field), our representation can be converted into the qubit state representation used in \cite{Trummer24}.}
The detailed definition and examples are provided in Appendix B1 of our online technical report, which is also included at the end of this letter. 


 


 %----------------------------------------------------------%
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.8\linewidth} % Adjusted width to fit three subfigures in one row
        \centering
        \includegraphics[width=0.4\linewidth]{figures/experiments/2212/query_legend.png}
        \phantomsubcaption
        \label{fig:query_mem_legend_l}
     \end{subfigure}
    \setcounter{subfigure}{0}
    \begin{subfigure}[b]{0.32\linewidth} % Adjusted width to fit three subfigures
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/query_mem_W.pdf}
        \caption{W state (\textbf{sparse} circuit)}
        \label{fig:wstate_memusg_l}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\linewidth} % Adjusted width to fit three subfigures
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/query_mem_GHZ.pdf}
        \caption{GHZ state (\textbf{sparse} circuit)}
        \label{fig:ghz_memusg_l}
     \end{subfigure}
     \hfill
      \begin{subfigure}[b]{0.32\linewidth} % Adjusted width to fit three subfigures
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/query_mem_QFT.pdf}
        \caption{QFT (\textbf{dense} circuit)}
        \label{fig:qft_memusg_l}
     \end{subfigure}
     % \vspace{-6mm}
    \caption{Memory usage comparison of SQL query generation \cite{einsteinSQL2023} vs. SQL query execution for SQLite. The y-axis in (a) and (b) uses $\log_{10}$-scale due to significant memory usage differences. Query generation incurs substantial memory overhead, in sharp contrast to query execution, especially for sparse circuits like W and GHZ states, where RDBMS solutions are more memory-efficient. This overhead results from tensor transformations and the translation of contraction paths into SQL join operations in \cite{einsteinSQL2023}.
  }
    \label{fig:mem_qcreate_l}\Description[]{}
    % \vspace{-6mm}
\end{figure*}
% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.46\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/experiments/0912/QueryCreation_memory_W.png}
%         \caption{W State (\textbf{sparse} circuit)}
%         \label{fig:memquery_wstate}
%      \end{subfigure}
%      \hfill
%       \begin{subfigure}[b]{0.46\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/experiments/0912/QueryCreation_memory_GHZ.png}
%         \caption{GHZ (\textbf{sparse} circuit)}
%         \label{fig:memquery_ghz}
%      \end{subfigure}
%     \caption{Memory comparison of SQL query creation vs. SQL query execution}%: $a)$  circuit GHZ $b)$ Dense circuit QFT}
%     \label{fig:querymem}
%     % \vspace{-6mm}
% \end{figure}
%----------------------------------------------------------%


% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.46\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/experiments/0512/W_circuit_memory_log_MPS_comparison.png}
%         \caption{W State (\textbf{sparse} circuit)}
%         \label{fig:wstate_mem_mps}
%      \end{subfigure}
%      \hfill
%       \begin{subfigure}[b]{0.46\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/experiments/0512/QFT_circuit_memory_log_MPS_comparison.png}
%         \caption{QFT (\textbf{dense} circuit)}
%         \label{fig:qft_mem_mps}
%      \end{subfigure}
%     \caption{Memory usage comparison of naive NumPy vs MPS solutions}%: $a)$  circuit GHZ $b)$ Dense circuit QFT}
%     \label{fig:npvsmps}
%     % \vspace{-6mm}
% \end{figure}


%================================================================%
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.8\linewidth} % Adjusted width to fit three subfigures in one row
        \centering
        \includegraphics[width=0.4\linewidth]{figures/experiments/2212/query_legend.png}
        \phantomsubcaption
        \label{fig:query_mem_legend_gen_l}
     \end{subfigure}
    \setcounter{subfigure}{0}
    \begin{subfigure}[b]{0.32\linewidth} % Adjusted width to fit three subfigures
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/query_time_W.pdf}
        \caption{W state (\textbf{sparse} circuit)}
        \label{fig:wstate_extime_l}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\linewidth} % Adjusted width to fit three subfigures
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/query_time_GHZ.pdf}
        \caption{GHZ state (\textbf{sparse} circuit)}
        \label{fig:ghz_extime_l}
     \end{subfigure}
     \hfill
      \begin{subfigure}[b]{0.32\linewidth} % Adjusted width to fit three subfigures
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/query_time_QFT.pdf}
        \caption{QFT (\textbf{dense} circuit)}
        \label{fig:qft_extime_l}
     \end{subfigure}
     \vspace{-2ex}
\caption{Comparison of SQL query generation time \cite{einsteinSQL2023} vs. SQL query execution time for SQLite.  Query generation requires more time than execution for sparse circuits like W and GHZ states, where RDBMS solutions are more efficient. Query generation incurs higher time costs due to the string construction proportional to the number of gates, along with overhead from tensor  transformations and contraction path translation into SQL join operations in \cite{einsteinSQL2023}.}
    \label{fig:time_qcreate_l}\Description[]{}
\end{figure*}




% %-------------------------------------------------------------------------------------%
% A critical component of the simulation engine is its application to \textbf{circuit optimization} as described in Section 4.2.1. Efficient simulation is essential for equivalence checking in circuit optimizations—a task that remains computationally challenging in the worst case \cite{janzing2005non}. Our approach builds on advances in combining circuit optimization with formal verification, including the use of proof assistants for correctness validation \cite{hietala2020proving, hietala2023verified}. This integration enables robust verification of practical optimizers, aligning with the broader goal of leveraging data management technology for simulating quantum circuits.
% %-------------------------------------------------------------------------------------%
As summarized in Table~\ref{tab:representation_l}  and \ref{tab:time_l}, our main focus is the space and time complexity analysis of the relational representation, comparing it with existing representations—an important analysis not conducted in previous works \cite{einsteinSQL2023, Trummer24}. The  preliminaries and detailed analysis are provided in Appendices A, B1 and B2.


% Tensor networks, a widely used family of general simulation methods, serve as the foundation for many existing simulators   \cite{biamonte2019lectures, young2023simulatingquantumcomputationsclassical}. At their core, an n-qubit state is represented as an order-n tensor, where quantum gate operations are performed through tensor contraction.  
Multi-dimensional tensors are the foundation of many successful simulation methods, including tensor networks. In such methods, quantum gate operations are performed through tensor contraction. 
We primarily compare the relational representation with an $n$-dimensional (also called order-$n$) tensor representation, where $n$ is the number of qubits. 
Our analysis in Table~\ref{tab:representation_l}  and \ref{tab:time_l} indicates that the relational representation shows advantages in circuits involving sparse tensor computations, such as W and GHZ state preparation circuits. However, it might be less effective for circuits dominated by dense tensor computations, such as quantum Fourier transform (QFT) circuits. 
%

Data representation is an active area of research in the quantum computing community. Matrix product state (MPS), a state-of-the-art compact representation optimized for low entanglement circuits, also leverages sparsity and is included in our comparisons here. 
 

\smallskip
\textit{(ii) Preliminary experiments.}\ 
We have conducted preliminary experiments on RDBMS solutions (implemented in SQLite, PostgreSQL, and DuckDB) to assess memory usage (Fig.~\ref{fig:mem_l} and Fig.~\ref{fig:memlimit_l}) and time efficiency (Fig.~\ref{fig:exp_l}). The detailed experimental setting (Appendix B3) and results (Appendix B4) are available in the online technical report \cite{techreport} and at the end of this letter. 
% The codes are also publicly available\footnote{\url{https://github.com/InfiniData-Lab/Quantum}}. 
% An interesting finding was that RDBMSs may not suit the simulation of all circuits but are effective for circuits with specific characteristics, e.g., sparse tensor computation. 


From the preliminary
experimental results, the main take-away is that relational representations are efficient and scalable for quantum circuits involving sparse tensor computations. They are competitive with, and may even outperform, state-of-the-art representations like MPS in specific scenarios. 

In addition, although not in our original submission, we identified a new research gap related to pushing simulation workload to RDBMSs.
Preliminary results revealed that the state-of-the-art SQL query generation method \cite{einsteinSQL2023} for quantum circuit simulation is inefficient, especially or sparse circuits like W and GHZ states. Compared to the query execution, the query generation has large memory overhead (see Fig.~\ref{fig:mem_qcreate_l}) and is relatively slow (see Fig.~\ref{fig:time_qcreate_l}) for sparse circuits, where the RDBMS solutions have the advantage. 
This finding suggests that future research on classical simulation over RDBMSs needs more efficient methods for generating SQL queries for input circuits, along with corresponding open-source tools.



% As an early study the relational representation we provided is straightforward, which could be improved, for dense circuits like QFT, our complexity analysis and preliminary results would be useful to further explore research Q4: What are good data representations -- possibly beyond tensors -- for supporting simulations?
% Moreover, in preliminary experiments we mainly used the default configuration with sophisticated system-level optimization. From the results we see much room for further optimization
% opportunities remain for even better performance. We are now confident with the research direction of Q3. Can we build an optimizer for simulations?



In light of your feedback, we have revised the manuscript to explicitly foreground these technical contributions and their implications, marked in orange in Sec. 4.2. Due to the six-page limit, we could only include a small portion of the results in the main text. 
For your convenience, the newly added text is highlighted below. We also include here the referenced Fig.~\ref{fig:mem_ghz_qft} as Fig~\ref{fig:mem_ghz_qft_l}.

``
\revisionthree{Moreover, our preliminary results in Fig.~\ref{fig:mem_ghz_qft} demonstrate that RDBMS-based simulations are efficient for quantum circuits involving sparse tensor computations. 
All experimental details, together with a space and time complexity analysis, can be found in Appendix B of  \cite{techreport}.\footnote{Codes are  available at \url{https://github.com/InfiniData-Lab/Quantum}}
% Our codes and technical report containing experimental setup and full results are available online\footnote{\url{https://github.com/InfiniData-Lab/Quantum}}. 
RDBMS-based solutions are competitive with, and may even outperform, state-of-the-art representations like MPS in specific scenarios. 
Interestingly, this advantage does not extend to dense circuits such as quantum fourier transform (QFT) circuits, highlighting the need for further optimizations to enhance RDBMS systems for simulation workloads.} ''
% \\\revisionfour{\para{Q1 summary} Pushing simulation workloads to DBMSs leverages their efficiency, showing promise for sparse circuits, yet challenges in optimization and scalability remain. 
% }
% \tim{sparsity is also captured by decision diagrams, although they suffer from numerical instability...should we mention these, and that our experiments make a numerically-stable step in the right direction, i.e. a step that also works in practice?}
% \tim{Should also mention theoretical proposal LIM-MPS here}

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.95\linewidth} % Adjusted width to fit three subfigures in one row
        \centering
        \includegraphics[width=0.8\linewidth]{figures/experiments/2212/std_legend.png}
        \phantomsubcaption
        \label{fig:mem_legend_three}
     \end{subfigure}
     \setcounter{subfigure}{0}
     \begin{subfigure}[b]{0.48\linewidth} % Adjusted width to fit three subfigures in one row
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/mem_GHZ.pdf}
        \caption{GHZ State (\textbf{sparse} circuit)}
        \label{fig:ghzstate_mem_l}
     \end{subfigure}
    \hfill
      \begin{subfigure}[b]{0.48\linewidth} % Adjusted width to fit three subfigures in one row
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/mem_QFT.pdf}
        \caption{QFT (\textbf{dense} circuit)}
        \label{fig:mem_qft_ l}
     \end{subfigure}
         \caption{\revisionthree{Memory usage comparison of three RDBMS-based solutions (red) against general order-n tensor baseline (blue) and SotA MPS baseline (green). The x-axis shows increasing numbers of qubits, and the y-axis shows memory consumption (KB) in $\log_{10}$-scale. For sparse circuit (GHZ), RDBMS solutions demonstrate significantly lower memory usage than the order-n tensor baseline, with SQLite showing a slight advantage over the MPS baseline. For the dense circuit QFT, the memory usage of RDBMS solutions grows comparably to or exceeds the order-n tensor baseline, indicating the need for improvements in handling dense tensor computations.}}
    \label{fig:mem_ghz_qft_l}\Description[]{}
\end{figure}


\smallskip
\textit{(iii)~ Analysis for other research directions.}\
To advance relational representations and RDBMS solutions, it is essential to consider also recent developments in the quantum computing community. Building on our expertise and earlier work \cite{vinkhuijzen2024knowledge}, we propose a novel solution detailed at the end of Q4 in Sec. 4.2. 
This includes integrating  matrix product states with the recently introduced local-invertible map decision diagram (LIMDD) \cite{vinkhuijzen2023limdd}. This hybrid representation addresses scalability challenges by enabling compact and efficient tensor operations, forming the basis of our envisioned simulation engine. The newly added text is provided below.

% Our analysis further emphasizes the pivotal role of linear algebra in quantum simulation, especially for tensor network-based simulations. A key challenge in this domain is the exponential growth of tensor size with the number of qubits, which necessitates efficient \textbf{tensor representation} strategies. Section 4.2.2 elaborates on our proposed integration of Matrix Product States with the recently introduced Local-Invertible Map Decision Diagram (LIMDD) \cite{vinkhuijzen2023limdd}. This hybrid representation addresses the scalability issue by enabling compact and efficient tensor operations, forming the foundation for our envisioned simulation engine. 
% % We also explore its potential for optimizing Clifford operations and handling long-distance correlations. 
%  For your convenience, we have included %the newly added in-depth technical solutions
% newly added solutions addressing Q4 below.

\smallskip
% \floris{This needs to be cleaned up and references need to be added. Tim?}
% \tim{thanks, will do.}
``\revisionone{A concrete idea for a novel data representation is to combine matrix product states (MPS) and the recently-proposed \emph{local-invertible map decision diagram} (LIMDD)~\cite{vinkhuijzen2023limdd}. LIMDD compresses a state vector by lumping together parts of the vector that are equivalent modulo simple quantum gates.
LIMDDs can simulate circuits that MPS cannot and vice versa~\cite{vinkhuijzen2024knowledge}.
One approach to combine these strengths in a single data structure is applying the lumping to the MPS matrices instead of quantum state vectors, by building upon existing work on equivalence characterizations of MPS~\cite{PhysRevLett.133.010602}.
%, hence combining the two into a single data representation resolves this incomparability, 
%are incomparable in the sense that each can, in polynomial space in the number of qubits, represent a family of quantum state vectors for which the other needs exponential space~\cite{vinkhuijzen2024knowledge}.
}''

We also added another analysis for quantum error correction, please refer to our response to Reviewer 1, W1 for more details.

% %-------------------------------------------------------------------------------------%
% To enhance usability, the design incorporates a \textbf{declarative interface} for quantum simulation. This interface draws on principles from query language development \cite{Brijder+2019,Geerts+2021,GeertsR22} and differential quantum programming \cite{}, offering a structured and accessible way for users to interact with the simulation engine. Finally, we \textbf{integrate} the different components in a system, resembling how ML workloads have been incorporated \cite{10412203}.
% %-------------------------------------------------------------------------------------%


% \cite{10412203}. She is also a leading researcher in quantum data management \cite{10597772}

% %-------------------------------------------------------------------------%
% We emphasize that the new analyses presented in this paper are grounded in the authors' recent work. Each contributor brings unique expertise that enriches our approach:
% \begin{itemize}
% \item Tim Coopmans advances efficient and tractable representations of quantum circuits, leveraging insights and tools from the formal verification field to deal with exponentially-large yet highly-structured state spaces.

% \item Rihan Hai specializes in building systems at the intersection of machine learning and database technologies, providing robust foundations for scalable and efficient quantum data management.

% \item Shih-Han Hung offers deep insights into quantum circuit optimization verification and differential quantum programming languages, bridging critical gaps between optimization techniques and their practical implementation.

% \item Floris Geerts contributes expertise in declarative query language design tailored for linear algebra and tensor computations, enabling intuitive and high-performance interaction with quantum simulation engines.
% \end{itemize}
% %-------------------------------------------------------------------------%



% Thank you for your valuable feedback. The scope of our paper was deliberately designed to leverage our collective expertise in outlining key directions and opportunities in the field. However, we acknowledge that we may not have sufficiently clarified why our combined expertise uniquely positions us to address the proposed challenges. In fact, it was our shared expertise and interests that inspired us to write this vision paper.

% We realize that our novel analysis and approach, particularly in the context of quantum simulation, may have been understated by being referenced through our prior work. In response to your feedback, we have revised the manuscript to explicitly highlight these and make our analysis more visible.

% \floris{Rihan rightly pointed out that we should focus on contributions, having expertise does not mean the vision is good....she is right. Let's discuss on Monday.}
% We would like to respond in detail, by explaining how the vision paper originated. This vision paper was initiated by Rihan Hai, an expert in building database systems tailored to data lakes and linear algebra/ML workloads \cite{10412203}. She is also a leading researcher in quantum data management \cite{10597772}. Linear algebra functionality plays a critical role in quantum simulation, particularly for simulations leveraging tensor networks. One significant distinction between quantum and ML workloads is the exponential growth in tensor size with the number of qubits, making efficient tensor representation essential for a quantum simulation engine.

% Tim Coopmans contributes his expertise in the efficient and tractable representation of quantum circuits, as well as formal verification methods. A key component of our vision, further elaborated in section 4.2.2, builds on his recent insights into combining Matrix Product States with the newly proposed Local-Invertible Map Decision Diagram (LIMDD) \cite{vinkhuijzen2023limdd}, enabling efficient tensor representations. We plan to structure our system around this novel representation, which we see as a significant innovation. \floris{@Tim: If any theoretical guarantees can be mentioned, or if knowledge compilation could play a role here, let's discuss further.}
% \tim{note to self: efficient Clifford operations on LIM-MPS. Long-distance correlations possible?}

% A second essential aspect of a quantum simulation engine is its application on circuits optimizers. \ 
% Here, Shih-Han Hung’s extensive work on the verification of quantum circuit optimizations is highly relevant \cite{hietala2020proving,hietala2023verified}. \ 
% Our vision on exploiting data management technology for simulating quantum circuits builds upon his insight into combining circuit optimization and formal verification. \ 
% To verify the absence of error in circuit optimization, one of the fundamental challenges is an efficient simulation of quantum circuits for equivalence checking. \ 
% While the task is known to lack an efficient classical algorithm in the worst case \cite{janzing2005non}, his previous works have enabled the use of proof assistants to prove the correctness of practical optimizers. \ 
% \floris{@Shih-Han: Do you see any concrete contributions we could highlight further in the optimization section?}
% \shih{how about the above?}

% Finally, to enhance usability, we aim to provide a declarative interface for the quantum simulation engine. This design leverages expertise in query language development (Floris Geerts) and differential quantum programming languages (Shih-Han Hung). \floris{We had previously included content on the declarative aspect, and we may consider adding this—potentially in the appendix—if we have a strong idea to expand upon.}

% \tim{We should say more about Floris if we decide to continue with this answer!}


% \floris{We may want to revise this response in accordance with how we respond to the main metareview question?}

% \floris{The comment seems to be centered on the fact that we ``always rely'' on related work, but do not make clear ``our own novel'' analysis for at least one of the challenges. Actually, this is a good point. Since this reviewer gave lowest score and this question is repeated in the metareview we need to answer it well}

% \floris{the original option was to show some new theoretical results or experimental evidence. This may be challenging.}

% \floris{Another option is to highlight our own expertise and results, and show that based on our combined expertise, we can address the challenges posed. As suggestion may be to push the data representationw work by Tim forward, and also perhaps the language design work by Shih-Han as a good interface formalization of quantum computation in our simulation engine? On the other hand, Rihan has experience in DB for ML and building systems...}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.32\linewidth} % Adjusted width to fit three subfigures in one row
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/memlimit_W.pdf}
        \caption{W state (\textbf{sparse} circuit)}
        \label{fig:memlimit_wstate_l}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\linewidth} % Adjusted width to fit three subfigures in one row
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/memlimit_GHZ.pdf}
        \caption{GHZ State (\textbf{sparse} circuit)}
        \label{fig:memlimit_ghz_l}
     \end{subfigure}
    \hfill
      \begin{subfigure}[b]{0.32\linewidth} % Adjusted width to fit three subfigures in one row
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pdf/memlimit_QFT.pdf}
        \caption{QFT (\textbf{dense} circuit)}
        \label{fig:memlimit_qft_l}
     \end{subfigure}
         \caption{Comparison of the simulated numbers of qubits for RDBMS solutions and the order-n baseline under a 2.0 GB memory limit. The y-axis is in log\(_{10}\)-scale for W and GHZ state preparation circuits. RDBMS-based approaches exhibit significant scalability in sparse circuits, simulating up to 16,850, 15,117, and 53,017 qubits on average for W states---yielding improvements of $991\times$, $889\times$, and $3,118\times$, respectively. For GHZ states, RDBMS solutions simulate $1.4 \cdot 10^7$, $3.1 \cdot 10^6$, and $4.0 \cdot 10^6$ qubits, achieving enhancements of $8.3 \cdot 10^5\times$, $1.8 \cdot 10^5\times$, and $2.4 \cdot 10^5\times$, respectively. For the dense circuit QFT, RDBMS solutions simulate up to 14 qubits, slightly below the 16 qubits supported by the order-\(n\) tensor baseline, indicating the need for further improvements. 
  }
    \label{fig:memlimit_l}\Description[]{}
\end{figure*}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7\linewidth]{figures/experiments/pdf/sparsity.pdf}
%     \caption{Sparsity ($s=1-\frac{\text{nnz}(\ket{\Psi})}{2^n}$) comparison for GHZ and W state preparation circuits and QFT circuit, where $\text{nnz}(\ket{\Psi})$ denotes the number of  non-zero probability amplitudes in the state $\ket{\Psi}$, $n$ is the number of qubits and $2^n$ is total number of possible states.}
%        \label{fig:sparsity_GW}
% \end{figure}



\vspace{0.2cm}
\begin{myframe}[innerleftmargin = 5pt]
D2: The authors do not cover a discusssion about the full benefits of applying database technologies for their proposed classical-quantum simulation system. The authors should taggle topics like consistency, recovery, transactions etc. as well. The authors may shorten the introduction to the absolute necessary parts for understanding the challenges for simulation.
\vspace{1ex}
\\ R2: Add a discussion about the benefits of utilizing database benefits like consistency, recovery, transactions etc. for simulation (see D2).
 \end{myframe}
 \vspace{0.2cm}
\para{Response} 
Thank you for your valuable suggestion. 
The primary reason why we did not discuss these aspects in more details is space limitations. But indeed, these database concepts may play an important role in quantum simulation, based on our discussions with quantum practitioners actively working on simulation. For large-scale quantum computation simulations, which run weeks and may occasionally crash, the reliability offered by mature database systems—such as recovery mechanisms—could be highly beneficial. 

% There is indeed a practical demand within the quantum community to leverage these database techniques. However, we found that some of these requirements may be more engineering-oriented than novel database research and are specific to the quantum domain. Therefore, we maintain that research interest should prioritize the foundational questions (Q1–Q4 in Sec. 4.2) we outlined, especially as the first steps of this new field of data management for quantum computing.
We recognize a practical demand within the quantum community for consistency, recovery, and transactions, and see the promising research potential in adapting these database technologies to simulation. However, foundational research questions (Q1–Q4 in Sec. 4.2) need to be addressed first, as they provide the underlying framework upon which these advanced database capabilities can be effectively built.  
For instance, we are still investigating which types of quantum circuits could benefit most from pushing simulation workloads to existing DBMSs, considering circuit characteristics such as qubit count, entanglement, circuit depth, circuit structure, and tensor sparsity (Q1). Moreover, our choice of data representations (Q4) could influence how we implement simulation workload using database technologies like RDBMSs (e.g., PostgreSQL, SQLite, DuckDB) or distributed frameworks using Spark, along with their corresponding consistency, recovery, and transaction mechanisms within CQSS.  We believe that pursuing these core questions (Q1-Q4) will establish a strong foundation for future studies in consistency, recovery, and transaction management for quantum data management.
% \tim{I think we could shorten the above paragraph is just saying `we have no space', followed by the response below} \rihan{We should be careful and not use no space, otherwise, reviewer 3, as an expert, may decide that we didn't do enough work here}



Now, in response to the reviewer, at the end of Sec. 4.2, we have added a new question (Q5) and present a discussion of the potential benefits of utilizing database features like consistency, recovery, and transactions in  simulations. We include the newly added text below.

``\revisionthree{By using database technology we aim for the simulation of complex circuits that require significant memory, without relying on HPC infrastructures or the operating system's memory management. By controlling what data is pushed to secondary storage during simulations, we can achieve more efficient I/O behavior. Additionally, transaction management and recovery become important—where a transaction could, for example, represent a sequence of quantum gates—ensuring that computations can restart from saved checkpoints while maintaining the correctness of partially saved results. Parallel evaluation strategies in quantum circuit simulations also highlight the need for effective transaction scheduling, leading to more reliable computational processes. 
Undoubtedly, many challenges remain in this context when considering quantum simulation. We prioritize Q1–Q4, however, as first steps. A more extensive discussion can be found in Appendix D in~\cite{techreport}.}''

In addition, also in response to the reviewer's comment D3, we summarize this also in a feature table, Table~\ref{tab:comparison_l}, in which we provide a more general overview of advantages of using database technology. Please refer to the response to D3/R3. 

% \floris{One thing that I would add is that when using HPC, many checkpointing features are in place that somehow do for computation, what transactions management does for transactions. So, perhaps the importance of transaction management is for cases when your don't have access to HPC or can't simply throw more memory to the problem?}




\vspace{0.2cm}
\begin{myframe}[innerleftmargin = 5pt]
D3: The authors should provide a better way to compare the benefits of utilizing databases besides the short overview in Section 4.2. One way would be to present a feature table. Some discussed benefits like applying the most efficient simulation are also promised by already existing simulators. Hence another way could be to show the limits of simulation without databases (e.g., by experiments).
\vspace{1ex}
\\R3:  Provide a direct comparison between simulation with and without databases (see D3).
 \end{myframe}
 \vspace{0.2cm}
\para{Response} 
 % \floris{I would say}
Thank you for the valuable suggestions. As mentioned in D1/R1, we have added preliminary experiments in Sec. 4.2, which shows the advantage with databases. Here we include another experiment to highlight the memory limitations of simulations without databases. Detailed experimental settings and   results are provided in Appendix B3 and B4 of the online technical report,
% \footnote{\href{https://github.com/infiniData-Lab/Quantum/blob/main/technical_report.pdf}{github.com/infiniData-Lab/Quantum/quantum\_vision.pdf}}
 which is also included at the end of this letter. Moreover, we included a feature table (Appendix D) comparing key features of simulations without and  with databases. 
% For your convenience, the preliminary results and the feature table are included here as well.
% \floris{How to address experiments? depends on Tim's experiments.}
% We also added Q5 at the end of Sec. 4.2. Below, we offer a more detailed explanation.

% \floris{Just note to ourselves: we may need to discuss the table together..}





\para{Preliminary experiments} 
We further explore the scalability advantages of RDBMS solutions compared to the general baseline using order-n tensor representation.
Fig.~\ref{fig:memlimit_l} compares the maximum number of qubits that can be simulated by each method under a 2.0 GB memory limit.
% To further investigate the impact of memory constraints, experiments with a $1.0$GB memory limit were conducted. 
For
the W state preparation circuit in Fig.~\ref{fig:memlimit_l}a, the RDBMS solutions
(SQLite, PostgreSQL, DuckDB) significantly outperform the order-n
tensor baseline. In the best case (DuckDB), supporting 53017
qubits compared to just 17 qubits for the baseline, which represents
a $3118\times$ improvement in scalability.  For GHZ state preparation circuit, SQLite
performs the best and simulates up to $1.4\cdot10^7$ qubits, compared to
17 for order-n tensor baseline, yielding an $8.3\cdot10^5 \times$ improvement.\footnote{The exact qubit counts are 14107345, 3079324, and 4000862 for SQLite, PostgreSQL, DuckDB, respectively.}  
These results demonstrate the substantial memory efficiency and scalability advantages of RDBMS solutions in handling sparse circuits. %when the number of qubits can be simuluated scales up.
For the dense circuit QFT, RDBMS solutions simulate up to 14 qubits, which is comparable to the 16 qubits supported by order-n tensor baseline with a reduction of $14\%$. 
\\ \emph{Take away: 
For circuits with sparse tensors (e.g., W and GHZ), RDBMS solutions enable simulations of much larger qubit counts compared to the order-n tensor baseline. Further optimization
opportunities remain to improve performance for dense circuits (e.g., QFT).}
 


\para{Feature table} We conducted extensive discussions with quantum theorists and simulation engineers to understand their practical needs and identified potentially useful database functions in Table~\ref{tab:comparison_l}. A key takeaway is that quantum simulation applications vary significantly regarding data sizes, computation complexity, and user demands. These variations suggest that different database technologies may be more effective for specific scenarios (exact or approximate simulations, applications such as quantum supremacy or quantum networks, etc.). Currently, database technologies remain underutilized in the simulation landscape, highlighting substantial opportunities for future research.

\begin{table*}[ht]
\centering
    \captionof{table}{\revisionthree{Comparison of simulation with and without databases technology}}
    \label{tab:comparison_l}
    % \vspace{-0.3cm}
    \revisionthree{
            \begin{tabular}{|p{3.5cm}|p{6cm}|p{6cm}|}
                \hline
                \rowcolor[gray]{0.9} % Light gray background for the header row
                \textbf{Feature} & \textbf{Without Databases} & \textbf{With Databases} \\
                \hline
                \textbf{Data Storage \& Retrieval} & 
                Data, such as simulation configurations, intermediate and final results, is stored in flat files (e.g., HDF5, JSON). Retrieval requires custom scripts and manual searches, which hinders data discovery, mining, and analysis. & 
                Data stored in structured, %tensor based, 
                indexable formats, enabling efficient organization and querying; optimized retrieval through indexing, caching, and execution plans, 
                %greatly enhancing data access performance 
                and facilitating the use of existing tools for data discovery, mining, and analysis.\\
             \hline
                \textbf{Query Languages} & 
                Accessing data relies on low-level programming, inefficient for querying data. & 
                High-level query languages like SQL, relational algebra, or tensor languages simplify data retrieval by providing intuitive, abstract constructs. These languages allow users to perform efficient and complex queries without requiring low-level programming, optimizing the interaction with large datasets.
                % High-level query languages (e.g., SQL, relational algebra, or Tensor Languages) simplify retrieval, enabling efficient queries.
                % for tensor structures, gate sequences, and circuit outputs. 
                \\
                \hline
                \textbf{Consistency, Recovery, and Transactions} & 
                Manual effort or customized scripts, error-prone. & 
                Well-developed theory and tools, reducing human effort and possible errors. \\
                \hline
                \textbf{Scalability} & 
                Limited by hardware capacity. & Potential benefits of databases for memory-efficient simulations; 
                extended by using secondary storage and out-of-core database technologies\\
                \hline
                % \textbf{Integration} & 
                % Custom solutions needed with manual overhead, limited commercial tool suppor. & 
                % Easy integration with existing DBMSs and their ecosystems. \\
                % \hline
            \end{tabular}
    }
\end{table*}

\emph{1. Data Storage \& Retrieval.} A common need in many simulation applications is managing data effectively, particularly optimizing retrieval and supporting advanced data analytics. Existing simulation tools often rely on flat files to store configurations and results, requiring custom scripts (e.g., Python) or manual searches for access. This approach is inefficient, time-consuming, and limits data discovery, mining, and analysis. For instance, in quantum network simulations, distributed experiments generate data from multiple users, but lack efficient tools for data discovery and analytics.
In contrast, databases store data in structured, indexable formats, enabling efficient organization and fast querying. Optimized retrieval through indexing, caching, and execution plans enhances performance. Another benefit is that database technologies are widely used and have a rich ecosystem of commercial and open-source tools (e.g., data analytics, discovery, integration, and cleaning platforms) that support advanced analysis and integration with existing simulation workflows.



\emph{2. Query Languages.} Current simulation tools typically access data relying on programming languages (e.g., Python) requiring customized optimizations for different quantum applications. This approach significantly increases development overhead and limits flexibility. In contrast, 
database systems leverage high-level query languages like SQL, relational algebra, or tensor-specific languages \cite{DBLP:journals/pvldb/KoutsoukosNKSAI21, geerts2021matrix, brijder2019matlang} to simplify data retrieval. These languages allow users to perform complex queries in a declarative and efficient manner, facilitating more effective querying and more sophisticated analyses with less human effort.

 
% \tim{can you please check below, where quantum networks are mentioned}

\emph{3. Consistency, Recovery, and Transactions.} Please refer to our response in D2/R2.   
% \tim{text seems to be copied directly from reviewer comments, including copying of references to their questions}
% we have elaborated on the potential of these database recovery technologies for simulation.
%Another interesting future research direction is to explore consistency and transactions in distributed quantum computing applications such as quantum networks. We take \emph{NetSquid}\footnote{\url{https://netsquid.org/}} for example. NetSquid is a widely used quantum network platform developed at TU Delft, which enables researchers to model, simulate, and analyze quantum communication protocols and hardware. NetSquid supports discrete-event simulation, where an event starts only after the previous event ends. Please refer to our previous work \cite{coopmans2021netsquid} for more technical details. A possible extension of NetSquid's discrete-event simulation is to allow concurrency simulation requests from multiple users. In this future direction, we foresee the potential to utilize and further develop database consistency and transaction management technologies. 
% \tim{I commented the original text out and wrote updated text for item 3 below}



 

\emph{4. Scalability.} We have discussed the bottleneck of scalability without databases in Sec.  4.1. With Fig.~\ref{fig:mem_l} and \ref{fig:memlimit_l}, we identified the potential benefits of database-based approaches for memory-efficient simulations. Another promising direction is out-of-core simulation using databases \cite{Trummer24}. 
When data sizes exceed memory limits, most main-memory databases switch to out-of-core strategies to complete queries. However, this often results in performance that is significantly slower than in-memory processing. %orders of magnitude slower
Recent advancements in out-of-core database techniques, such as sorting \cite{10184754}, aggregation \cite{10597735}, and joins, have redesigned operators to ensure performance degrades significantly less when the data size exceeds memory limits. It is an intriguing research direction to explore whether these techniques can enhance out-of-core simulation when simulation workloads are integrated with database systems.

 
\newpage
\section*{Response to Reviewer 4}


\vspace{0.2cm}
\begin{myframe}[innerleftmargin = 5pt]
D1. The efficient pre- and post-processing of classical data (input / results) for quantum computers / simulators is a relevant topic, since these processes must be executed as efficiently as possible. Otherwise, there is a high risk of losing any advantages that quantum computers potentially offer. In my view, this is the biggest motivation for the paper. 
 \end{myframe}
 \vspace{0.2cm}
\para{Response} 
%=====================================================%
% Efficient pre- and post-processing of classical data is indeed one of the biggest motivations of the vision. To emphasize this further, we provide an additional example showcasing this in Sec. 3, Paradigm II. For your convenience, the new additions are highlighted in green below.
%
%
% ``For some applications, this process is continued as a loop: 
% %  new instructions
% % are computed from the classical output, which are then fed back as
% % input into the quantum computer.
% the measurement output of the current iteration contributes to the next iteration's input instructions, and both are classical data. \revisionone{For example, variation quantum algorithms (VQA) are considered as a promising proposal to obtain quantum advantage with a near-term device \cite{cerezo2021variational}. Similarly to classical neural networks, VQAs run a quantum circuit parameterized by a set of parameters, whose optimization is delegated to a classical computer receiving measurement outcomes from the quantum computer.} \revisionfour{While the optimization of parameters appears to be an active research problem in data management (see e.g., \cite{zhang2021facilitating}), whether VQAs can exploit the state-of-the-art development in data management remains unexplored to the best of our knowledge. }''
%
% \floris{I would not add VQA to the place it is now in the main paper and instead state it as an example of the second applications at the end of (where quantum states are waiting for input...). For example:}
% \revisionfour{As another example, Variational Quantum Algorithms (VQAs) offer a promising path to quantum advantage on near-term devices~\cite{cerezo2021variational}, using parameterized circuits optimized by classical computers. Their performance relies heavily on efficient data management, encompassing tasks such as encoding data into quantum circuits, initializing parameters, and processing quantum measurement outcomes, all of which are crucial to realizing their full potential.}
% % \floris{the reviewer is not asking anything here, actually. I would respond as follows.We appreciate the reviewer’s interest in the pre- and post-processing of classical data described under Paradigm I in Section 3. As noted at the conclusion of that section: "In this paradigm, fast processing of classical data (including I/O with quantum devices) is often crucial for practical use, as quantum devices in the NISQ era are noisy, and the quality of quantum data degrades rapidly over time." We fully agree with the reviewer on the importance of this aspect. However, based on our expertise, we have chosen to place greater emphasis on quantum simulation, which we consider equally significant for motivating the discussion. We did not see any request for a concrete action on this comment by the reviewer, but of course are willing to implement any additional changes if needed}
% %=====================================================%
% \shih{add the following paragraph to explain that preprocessing of classical data for quantum use is a big challenge}
Thank you for your thoughtful comment. Indeed, we agree that quantum algorithms risk losing their computational advantage without proper preprocessing and postprocessing of classical data. Addressing the challenges of pre- and post-processing for quantum systems is a key motivation for this paper and central to the Joint Quantum-Classical Computing Paradigm (Paradigm II). 
To emphasize this critical aspect, we have expanded Sec. 3 by adding a specific application example at the end of Paradigm II.
 For your convenience, the newly added text is provided below. 

``\revisionfour{Third, efficient preprocessing is critical for quantum algorithms, which  requires  \emph{loading} or \emph{encoding} classical data into the quantum domain, typically by mapping classical bits onto quantum bits. This process often requires encoding classical data into a quantum circuit, either as part of the algorithm~\cite{suenderhauf2024blockencoding} or to output a quantum state with amplitudes representing the classical data~\cite{cortese2018loading}. This is a challenging problem.
For example, the Harrow–Hassidim–Lloyd (HHL) algorithm, a well-known quantum approach for solving a system of linear equations \cite{harrow2009quantum}, achieves exponential speedup over classical methods. However, this requires encoding the problem's vector elements into the amplitudes of the input quantum state. Developing a general and efficient method to encode arbitrary vectors into quantum states for the HHL algorithm is an open research question.}''

% Take the well-known  Harrow–Hassidim–Lloyd (HHL) algorithm as example, which is a quantum algorithm for solving a system of linear equations \cite{harrow2009quantum}. \ 
% To solve the problem exponentially faster than its classical counterparts, the vector elements in the problem must be encoded in the amplitudes of the input quantum state to the algorithm. \ 
% Currently, it is still an open question to find a general, effective process to encode any vector into a quantum state for HHL algorithm. 
% While it lacks a general quantum process to encode any vector into a quantum state, we note that in some applications, e.g., solving polynomial equations, the state preparation used by the algorithm is efficient (e.g., \cite{}). \ 
% % \shih{not sure yet where we are heading with adding examples of state preparation and quantum advantage}

 

\vspace{0.2cm}
\begin{myframe}[innerleftmargin = 5pt]
D2: For the vision, it makes sense to think about the most suitable database types. SQL is discussed in the discussion of question 1. This is a somewhat conservative view. It is interesting to consider whether NoSQL databases could also be used.
 \end{myframe}
 \vspace{0.2cm}
\para{Response}
%Thank you for this useful  suggestion. We have expanded the discussion in Sec. 4.2 to include NoSQL databases alongside RDBMSs. We now additionally emphasize the importance of NoSQL databases for scientific data management in quantum computing. To this aim, we added new discussion in Sec. 4.3, the paragraph of "Quantum Experiments \& Scientific Data Management. We next discuss these two points in turn.
% Related to NoSQL, it is indeed more comprehensive and less conservative to also explore the potential of NoSQL for quantum data management, as the reviewer suggestions. In view of the sheer variety in NoSQL databases, includin key-value stores, document stores, column-family databases, array databases, vector databases, and graph databases, due to space restrictions we focus on two examples: array databases and document stores. These support file types commonly used in quantum experiments.  For your convenience, the newly added text is highlighted below: 
% \revisionfour{A forward-thinking extension of Q1 is to choose most suitable databases for simulation. NoSQL databases such as  TileDB, an array database, offers native storage and retrieval of multi-dimensional arrays (tensors), leveraging parallel processing, distributed computing, and easy integration with machine learning and data science tools. The downside is that much effort is needed to support in-database computation and query optimization for simulation workload and expand the ecosystem to match the versatility of RDBMSs, highlighting critical areas for future research in adapting array databases for simulation workloads.}
% In `Quantum error correction \& Graph analytics,'' we examined the role of graph databases. The suitability of a specific database type will depend on the nature of the quantum experiment, and it is unlikely that one system will fit all needs—making this a promising area for further exploration. For your convenience, the newly added text is highlighted below:
Thank you for this valuable suggestion. Indeed  the discussion of question 1 can be expanded to include NoSQL databases alongside RDBMSs.  In addition, we see the potential of NoSQL databases in scientific data management for quantum computing and quantum error correction.
Regarding NoSQL databases, we agree that exploring their potential for quantum data management is more comprehensive and less restrictive, as suggested by the reviewer. Given the variety of NoSQL databases --- such as key-value stores, document stores, column-family databases, array databases, vector databases, and graph databases --- we focus on three examples: array databases, document stores and graph databases. 
% These examples align with file types commonly used in quantum experiments. 
Due to the six-page space restrictions, we have  added the new discussion in Appendix C of  online technical report, 
% \footnote{\href{https://github.com/infiniData-Lab/Quantum/blob/main/technical_report.pdf}{github.com/infiniData-Lab/Quantum/quantum\_vision.pdf}}, 
which is also included at the end of this letter.  For your convenience, the newly added text is provided below: 

\smallskip
``\revisionfour{ \para{NoSQL databases \& Quantum data management}
NoSQL databases offer a promising solution for analyzing simulations and quantum experiments, since NoSQL databases are well-suited for managing unstructured data with their scalability and flexible schemas. 
% They include key-value stores, document stores, column-family databases, and graph databases, with the capability of horizontal scaling, making them ideal for large datasets. Their flexible schemas adapt easily as models evolve, which is crucial for dynamic simulations. 
A forward-thinking extension of Q1 in Sec. 4.2 is to choose the most suitable databases for simulation. For example, TileDB \cite{TileDB}, an array database, offers native storage and retrieval of multi-dimensional arrays (tensors), leveraging parallel processing, distributed computing, and easy integration with machine learning and data science tools. Adapting array databases to simulation workloads remains an open challenge, requiring significant effort to enable in-database computation and query optimization for simulation workload and expand the their ecosystem to match the versatility of RDBMSs.}

\revisionfour{
% TileDB  supports HDF5 files, enabling the conversion of HDF5 datasets into TileDB arrays for more efficient queries and storage.
Moreover, JSON is a widely used file type for circuit descriptions and simulation configurations in quantum frameworks, e.g., Qiskit \cite{Qiskit}, Cirq \cite{cirq}, or Braket \cite{Braket}.  
Document stores like MongoDB \cite{MongoDB} can efficiently manage JSON and could play a critical role in this context. 
% For instance, key-value stores such as Redis and DynamoDB are optimized for low-latency access for simulation workloads requiring low latency.   These features make NoSQL a strong choice for large-scale, low-latency, flexible simulation data management. 
Furthermore, for error correction techniques discussed in Sec. 4.3, exploring the recent effort of graph analytics \cite{10.14778/3611540.3611577, yan2005substructure, 10.1145/3448016.3452826, 
10.1145/2627692.2627694,
behnezhad2023exponentially} and graph databases \cite{tian2023world} such as Neo4j\footnote{\url{https://neo4j.com/}},  TigerGraph\footnote{\url{https://www.tigergraph.com/}}, might yield valuable insights.} 

\revisionfour{In summary, relational and NoSQL databases, each offer unique advantages, but no single database system is likely to meet the diverse requirements of all quantum applications; the optimal choice will depend on the specific needs of each quantum application.}''
%-----------------------------------------------------------------%
% Additionally, in the section "Quantum Error Correction \& Graph Analytics," we have discussed the role of graph databases. The suitability of specific database types depends on the nature of the quantum experiment, and it is unlikely that a single system will address all requirements—making this a highly promising area for further exploration. For your convenience, the paragraph and newly added text are added below.

% \smallskip
% ``\para{Quantum experiments \& Scientific data management} Quantum experiments, like any other scientific experiments, generate data and require data management. 
% For instance, quantum mechanics experiments on supercomputers often apply HDF5 files to store data \cite{de2011implementing}.
% % and XML files for metadata \cite{de2011implementing}.
% \revisionfour{
% NoSQL databases, present a promising direction for managing unstructured data, offering scalability and flexible schemas that are well-suited for analyzing quantum experiments and simulations. 
% % They include key-value stores, document stores, column-family databases, and graph databases, with the capability of horizontal scaling, making them ideal for large datasets. Their flexible schemas adapt easily as models evolve, which is crucial for dynamic simulations. 
% For instance, TileDB \cite{TileDB}  is an array database that supports HDF5 files, enabling the conversion of HDF5 datasets into TileDB arrays for more efficient queries and storage.
% JSON is a widely used file type for circuit descriptions and simulation configurations in quantum frameworks, e.g., Qiskit \cite{Qiskit}, Cirq \cite{cirq}, or Braket \cite{Braket}.  
% Document stores like MongoDB \cite{MongoDB} can efficiently manage JSON. 
% % For instance, key-value stores such as Redis and DynamoDB are optimized for low-latency access for simulation workloads requiring low latency.   These features make NoSQL a strong choice for large-scale, low-latency, flexible simulation data management. 
% Continuing the discussing in Sec. ~\ref{ssec:dbq2},
% relational and NoSQL databases, each offer unique advantages, but no single database system is likely to meet the diverse requirements of all quantum applications; the optimal choice will depend on the specific needs of each quantum use case.''
% % Typical challenges include avoiding I/O bottleneck (efficient I/O parallelization) and handling the sheer volume and heterogeneity of data files.  The scientific data management challenge is also domain-dependent, such as those arising from quantum chemistry %\cite{rossi2014code} 
% % or condensed matter physics experiments.  These challenges may require us to push forward the frontier of existing database topics such as metadata management \cite{bernstein2000panel, amano2014xml} and data formats \cite{zeng2023empirical}. 
% }
%------------------------------------------------------------------------------------%

% \floris{The response is good but it is perhaps a bit too much? The reviewers asks noSQL in connection with Question 1? So, if you know of any noSQL system that could be used in the context of Q1, I would simply add it to the text of Q1. If space permits, the use of noSQL for other questions/challenges may be added as well of course? } \rihan{good point, we can drop or greatly shorten the second part in Sec. 4.3}


\vspace{0.4cm}
\begin{myframe}[innerleftmargin = 5pt]
W1: The answers to the questions posed in Section 4: The reader must deduce these from the explanations. A final, recognizable answer/statement based on 1-2 sentences would be helpful for each question.
\\D3: A clear, concise concluding statement for each question in Section  4 is missing.
 \end{myframe}
 \vspace{0.2cm}
\para{Response} Thank you for the nice suggestion. We have added a final summary for each question in Sec. 4.2.
% \floris{good, let's not forget to do this ;-)}
% \rihan{After all texts finished. I will redo this item. Let's have a final check together}
% \floris{Let's do this at the end indeed.}

\noindent\revisionfour{\para{Q1 summary} Pushing simulation workloads to DBMSs leverages their efficiency, showing promise for sparse circuits, yet challenges in optimization and scalability remain. 
}

\noindent\revisionfour{\para{Q2 summary} Tensor-based database technologies are promising for boosting simulation performance, with efficiency depending on tensor operations, sparsity, memory layouts, and hardware.} 

\noindent\revisionfour{\para{Q3 summary} Quantum-specific optimizations require a dedicated simulation optimizer to handle tensor contraction, state sparsity, noise levels, and task-specific strategies, while also eliminating redundant computations through equivalence checking.}

\noindent\revisionfour{\para{Q4 summary} Effective data representations for quantum simulations require a balance of expressiveness, closure, and succinctness.}
 
\noindent\revisionfour{\para{Q5 summary} Database technology holds promise for consistency, transaction management,  and recovery, paving the way for more reliable and scalable simulations.}


\vspace{0.4cm}
\begin{myframe}[innerleftmargin = 5pt]
W2: The contribution to database research in Section 3 is very vague and general. Various aspects (like efficient data storing systems, efficient queries) mentioned are not only unconditionally quantum computing-specific and affect many possible application areas.
\end{myframe}
 \vspace{0.2cm}
\para{Response} 
%\floris{Just a a proposal reply if nothing concrete comes, so this is plan B reply.}
%Section 3 aims to structure the research landscape by exploring how classical and quantum computing can interact and identifying specific quantum problems where database technology could play a crucial role. Each of the three paradigms outlined necessitates distinct approaches—ranging from general-purpose database solutions (applicable beyond the quantum context) to methods specifically tailored for quantum applications. For instance, quantum simulation, discussed in detail in Section 4, highlights potential contributions from database research.
%
%In other places, we are indeed more generic. However, even in cases where quantum-specific database techniques may initially seem unnecessary, complexities or specialized requirements could emerge, underscoring the need for tailored solutions. 
%With this paper, one of our goals is to raise awareness of the valuable contributions database research can make in this evolving field. At the same time, for quantum simulation, detailed database contributions are provided, as this fits best with our expertise.
%\tim{What about the following alternative?}
% \tim{Floris' reply (commented out above) was good, but I tried to polish it a bit more as in below}
Thank you for the comment. 
Regarding generality: The contribution of Section  3 is a distinction into paradigms where data management research can benefit quantum computing, based on the nature and role of the data involved.
The goal of Section 3 is to guide and focus future data management research, and for that reason is high-level and plays a dual role as an introduction to various quantum use cases for data management researchers.
It is only in Section  4, where we provide concrete research questions and goals for one of the paradigms from Section  3. For instance, we discuss \emph{quantum-specific} optimization challenges in Section  4.2.1.
Because of this choice of generality in Section 3, especially in contrast with the concrete questions in Section 4, we understand that our current writing of Section  3 could be interpreted as unspecific.

To clarify the intention of Section 3, we added the following text to the end of the first paragraph in Section  3:

\smallskip
``\revisionfour{
Our goal is to introduce data management researchers to quantum use cases, and by making a distinction based on the nature and role of data within cases. We primarily present future data management research for quantum computing. In Sec. 4, we provide concrete research directions in  these paradigms.}''
% The goal of this section is to introduce data management researchers to quantum use cases, and by making a distinction based on the nature and role that data in it plays, focus future data management research for quantum computing. In Sec. 4, we will provide concrete research directions in one of the paradigms we distinguished.}''
\smallskip

% Regarding application beyond quantum computing: the aim of this section is to sketch the vision which research, tools and practices from data management can benefit quantum technology development. These are indeed not limited to quantum computing only, but since the focus of this vision paper is on applications in quantum computing, the section only involves the latter.
% To clarify this, we added the word `existing' at the start of the section, in
% ``Each paradigm not only guides the exploration of quantum research topics leveraging \revisionfour{existing} database technologies but also paves the way for new opportunities in database systems, ultimately driving the development of quantum computing.''

Additionally, in Sec.  3, specifically in \emph{II Joint Quantum-Classical Computing paradigm}, we added the link to Section  4 to provide concrete examples and practical details. This connection aims to clarify the quantum computing-specific aspects discussed in Section  3, making them more tangible and easier to understand. More specifically, the revised text reads as follows.

\smallskip
``Database research can enhance this process by developing efficient systems for managing, storing, and querying the classical data involved in preprocessing, postprocessing, and iterative feedback loops between classical computers and quantum devices, ensuring seamless integration and optimization of data workflows. \revisionfour{For instance, the development of quantum error correction—a critical area in quantum computing—can benefit significantly from efficient graph data analytics techniques, as further discussed in Sec.~4.3.}''

%\tim{could also make remark that quantum computing is applied linear algebra, so not strange that the methods for quantum computing can be applied elsewhere too. But I'm not sure if that makes the reply stronger.}



\vspace{0.4cm}
\begin{myframe}[innerleftmargin = 5pt]
W3: Terminology: The names of the principles I (Classical) and II (Classical-Quantum) are somewhat confusing. Principle I contain classical components and quantum hardware (and is just called “Classical”), while principle II contains only classical components and is called " Classical-Quantum ".
\\ D4: To rethink the naming of the principles and to compare them with the state of the art. In the literature, there are established constructs such as "Hybrid Quantum-Classical Computing"
 \end{myframe}
 \vspace{0.2cm}
\para{Response} 
Thank you for pointing this out. To align with existing works and improve clarity, we have renamed `` Classical paradigm: Classical preprocessing \& postprocessing for quantum computing'' to ``Joint Quantum-Classical Computing paradigm: Classical preprocessing \& postprocessing for quantum computing.''
To avoid confusion, note that as overarching term for this paradigm we no longer use the term `hybrid'.
Similarly, we have renamed “  Classical-quantum paradigm: classical data represents quantum states and operations” to ``Classical Simulation of Quantum Computing,'' as this process represents data classically and requires only classical computers. 

We have revised paradigm names below to ensure they are appropriate and consistent with established terminology. 
We reordered the first two paradigms in the paper to improve the logical flow: classical $\rightarrow$joint quantum-classical$\rightarrow$pure quantum.
% \floris{This reviewer is right since simulation somehow only deals with classical, the first paradigm with  both, and the last only with quantum. Why not switch the order of the paradigms around?, as follows. 
Before:
\begin{enumerate}
\item 
 I Classical paradigm: classical preprocessing \& postprocessing for quantum computing. 
\item II  Classical-quantum paradigm: classical data represents quantum states and operations. 
\item III Quantum paradigm: quantum-native data storage and processing.
\end{enumerate}
After:
\begin{enumerate}
\item I  Classical simulation of quantum computing paradigm: classical data represents quantum states and operations. 
\item II Joint quantum-classical computing paradigm: classical preprocessing \& postprocessing for quantum computing.
\item III Pure quantum computing paradigm: quantum-native data storage and processing.
\end{enumerate}
% This is all up for discussion. It feels more natural to hybrid in the middle?

% \floris{Tim's suggestions are
% \begin{itemize}
%     \item I Supporting domain: Classical preprocessing \& postprocess-
% ing for quantum computing.
% \item II Representation domain: classical data represents quantum
% states and operations.
% \item III Quantum-memory domain: quantum-native data storage
% and processing.
% \end{itemize}
% Let's discuss on monday.}
% \tim{What about `Synergy domain' for Domain I?}


These paradigm name changes are reflected in Sec. 3 and 4 and are marked in \revisionfour{green}. 



\vspace{0.2cm}
\begin{myframe}[innerleftmargin = 5pt]
D5: For a better understanding of the principles in Fig. 2: These concepts should be better embedded in the running text and, if necessary, explained more succinctly. While 2a and 2c are referenced in the running text, 2b and 2d are not.

 \end{myframe}
 \vspace{0.2cm}
\para{Response} Thanks for pointing out this.  In Sec. 4.2 we have added further explanations of key terms while keeping them succinct, such as tensor networks and contraction order. We have also ensured their consistency with Fig. 2. Due to the six-page limit, we needed to remove the original Fig. 2c and 2d. 
To supplement this, we have provided detailed definitions, explanations and examples in Appendix A of our online technical report \cite{techreport}, 
% \footnote{\url{https://github.com/infiniData-Lab/Quantum/blob/main/technical_report.pdf}},
which is also included at the end of this letter. 






%  \bibliographystyle{ACM-Reference-Format}
% % \bibliographystyle{plain}
% \bibliography{ref.bib}

%\onecolumn
% \appendix
% \input{appendix.tex}

% \end{document}
% \endinput


==> misconceptions.tex <==
% \subsection{Avoiding a few misconceptions} 
\para{Avoiding a few misconceptions} 
\label{sec:misconceptions}
\tim{thinking about this, this can be probably be removed by: writing the second and third misconception as a single phrase into the intro,and removing the first.misconception alltogether}
%-------------------------------------------------------
% \rihan{a rigorous discussion that quantum-related data management is in infantile state: we are really just talking about qubits, not data; limited no. of qubits; lower-level gate-based computation; noisy}
% \tim{todo FILL with similarities and differences. ``Therefore a structured approach is needed''}
%-------------------------------------------------------
 % \floris{The aim of this section is not very clear to me}
% \tim{I updated, better now?}
%Quantum computing fundamentally differs from classical computing, often leading to misinterpretations about its capabilities and limitations.
We clarify a few potential misunderstandings, which might hinder the future research on quantum and classical data.
% before sketching our vision in the next sections.

%We here aim to take away a few potential misunderstandings about quantum computing and its relation to data management before sketching our vision in the next sections.
%These misconceptions can misdirect research directions in data management for quantum computing. Next, we aim to clarify a few common misunderstandings by examining key quantum computing principles and their implications.

% Similarities:
% \begin{itemize}
%     \item ...
% \end{itemize}
% Differences:
%\tim{@Rihan:
%\begin{itemize}
%\item{ I also shortened the text (original commented out). Please check}
%\item{I removed underline because it breaks latex formatting}
%\item{to clarify: superdense coding is for faster communication, not better compression: communicating 2 bits by sending 1 qubit, which was entangled beforehand to a qubit on the receiver's side.}
%\item{I rewrote the `data loading' part to also address Floris' question ``Perhaps a silly question, but these non-cloning, non-deletion and non-copying properties of quantum, don’t they rule out a native implementation of database, that is, if one would attempt to store data inside the qubits, there will be no way to do standard operations (like copy/delete) on them.''}
%\end{itemize}
%}
\begin{itemize}[leftmargin=*]
    \item \emph{A quantum computation does not perform parallel computation with exponentially-many processors.}
Classical parallel computing relies on splitting the task across many processors, each working \emph{independently}.
Quantum computing might at first sight look similar as a quantum state also represents multiple (exponentially-many) possibilities.
However, these possibilities are in a single \emph{superposed} state.
Moreover, to extract information from the state, one needs measurement (see Sec.~\ref{sssec:measurement}), which returns only one random outcome and also permanently changes the state.
    % \item \emph{\underline{Quantum computers do not run parallel computation}}: 
%    While quantum algorithms can exhibit substantial speedups for various computational problems, a common misconception of why this is possible is that quantum computers achieve fast computation by creating superpositions to execute exponentially many threads simultaneously. \ 
%    As discussed in Section~\ref{sec:classical-vs-quantum-data}, quantum measurements allow for the extraction of classical information from quantum states. \ 
%    Upon measurement, only one random outcome is extracted from the state, and the state changed permanently to the example we observe.
Since measurements only provide a probabilistic outcome determined by the quantum state's amplitudes, quantum computers cannot fully leverage parallel computation across all possible states simultaneously, and cannot conduct parallel computations on exponentially many threads. 
These make a quantum computation qualitatively different.
%Consequently, a quantum computation is qualitatively different from a parallel computation on exponentially-many processors.
% (it is even expected, but not proven(?), to be strictly weaker in the complexity-theoretic sense~\cite{}).
%It is therefore incorrect to say that quantum computing is the same as parallel computing with exponentially-many processors, 
%even though its computation power in the complexity-theoretic sense has not yet been fully pinpointed yet~\cite{}.
%quantum computing different from parallel computing with many processors, although the unconditional complexity-theoretic separation remains unproven.
%It is expected that there are tasks that quantum computers can efficiently tackle
%From a complexity-theory perspective, quantum computing is separate from
%lies somewhere in between parallel computing with exponentially-many processors (strict separation~\cite{}) and single-core classical computing (separation only proven for tasks with restricted input, i.e. promise problems~\cite{}).
%    \floris{I understand what you want to say but the latter goes beyond the capabilities of understanding by VLDB folks :-). Perhaps something more simple like this suffices: "Classical parallel computing relies on splitting the task across many processors, each working \emph{independently}. Quantum computing, on the other hand, handles multiple possibilities in a \emph{superposed} and \emph{entangled} state, and extracts one random outcome from the state, hereby permanently changing the state."}
%

\item \emph{There exist other quantum computers and database applications than only quantum annealers and QUBO solving.}
Quantum annealers~\cite{schonberger2023quantum} are a different type of quantum computers than the gate-based type explained above.
Recent works on accelerating database operations \cite{trummer2016multiple, fankhauser2021multiple, fankhauser2023multiple, SchonbergerSIGMOD22, schonberger2023SIGMOD, schonberger2023quantum, ScherzingerVLDB2023demo, GroppeIDEAS20, OJCC,  groppe2021optimizing} have a heavy focus on quantum annealers because some database problems are formulated as \emph{quadratic unconstrained binary optimization} (QUBO) problem, which are natural to solve on quantum annealers.
Although quantum annealing is in principle capable of running any quantum computation~\cite{aharonov2008adiabatic}, the focus is typically to solve QUBO on a specialized, non-universal quantum annealer such as the one by D-Wave Systems Inc.~\cite{dwavewebsite}.
% implementing the transverse Ising Hamiltonian https://journals.aps.org/rmp/pdf/10.1103/RevModPhys.94.015004
Our vision is not restricted to quantum annealing and QUBO, and broadens the view to universal quantum computing and other applications.
%However, gate-based quantum computers are universal, potentially enabling opportunities for database research that annealers do not.\tim{such as... Let's link to the rest of the paper} \floris{Is this all still true given \url{https://arxiv.org/abs/quant-ph/0405098}?}
  
%    Quantum computers come in various models, including quantum annealers and physical systems for implementing gate-based models such as superconducting \cite{}, semiconductor quantum dots \cite{}, and trapped ion \cite{}. %, neutral-atom, topological, and photonic quantum computers. 
%    Recent works on accelerating database operations \cite{trummer2016multiple, fankhauser2021multiple, fankhauser2023multiple, SchonbergerSIGMOD22, schonberger2023SIGMOD, schonberger2023quantum, ScherzingerVLDB2023demo, GroppeIDEAS20, OJCC,  groppe2021optimizing} have a heavy focus on quantum annealers and quantum-inspired classical hardware, i.e., digital annealers \cite{schonberger2023quantum}. The reason is, take query optimization \cite{trummer2016multiple, schonberger2023SIGMOD} for example, compared to gate-based quantum computers, quantum/digital annealers
%    provide a larger number of qubits/bits and better connectivity, which facilitates query optimization over more tables. Accordingly, the database problems \cite{trummer2016multiple, fankhauser2021multiple, fankhauser2023multiple, SchonbergerSIGMOD22, schonberger2023SIGMOD, schonberger2023quantum, ScherzingerVLDB2023demo, GroppeIDEAS20, OJCC,  groppe2021optimizing} are formulated as \emph{quadratic unconstrained binary optimization} (QUBO) problem, which is a typical problem solved by annealers.  
%    % So far, database studies only looked into QUBO \cite{trummer2016multiple, fankhauser2021multiple, fankhauser2023multiple, SchonbergerSIGMOD22, schonberger2023SIGMOD, schonberger2023quantum, ScherzingerVLDB2023demo, GroppeIDEAS20, OJCC,  groppe2021optimizing} and variational quantum circuit (VQC) algorithm \cite{GroppeQMLBiDEDE23}.  
%    Although quantum annealers or digital annealers offer more qubits and better qubit connectivity for tackling near-term optimization problems in databases, we should also put effort into gate-based quantum computers. 
%    Because quantum annealers are not universal quantum computers, we do not expect them to solve all computational problems that a full-power quantum computer can do. 
%    % \shih{revise the previous sentence to explain why quantum annealer is not as powerful as gate-based models, it solves a subset of problems; maybe with refs}
%    Exploring more quantum algorithms for gate-based models will bring more opportunities in this line of research. 

\item \emph{Loading large relational-database tables into a quantum computer will not be possible in the near term, and will maybe never be advantageous at all.}
In principle, one could load classical data onto a quantum chip by simply copying a single bit onto a quantum bit.
This however does not make use of quantum-computing properties such as superposition, which is crucial for a quantum advantage.
%Loading data to quantum amplitudes is done by
%Loading classical data onto a quantum chip in a way that takes advantage of exponential superposition is done by
%encoding the data as the quantum state's amplitudes.
		\tim{This can.now be shortened given the explanation of data loading in sec 2.2}
A functional alternative is to convert the data into a quantum circuit, which is either used directly as part of a quantum algorithm~\cite{suenderhauf2024blockencoding} or outputs a quantum state whose amplitudes hold the classical data~\cite{cortese2018loading}.
%The size of the circuit depends on the data and the used encoding, but is typically at least $O(\log(N))$ large for encoding $N$ classical bits.
For large amounts of data, this data-loading will not be beneficial practically in the near term, as qubits will be limited in number but also in lifetime (see Sec.~\ref{sec:classical-vs-quantum-data}), hindering their ability to store large amounts of data for a long time.
%However, given the decade-long perfectioning of performance and I/O for classical databases and the limited speed, lifetime and accuracy of quantum operations,
It is at the moment not clear for which applications this quantum data-loading will ever outweigh the use of the classical database for acting on the data directly~\cite{aaronson2015read,Preskill_2018}.
% also cite viamontes et al. "Is Quantum Search practical?"
In this work, we consider this question out of scope, as we focus on data management for supporting quantum technologies.
%, in contrast to the converse.
%a quantum data-management advantage.

%sketch how data management can contribute to quantum technologies, instead of the opposite question of 
%This avoids 

%describe different means in which classical data can contribute to a future with a quantum advantage.

%\tim{This is the vision that quantum computers will be good for computationally-hard problems which can be phrased succinctly}
%\floris{The above clearly dispels that an implementation of quantum database which stores all the day is not what one may want to aim for.}
%\todo[inline]{Tim: trying to answer Floris' question here: Perhaps a silly question, but these non-cloning, non-deletion and non-copying properties of quantum, don’t they rule out a native implementation of database, that is, if one would attempt to store data inside the qubits, there will be no way to do standard operations (like copy/delete) on them. }

%For the existing limitation of qubits we cannot process any industrial-level tables in the classical database in a quantum processor due to the constraint of limited quantum resources. It may be not worth the effort to import all classical data into a quantum processor. 
%    Furthermore, it lacks generic methods to transform classical data to a quantum state that encodes the information in the amplitudes, which is essential for quantum algorithms to exhibit speedups (see, e.g., \cite{harrow2009quantum}). 
%    It is important to think about which subset of classical data (or a sketch, metadata) needs to be encoded and passed to a quantum device, and design corresponding quantum algorithms for transforming it to useful quantum states. 

%\todo[inline]{mention loading data onto a quantum chip, which is done by preparing a quantum circuit, not copying}


%For the existing limitation of qubits we cannot process any industrial-level tables in the classical database in a quantum processor due to the constraint of limited quantum resources. It may be not worth the effort to import all classical data into a quantum processor. 
%    Furthermore, it lacks generic methods to transform classical data to a quantum state that encodes the information in the amplitudes, which is essential for quantum algorithms to exhibit speedups (see, e.g., \cite{harrow2009quantum}). 
%    It is important to think about which subset of classical data (or a sketch, metadata) needs to be encoded and passed to a quantum device, and design corresponding quantum algorithms for transforming it to useful quantum states. 


    % \item \emph{\underline{query model is different}}: superposition is different from parallel computing;
    % cannot extract classical information in general without destroying the properties of the quantum state. Measurement destroys information.
    


\end{itemize}


==> oldSec4.tex <==
\section{Near-term research problems}
\label{sec:structure}
\floris{This is Rihan's version}

\begin{figure*}[t]
    \centering
        % \includegraphics[width=\linewidth]{figures/tn-Page-1.drawio.pdf}
                \includegraphics[width=\linewidth]{figures/tn-Page-1.drawio_new.pdf}
    % \includegraphics[width=0.7\linewidth]{figures/tn-Page-1}
    \caption{(a) The 3-qubit  GHZ state  $D=\frac{1}{\sqrt 2}(\ket{000}+\ket{111})$ represented in state vector, whose amplitude is $2^3=8$. (b) GHZ state represented as matrix product states, factorized as three tensors. Each qubit is represented as a tensor. For understandability we write the tensors in  vector/matrix form. 
    (c) Tensor contraction between A and B.
    (d) Quantum operation, Hardmard gate, represented in matrix product operators.} 

    \label{fig:tensors_example}
         \vspace{-0.2cm}
\end{figure*}


In this section, we explore the open research questions across the three paradigms of quantum data management. To provide specific directions,  Sections~\ref{ssec:simu} and \ref{ssec:dbq} focus on a key challenge within Paradigm II, the hybrid classical-quantum approach. By integrating recent advancements from the database community, we identify and discuss emerging research opportunities. In Section 4.3, we broaden our scope to highlight further opportunities across all three paradigms.

\subsection{Quantum challenge of simulation} 
\label{ssec:simu}
% \floris{I think it is perhaps more insightfull to describe the problem of simulation in more details? There are various notions, strong/weak and for some classes, strong is $\#P$-hard whereas weak is poly, in general weak is PH-hard. Clifford stuff is poly. What should we focus on?}
% \floris{Perhaps weak simulation is not good but it may open up extra challenges \url{https://arxiv.org/pdf/2007.15285} Theoretically, connections with tractable circuits \url{https://starai.cs.ucla.edu/papers/ProbCirc20.pdf} maybe be possible as well?}
% \floris{\url{https://arxiv.org/abs/0811.0898} argues against strong simulation ...}
% \floris{Another point: \url{https://arxiv.org/pdf/2406.16142} refers to $d$-sparse quantum states (those having at most $d$  nonzero amplitudes). Not sure whether this is *the* reference for that, but just pointing out sparse things exist in the quantum world.}
\emph{Simulation} is the process of emulating quantum computation,  
allowing researchers to model and analyze quantum processes as if they were running on actual quantum hardware
\cite{young2023simulatingquantumcomputationsclassical, xu2023herculeantaskclassicalsimulation}.\footnote{In this work, by simulation we refer to \emph{classical simulation}. Another similar term is \emph{quantum simulation} \cite{georgescu2014quantum}, which refers to simulating quantum mechanics, a topic studied in physics.} % and out of the scope of this paper. } 
Simulations are of upmost importance in the NISQ era. Indeed, take quantum supremacy \cite{boixo2018characterizing} for example, which aims to demonstrate the superior capabilities of quantum computers over classical computers. 
% In the NISQ era, researchers are still exploring how powerful quantum computing will be,  such as calculation that is infeasible for any classical computer, even the most powerful supercomputers. A core question in near-term quantum computing is quantum supremacy : how much do quantum computing methods and hardware surpass classical computational methods and hardware? 
Large-scale quantum computers are not yet available in the NISQ era, simulation is indispensable to compare scalable quantum computers with classical computers. 
Another use of simulations is for the development of new quantum algorithms. Indeed, simulation enables researchers to design, debug, and validate the correctness of quantum algorithms before deploying them on expensive quantum processors. 
% One of the key challenges in quantum computing is verifying that a quantum algorithm is functioning correctly, especially when quantum hardware is prone to errors. Classical simulators can precisely calculate the expected outcomes of quantum circuits for small to moderate-sized systems. By comparing the outputs of quantum hardware to those of a classical simulation, researchers can validate the correctness of quantum algorithms and ensure they are implemented as intended.
% \floris{I would also briefly explain what simulation actually entails. }
% Using classical representation and methods to simulate quantum computations, is one of the main driving forces in the development of quantum technologies such as new quantum algorithms, error correction, and quantum circuit compilation \cite{jones2019quest, villalonga2019flexible,  xu2023herculeantaskclassicalsimulation}. \floris{Perhaps add why simulation is needed? Eg., because running quantum system is slow/expensive?}
% In the NISQ era, 
Other examples illustrating that simulation is a foundational tool in the NISQ era relate to
% In general, in the NISQ era, simulation serves as a foundational tool across key areas of quantum computing, including  quantum supremacy, quantum algorithms, 
quantum hardware, error correction, and the exploration of potential quantum applications \cite{xu2023herculeantaskclassicalsimulation}. 
% Various notions of simulation can be found in the literature \ref{}. Here, we focus on strong simulation in which, given  (family of) quantum circuits and a final measurement, one wants
% to compute the measured probabilities to a certain precision using
% a classical computer. 

The major practical bottleneck of simulation is  \emph{scalability} \cite{boixo2018characterizing, 8869942, xu2023herculeantaskclassicalsimulation, young2023simulatingquantumcomputationsclassical}. 
Typically, a quantum state is represented as a vector, e.g., the two-qubit state in Example~\ref{exmp:EPR pair}. Additionally, Fig.~\ref{fig:tensors_example}a shows the vector form of a three-qubit state, Greenberger-Horne-Zeilinger (GHZ) state.
% , represented as a state vector with amplitude of 8. 
When simulating a quantum state with $n$ qubits, the state vector's amplitude is $2^n$, which grows exponentially 
% as the number of qubits $n$ in the state increases, 
as $n$  increases, 
hitting hardware limitations. 
For instance, in an experiment demonstrating quantum supremacy \cite{boixo2018characterizing}, the wavefunction needs to be stored in random-access memory. 
% in single precision, requiring  $2^{n+3}$ bytes, 
%$2^{n+4}$ for the amplitude of the vector, and 4 for the double-precision complex numbers
% where $n$ is the number of qubits. 
It required 2.25 petabytes for 48 qubits, reaching the memory limits of today's supercomputers.  To overcome the memory restriction, existing simulation tools have explored approximation \cite{vidal2003efficient, medvidovic2021classical, jonsson2018neural}, data compression \cite{wu2019full}, 
%tensor network  
parallelization \cite{huang2021efficient},  and distributed computing \cite{smelyanskiy2016qhipsterquantumhighperformance}. 
 
An rather unexplored direction is to store the simulation data in a DBMS, i.e., out-of-core simulations over databases, which has the potential to facilitate faster simulation of more qubits and to lower the hardware requirements on memory size and computational power. 
However, storing and querying such quantum data in modern DBMS is not straightforward. A widely adopted data structure for simulating quantum computation is \emph{tensor networks}.
% To represent qubit states and quantum operations, 
% tensor networks are one of the most widely used data structures.
A \emph{tensor} is a multidimensional array, and the dimensions along which a tensor extends are its \emph{indices}. 
 % The total number of indices is referred to as {rank}
 For example, a vector is a one-dimensional tensor, and a matrix is a two-dimensional tensor.  
 A \emph{tensor network} is a collection of tensors represented as nodes, 
 % with their connections represented as edges  
with the shared indices contracted, which leads to a more compact and efficient representation \cite{biamonte2020lecturesquantumtensornetworks}. 
% Tensor networks are widely used in machine learning \cite{} and quantum computing \cite{}. 
Tensor contraction is the summation of shared indices between tensors.

% \floris{moved this away from above.. let's discuss  }
% \cite{pan2021simulatingsycamorequantumsupremacy}, such as
We next exemplify tensor networks by means of
 \emph{matrix product states (MPS)}  \cite{perez2007matrix, orus2014practical} for representing quantum states and \emph{matrix product operator (MPO)}  \cite{pirvu2010matrix} for quantum operations. 
 % , which are well-supported by open-source libraries  \cite{broughton2020tensorflow}. 
 
\begin{exmp} (\textbf{Quantum state in tensor network}) 
In Fig.~\ref{fig:tensors_example}b, the three-qubit GHZ state is presented in MPS, a factorized form of 3 tensors.   
The three qubits $A$, $B$, and $C$ are represented as nodes, and each node can be written as a tensor. To simplify the visualization, we illustrate the tensor $A$ of size $2*2*1$ as $A^0$ and $A^1$. It is possible to transform MPS to the state vector. For instance, the value of the last element in GHZ's vector, i.e., $D_{111}$ for state $\ket{111}$, can be computed by the tensor computation of $A^1B^1C^1$. 
\end{exmp}
\begin{exmp} (\textbf{Tensor contraction}) 
Fig.~\ref{fig:tensors_example}c depicts two two-dimensional tensors, matrices $A_{ik}$ and $B_{kj}$, which share the same index $k$. The  contraction  of $A_{ik}$ and $B_{kj}$ is the matrix multiplication operation $C_{ij}=\sum_{k}^{}A_{ik} B_{kj}$, which is often written as $A_{ik} B_{kj}$   in Einstein notion \cite{albert1916foundation}. 
% The simulation takes two inputs: the qubit state and a bitstring representing the measurements, and produces another bitstring as output. 
% The contraction of the tensor network gives the amplitude of the output bitstring. 
\end{exmp}

Quantum algorithms such as Grover's algorithm \cite{grover1996fast}, are implemented via quantum circuits. A quantum circuit include qubits, gates, and measurement. The gates  perform operations on qubits, and manipulate the qubit states. 
To represent quantum circuits,  in a tensor network a quantum state is represented as a node, and the gate operations can be seen as a series of tensor contractions. That is tensor contraction is the core operation when applying an MPO to an MPS or when measuring an MPS
\begin{exmp} (\textbf{Quantum operations in tensor network})  
Fig.~\ref{fig:tensors_example}d shows an example of a quantum operation, Hadamard gate, in MPO. 
The Hadamard gate H, represented as nodes $E$ and $F$, are performed on qubit states $A$ and $B$. The gate operation H is conducted by contracting $E$ and $A$,  $F$ and $B$, respectively, leading to new states of qubits $A'$ and $B'$. 
% The simulation takes two inputs: the qubit state and a bitstring representing the measurements, and produces another bitstring as output. 
% The contraction of the tensor network gives the amplitude of the output bitstring. 
\end{exmp}

\floris{It may be good for a db person to also get a feeling what the measurement is about and how it is implemented?}
As illustrated in above examples, the quantum-specific representations used in simulating quantum states and operations are different from the typical data representations and opertions supported in traditional database systems, which lay the unique challenges to out-of-core  simulations over databases.







% \floris{We may need a good argument why HPC people need db folks. I know it is memory, but we may never beat HPC in terms of speed.}

\subsection{Database to the rescue} 
\label{ssec:dbq}
 
The database community has a substantial body of work on tensor computation, 
especially with the recent synergies between databases and machine learning (ML) such as \emph{learning ML models over relational data} \cite{Khamis2020, boehm2023optimizing, Makrynioti2019survey, zhou2020database, 10107490}. These studies range from high-level representations to the runtime optimization of ML workflows. At the representation level, numerous studies represent data as tensors \cite{DBLP:journals/pvldb/KoutsoukosNKSAI21} and aim to integrate relational and tensor operations, with a commonly used algebraic notion being semi-rings \cite{DBLP:conf/sigmod/SchleichOC16, DBLP:conf/pods/Khamis0NOS18, DBLP:journals/pvldb/HuangSL023}. Meanwhile, system-building endeavors \cite{DBLP:conf/sigmod/GaoLPJ17, DBLP:conf/icde/LuoGGPJ17, DBLP:conf/sigmod/NikolicO18, DBLP:conf/sigmod/SchleichOK0N19, DBLP:conf/cidr/BoehmADGIKLPR20, DBLP:conf/osdi/NakandalaSYKCWI20, DBLP:journals/pvldb/HeNBSSPCCKI22, 10.1145/3514221.3526141} focus on performance efficiency and scalability, 
% LMFAO \cite{DBLP:conf/sigmod/SchleichOK0N19}
% F-IVM \cite{DBLP:conf/sigmod/NikolicO18}
% SystemDS \cite{DBLP:conf/cidr/BoehmADGIKLPR20}, 
% Hummingbird \cite{DBLP:conf/osdi/NakandalaSYKCWI20}, 
% TQP \cite{DBLP:journals/pvldb/HeNBSSPCCKI22}, 
% Raven \cite{10.1145/3514221.3526141} 
% SimSQL \cite{DBLP:conf/sigmod/GaoLPJ17, DBLP:conf/icde/LuoGGPJ17}
 employing optimization techniques during compilation (e.g., operator fusion \cite{boehm2018optimizing}) and runtime (e.g., parallelization \cite{DBLP:journals/pvldb/BoehmTRSTBV14}).

 



\subsubsection{Representation gaps} 

Initial efforts from the database community \cite{einsteinSQL2023, Trummer24} have started to tackle the out-of-core simulation challenge by mapping quantum states and gates to SQL queries. In \cite{einsteinSQL2023}, qubit states and gates are represented as tensor networks, with the sparse tensors in COO format\footnote{\url{https://docs.scipy.org/doc/scipy/reference/generated/scipy.sparse.coo_matrix.html}} and Einstein summation
 operation are mapped to SQL queries. The recent abstract \cite{Trummer24} provides the initial idea of supporting dense vectors by adding the SQL UNION ALL and CASE statements. Despite these early efforts that support basic quantum gates and states up to 10-qubit, the core challenges of representing general quantum states and operations in DBMS and scalability remain untouched. As mentioned above, from the database community intensive effort has been put into supporting tensor computation  
 % sparse tensors 
 at theoretical \cite{Khamis2020} and system aspect \cite{boehm2023optimizing}. Below, we initiate the discussion of filling the research gaps with a few open questions. 
 
\vspace{0.2cm}
\begin{myframe}[roundcorner=3pt]
Q1. \textit{How to design a \textbf{good} data abstraction to represent quantum states?} 
\end{myframe}
% \floris{I would start with the fact that on a logical level, quantum systems are commonly described by tensor networks, and as such, any db attempt to assist in quantum simulation must have the functionality  support the tensor computation. }
% \floris{I would use MPS etc as examples of how to represent tensor networks, i.e., physical level, that is, actual representation of tensor and their computation.}


With quantum data, i.e., quantum states, stored in DBMSs, we aim to support the simulation of quantum circuits. One of first questions is about finding the right data abstractions.
% at the logical level, which are independent from their physical implementation. We discuss the physical implementation later with Q3 and Q4. 
% data model,
% While we forsee the rich studies following this direction, 
We emphasize main requirements on the data abstraction: \emph{expressivity},  \emph{succinctness}, and \emph{equivalence}. 

\emph{Expressivity.}
First, the data abstraction should support representing possible quantum states, which also facilitates the gate and measurement operations of a quantum circuit. In Sec.~\ref{sec:classical-vs-quantum-data} we have explained key features of quantum data. Take entanglement for instance, in MPS, the level of entanglement is specified by a parameter called \emph{bond dimension}, which is the rank shared between two neighbouring tensors.  Bond dimension affects the dimensionality  of the tensors. We omit the complicated explanation of entanglement entropy and calculations here, but illustrate the impact of entanglement with the below example. 

\begin{example}
In the GHZ state, there are \emph{two} possible entangled components : $\ket{000}$ and $\ket{111}$. 
Thus, in Fig.~\ref{fig:tensors_example}b, the value of bond dimension is set as two, i.e., the shared rank value between A and B, B and C is two, illustrated in red color. This also affects the dimensions of tensors in MPS, which are marked in red in Fig.~\ref{fig:tensors_example}b. 
\end{example}


With qubit state as vectors (Fig.~\ref{fig:tensors_example}a) or tensors (Fig.~\ref{fig:tensors_example}b), straightforward choices of data abstraction from existing database literature include tensors \cite{DBLP:journals/pvldb/KoutsoukosNKSAI21}, tables \cite{einsteinSQL2023, Trummer24}, or their combination \cite{DBLP:conf/cidr/BoehmADGIKLPR20}. As explained in above example, to preserve the information in quantum states, we also need to consider their quantum-specific features. 

\emph{Succinctness.} In the context of databases, succinctness refers to the efficiency of data representation and storage. A succinct data abstraction minimizes the amount of space needed to store data while still allowing for efficient query processing. As discussed in Sec.~\ref{ssec:simu}, it is important to reduce the space representing a quantum state. 
This is affected with two parameters: number of qubits and the level of entanglement. For simulations based on state vector, the vector size grows exponentially as the number of qubits $n$ grows, i.e., $2^n$.
For MPS, it applies smaller matrices to preserve the information about a quantum state. The number of tensors is the same as the number of qubits. However, the dimensionality of the MPS tensors grow fast with the level of entanglement. It is interesting to explore with we can utilize existing studies of data abastraction from database community to find succinct abstractions for simulating quantum states.

\emph{Equivalence.} Often to choose the optimal data structure for simulation, it is important to check whether two given data structures are equivalent, e.g., whether the state vector in Fig.~\ref{fig:tensors_example}a and MPS in  Fig.~\ref{fig:tensors_example}b are equivalent (the answer is yes). It is an interesting problem how to define data abstraction that support such equivalence check. 
 
  
% \footnote{Tensor networks are widely used in quantum computing beyond simulation. Quantum circuits are a special class of tensor networks with unitary constraints. }




% \para{From formalism to implementation}
% \para{From formal properties to implementation}
% \textbf{From logical level to physical level.}  



% To tackle the data structure question from the implementation perspective,



\vspace{0.2cm}
\begin{myframe}[roundcorner=3pt]
Q2. \textit{Can we define a query language that serves as an abstraction layer \textbf{unifying} classical database operations and simulation programs?} 
\end{myframe}

 % \floris{Rihan: reference of complexity/tractability in db: \url{https://www.cs.rice.edu/~vardi/papers/stoc82.pdf}}

 The existing simulators for quantum computing are mostly implemented in Python \cite{nvidia_cuquantum_team_2022_6964823, vincent2022jet},  C++ \cite{qsim, vincent2022jet} or Julia \cite{luo2020yao}. There are also dedicated quantum programming languages and domain-specific compilation techniques, see the survey \cite{heim2020quantum}. 
% \floris{As described in \url{https://arxiv.org/pdf/2311.16505} Section 3.1, there are quantum programming languages, like \url{https://www.quantum-inspire.com/kbase/cqasm/} and perhaps others. One may need to differentiate from such attempts as well?}
The simulation workload, which includes preparing the initial state, gate, and measurement, requires intensive tensor computation. 
By connecting the simulators with data management systems, we have a pipeline of simulation workloads that are tensor computation and database operations.
To enable the optimization in the end-to-end pipeline


Besides gates and measurement, common quantum operations\footnote{For a more detailed explanation from the quantum computing perspective,  please refer to \cite{young2023simulatingquantumcomputationsclassical}.} also include addition and inner product between states, sampling measurement outcomes, and checking whether two states are equivalent   \cite{vinkhuijzen2024knowledge}.  \floris{Can we make it a bit more explicit what typical quantum operations are needed..}

To tackle the representation question from the logical level, we need to study formal properties such as \emph{expressive power} and \emph{tractability}. A key challenge in simulating quantum circuits is developing memory-efficient data structures that minimize memory usage while being computationally efficient for gate and measurement operations.
At the logical level, we need the data structure to be expressive enough to represent the general quantum states and gates and ideally tractable, i.e., the operation on this data structure finishes in polynomial time in the size of the input. New notions of equivalence check could be useful to verify whether two quantum states are exactly or approximately equivalent, analogous to checking equivalent conjunctive queries \cite{fagin2012local, fagin2008towards, cohen2007deciding}. \floris{Could this be undecidable, or are the results on this showing it is tractable? Perhaps ask Tim?}


Quantum circuits
Linear algebra, with tensor network such as




\floris{we may need to cite again, FAQ, LARA and other attempts for combining tensor and relational?}
We need a query language that can query matrices and tensors, possibly also relational tables. Such a query language would serve as an abstraction for both relational algebra and tensor computation operations. It is necessary to study the formal properties of this language, such as expressive power, complexity, etc. It is also interesting to explore whether we can obtain a generalization such as semi-ring. 
Moreover, many database tasks can
 be rephrased to problems on Boolean functions. By combining existing tractability results ofthe tensor network, can we derive the tractability of the main operation supported by this query language?
% matrix languages \cite{brijder2019matlang}.
% \floris{I don't think the matrix language developed there is human comprehensible. How complex can the queries be that quantum simulation people ask? And given building blocks, is there need for composing them? Who are the users? }



 
\subsubsection{Optimization gaps} 
Initial efforts \cite{einsteinSQL2023, Trummer24} still have not yet touched the challenges of system building and the massive opportunities of optimization. Although the computation of simulation tasks can be generalized as matrix multiplication, they differ significantly from the typical ML workflow studied in  \cite{DBLP:conf/sigmod/GaoLPJ17, DBLP:conf/icde/LuoGGPJ17, DBLP:conf/sigmod/NikolicO18, DBLP:conf/sigmod/SchleichOK0N19, DBLP:journals/pvldb/BoehmTRSTBV14, DBLP:conf/cidr/BoehmADGIKLPR20, DBLP:conf/osdi/NakandalaSYKCWI20, DBLP:journals/pvldb/HeNBSSPCCKI22, 10.1145/3514221.3526141}. Another open challenge is on the classical DBMS side. An interesting experiment result from \cite{einsteinSQL2023} is that it is questionable whether the query optimizers in existing RDBMS can effectively optimize SQL queries of simulation workload.  

\vspace{0.2cm}
\begin{myframe}[roundcorner=3pt]
Q3. \textit{Shall we push the simulation workload to existing DBMS?  Or design new tensor-native systems for simulating quantum states?}
\end{myframe}

By mapping the typical simulation workload to SQL queries, we can enjoy the efficiency and portability of modern database systems. We might need to design intermediate representations and seek more effective query optimization, even beyond existing query optimization techniques \cite{neumann2024closing}. On the other hand, a valuable experience of supporting ML workload \cite{DBLP:conf/cidr/BoehmADGIKLPR20} is that designing dedicated ML systems while adapting database techniques might bring more usability and efficiency. By adapting the representations of common quantum representations, such as tensor networks and existing simulation frameworks, the effort of building simulation tools using databases may be more easily adopted by quantum researchers. 

\vspace{0.2cm}
\begin{myframe}[roundcorner=3pt]
Q4. \textit{How to support efficient tensor computation of simulating quantum states and operations with database technologies?} 
\end{myframe}


% Tensor program 
Tensor computation optimization has been intensively studied by the database, compiler, and HPC communities \cite{schleich2023optimizing, boehm2023optimizing}. The system-building efforts include 
Taco \cite{kjolstad2017tensor}, 
 SystemML \cite{boehm2018optimizing}, TVM \cite{chen2018tvm}, Halide \cite{ragan2013halide}, TASO \cite{jia2019taso}, SystemDS \cite{DBLP:conf/cidr/BoehmADGIKLPR20}, and STOREL \cite{schleich2023optimizing}. 
With tensors as the representation, the runtime performance depends on the operations in the tensor program, the sparsity, and \emph{memory layouts}, i.e., how the tensors are stored in the memory, which can be row-major or column-major. The optimal memory layouts for runtime performance depend on the tensor computation operations (e.g., matrix multiplication), hardware (e.g., GPU module) \cite{jia2019taso}, and the sparsity of the data (dense or sparse). 
Recent work supports sparse matrix computation in relational databases \cite{DBLP:conf/pods/Khamis0NOS18}. There are also efforts to have a unified intermediate representation of relational algebra and tensor computation operations, and end-to-end pipeline optimization \cite{karanasos2extending, DBLP:journals/pvldb/HeNBSSPCCKI22}. The aforementioned works lay the foundation for supporting the tensor computation of simulating quantum circuits over DBMS. However, it is still an open area of how to tailor these techniques for quantum-specific characteristics: sparsity of tensors in the tensor network and compositional pipeline of quantum operations such as gates, measurement, and sampling. 

To identify the most suitable implementation of simulating quantum states and operations, the starting point is the large body of recent database studies exploring and supporting  ML applications over relational data \cite{Khamis2020, boehm2023optimizing, Makrynioti2019survey, zhou2020database, 10107490}. 
However, although both ML and quantum applications may share atomic building blocks of 
 matrices, tensors %\cite{DBLP:conf/cidr/BoehmADGIKLPR20}, 
 and tables, we need to tackle the quantum-specific challenges. 
For instance, the matrices representing quantum states, as shown in Fig.~\ref{fig:tensors_example}, their sparsity and size vary and may lead to different choices of data storage formats \cite{zeng2023empirical}, e.g.,  Parquet, ORC, HDF5, and Zarr.
% file format for large-scale data analytics
The compositional operations of quantum circuits may have different requirements for the data structure, such as searching the most efficient paths for tensor contraction.



% Q1: how to design a new data structure for centralized databases on quantum computers or distributed databases over the quantum internet, such that we can perform complicated computation?


% Q2: What is the optimum data structure that maximizes the quantum advantage and minimizes the quantum resources? 

% Q3: Can existing classical data structure help improve quantum data structures, e.g., simulation?

% \begin{figure}
% \centering
%  \includegraphics[width=\linewidth]{figures/arc.drawio.pdf}  
% %for discussion only, cannot use this picture
% \caption{Layered architecture}
% \label{fig:paradigms}
%  % \vspace{-0.4cm}
% \end{figure}


\subsection{More data management opportunities} 
\label{ssec:opp}

Beyond simulation for quantum computing,
quantum-related research is broad, e.g., error correction \cite{shor1995scheme, PhysRevLett.77.793, gottesman1997stabilizer}, %quantum mechanics \cite{}, quantum chemistry \cite{mcardle2020quantum}, 
quantum network \cite{wehner2018quantum, dahlberg2019link}. Next, we expand our discussion to uncover more opportunities spanning all three paradigms in Fig.~\ref{fig:paradigms}.

\vspace{0.2cm}
\begin{myframe}[roundcorner=3pt]
Q5. \textit{Can we develop novel data structures, formal methods, and systems for more quantum use cases?}  
\end{myframe}
 
\para{Quantum error correction \& Graph analytics  } 
As discussed in Sec.~\ref{ssec:nisq}, quantum processors in the NISQ era are inherently vulnerable to noise, which can significantly impact the reliability of computation results.  Quantum error correction is crucial for ensuring reliable quantum computation. This process consists of two main phases: coding and decoding. In the coding phase, the input quantum information is coded into a quantum error-correcting code such as the surface code \cite{fowler2012surface, bravyi2018correcting, fowler2009high}. During the decoding phase, errors are detected and corrected. Typically, errors are modeled as graphs. The error detection and correction algorithms, referred to as \emph{decoders}, are built upon graph theory such as graph matching \cite{fowler2015minimum} and shortest path problems. 
Exploring the recent effort of graph analytics \cite{10.14778/3611540.3611577, yan2005substructure, 10.1145/3448016.3452826} and graph databases \cite{tian2023world} such as Neo4j\footnote{\url{https://neo4j.com/}},  TigerGraph\footnote{\url{https://www.tigergraph.com/}}, might yield valuable insights to advance these error correction techniques. 
A unique challenge in graph data management for error correction is balancing accuracy and efficiency \cite{iolius2024decodingalgorithmssurfacecodes}. A more accurate decoder generally requires higher computational complexity and, therefore, operates more slowly. However, the fidelity of a qubit decays over time, demanding fast error detection and correction by the decoder. 

\rihan{ask Floris what this indicates}
\floris{\url{https://arxiv.org/abs/1901.03744} this is a paper based on FOCS 2019 paper on studying WMPC in the MPC model, the latter is being studied in db as well.}
\para{Quantum experiments \& Scientific data management} Quantum experiments, like any other scientific experiences, generate data and require data management. 
For instance, quantum mechanics experiments on supercomputers often apply HDF5 files to store data and XML files to store metadata \cite{de2011implementing}. 
Typical challenges include avoiding I/O bottleneck (efficient I/O parallelization) and handling the sheer volume and heterogeneity of data files.  The scientific data management challenge is also domain-dependent, e.g., experiment data from quantum chemistry \cite{rossi2014code} or condensed-matter physics.  These new data-related quantum challenges may require us to push forward the frontier of existing database topics such as metadata management \cite{bernstein2000panel, amano2014xml} and data formats \cite{zeng2023empirical}. It is also interesting to explore how to build novel data lakes \cite{nargesian2019data, hai2023data} or lakehouses \cite{armbrust2020delta, armbrust2021Lakehouse, jainanalyzing} for quantum applications.
% , i.e., \emph{quantum data lakes}.

% \para{Time series and stream processing}




\para{Quantum network \& Distributed databases} 
% \para{Distributed \& cloud-native databases} 
Quantum network holds the potential to offer advantages and capabilities beyond the power of classical internet systems, e.g., secure communication \cite{5438603} or distributed computing \cite{nickerson2014freely}. 
 Developing quantum network requires simulator tools such as NetSquid \cite{coopmans2021netsquid}, SimulaQron \cite{dahlberg2018simulaqron},  QuNetSim \cite{diadamo2021qunetsim}. 
It is interesting to explore whether these tools can be supported and enhanced by distributed databases \cite{ozsu1999principles} or cloud-native databases \cite{10574374}.







 










 

% \para{Indexing}
% \subsection{Other directions}
% Database acceleration using quantum computers \cite{ccalikyilmaz2023opportunities} \td{List recent qo, tm, di papers using QUBO}

% Quantum databases  \td{Early works realizing SQL using gates, and recent work from TUM}

% \subsection{Open-source tools}
% \para{General-purpose libraries and platform}

% \para{Quantum internet tools}

% \para{Post-quantum cryptography libraries}
% Liboqs, sandwich





 

==> table.tex <==
% \begin{table}[h]
%     \centering
%     \caption{Comparison of Simulation with and without Databases}
%     \begin{tabular}{p{4cm} p{6cm} p{6cm}}
%         \toprule
%         \textbf{Feature} & \textbf{Simulation Without Databases} & \textbf{Simulation With Databases} \\
%         \midrule
%         \textbf{Data Storage} & Data is stored in flat files or memory, leading to scalability issues with large datasets. & Utilizes database capabilities for structured data storage, enabling scalability with large datasets. \\
%         \textbf{Efficiency of Data Retrieval} & Manual or ad-hoc data retrieval, which can be time-consuming. & Optimized querying and indexing, leading to faster and more efficient data retrieval. \\
%         \textbf{Simulation Speed} & May achieve faster execution due to lightweight setup but lacks optimized data access. & Slight overhead due to database interaction but benefits from improved data access speed, especially for large-scale data. \\
%         \textbf{Integration with Existing Tools} & Requires custom solutions for integrating with analysis tools. & Easily integrates with existing database-supported tools, simplifying workflows and reducing development effort. \\
%         \textbf{Data Consistency and Integrity} & Relies on custom checks, prone to errors with large-scale simulations. & Built-in support for data consistency and integrity checks, reducing errors in data handling. \\
%         \textbf{Resource Management} & Limited resource management, potentially leading to higher memory usage. & Databases manage memory and disk usage more efficiently, optimizing resource allocation. \\
%         \textbf{Scalability} & Limited by the capacity of the computing environment. & Can scale horizontally using distributed databases, supporting larger simulations. \\
%         \textbf{Availability of Existing Simulators} & Some existing simulators promise efficient execution but may lack flexibility in data handling. & Databases support flexibility in combining simulators with tailored data handling and advanced analytics. \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:comparison}
% \end{table}

\begin{table*}[t]
\centering
\caption{Comparison of the Use of Databases for Quantum Circuit Evaluation and Tensor Network Computations}
\begin{tabular}{|p{3cm}|p{6cm}|p{6cm}|}
\hline
\textbf{Feature} & \textbf{Without Databases} & \textbf{With Databases} \\
\hline
Data Storage & Results from quantum circuit evaluation and tensor network computations are stored in flat files (e.g., HDF5 or custom formats), which lack structure and scalability for complex data. & Simulation data, including circuit results and tensor networks, is stored in structured, scalable, and indexable formats, enabling efficient organization and access. \\
\hline
Consistency, Recovery, Transactions & Data consistency and recovery depend on manual checks and scripts, leading to potential errors, especially with large-scale quantum simulations. & Built-in consistency checks, transactional support, and recovery mechanisms ensure reliability and error-free data handling, crucial for iterative computations. \\
\hline
Data Retrieval & Retrieving specific circuit results or tensor configurations requires custom scripts, which are slower and less efficient, especially for high-dimensional data. & Databases support fast and optimized retrieval of quantum states, gate configurations, and tensor data through advanced querying mechanisms. \\
\hline
Query Optimization & Data retrieval is not optimized, requiring manual indexing or exhaustive searches for locating specific tensor states or quantum gate sequences. & Databases utilize indexing, caching, and execution plans to optimize queries, drastically improving performance for accessing specific circuit or tensor data. \\
\hline
Query Languages & Accessing data relies on low-level programming or manual parsing, which is inefficient for querying specific quantum states or tensor relationships. & High-level query languages (e.g., SQL) simplify retrieval, enabling efficient queries for tensor structures, gate sequences, and circuit outputs. \\
\hline
Simulation Speed & Simulations may run faster as data is directly written to flat files, but performance suffers during subsequent retrieval or reuse of intermediate results. & Slightly slower due to database overhead during storage, but the faster retrieval and reusability of intermediate states improve overall workflow efficiency. \\
\hline
Resource Use & Requires significant memory for storing and processing tensor data or quantum state amplitudes, with potential redundancy in flat files. & Databases manage memory and disk space efficiently by storing only necessary data and leveraging dynamic retrieval for large quantum systems. \\
\hline
Scalability & Scaling simulations is limited by the hardware capacity, making it challenging to manage large tensor networks or quantum circuit outputs. & Databases can scale horizontally, supporting distributed computations and managing large-scale tensor and quantum circuit data seamlessly. \\
\hline
Integration & Manual integration with quantum simulation tools requires custom development, adding significant overhead to manage inputs, outputs, and dependencies. & Databases integrate seamlessly with quantum simulation frameworks and tools, allowing smoother workflows for evaluating circuits and tensor networks. \\
\hline
Tensor Data Management & Managing large tensor networks requires custom serialization and deserialization, increasing complexity and processing time. & Databases offer structured storage for tensor networks, supporting efficient slicing, indexing, and retrieval of tensor elements. \\
\hline
Quantum Circuit Data Handling & Handling quantum circuit data (e.g., gate sequences and states) requires ad-hoc solutions to organize and reuse results. & Databases provide robust support for organizing quantum circuits, storing gate sequences, parameters, and results in a reusable and searchable format. \\
\hline
\end{tabular}
\end{table*}

